Confined Gradient Descent: Privacy-preserving Optimization for Federated Learning

Federated learning enables multiple participants to collaboratively train a model without aggregating the training data. Although the training data are kept within each participant and the local gradients can be securely synthesized, recent studies have shown that such privacy protection is insufficient. The global model parameters that have to be shared for optimization are susceptible to leak information about training data. In this work, we propose Confined Gradient Descent (CGD) that enhances privacy of federated learning by eliminating the sharing of global model parameters. CGD exploits the fact that a gradient descent optimization can start with a set of discrete points and converges to another set at the neighborhood of the global minimum of the objective function. It lets the participants independently train on their local data, and securely share the sum of local gradients to benefit each other. We formally demonstrate CGD's privacy enhancement over traditional FL. We prove that less information is exposed in CGD compared to that of traditional FL. CGD also guarantees desired model accuracy. We theoretically establish a convergence rate for CGD. We prove that the loss of the proprietary models learned for each participant against a model learned by aggregated training data is bounded. Extensive experimental results on two real-world datasets demonstrate the performance of CGD is comparable with the centralized learning, with marginal differences on validation loss (mostly within 0.05) and accuracy (mostly within 1%).

==> chapters/abstract.tex <==
\begin{abstract}
The performance of machine learning largely relies on the availability of large and  representative datasets, which may contain sensitive information. 
In this work, we propose \codename (\short) to address the privacy concerns arising from the federated learning.
It is different from the existing federated learning frameworks where participants jointly learn/share one and the same global model. 
In \short, each participant  learns a different  global model  and these global models are also kept private, and confined  within the corresponding participants. 
We theoretically guarantees the convergence of \short optimization, i.e., each confined global model will converge to a different neighborhood of the optimal solution of centralized training. 
The maximum difference between the loss of \short solution and the centralized solution is bounded, and such bound can be further adjusted to a preferably small range by tuning hyper parameters during \short optimization. 
In addition, we formally prove that it guarantees privacy preservation in a honest-but-curious adversarial setting.
Extensive experimental results on two real-world datasets  demonstrate that \short can closely approach the performance of centralized learning (where all the data are collected centrally), and significantly outperform the local training (trained only with a single participant's data). 
\end{abstract}

==> chapters/abstract1.tex <==
\begin{abstract}

Despite designed to facilitate collaborative training without aggregating raw data, 
federated learning is still found insufficient for strong privacy guarantees by recent studies.
\baigd{One sentence to reveal the root cause of this insufficiency, which also points out the main threat model of \short, like (I may be wrong): the intermediate model parameters that have to be shared during the gradient decent based optimization are susceptible to XXX(reversion attack?) }
\baigd{Basically, the weakness of "It is different from the existing federated learning frameworks where participants jointly learn/share one and the same global model." should be said here}
In this work, we propose \codename (\short) that boosts the privacy preservation of federated learning by eliminating the synchronization of intermediate model parameters.
Each participant asynchronously and independently trains a \highlight{global model} \baigd{I don't feel it is a proper term}, and the training is strictly confined locally.
\baigd{need to give insight how these global models are joined into the final global model}
The design of \short guarantees each \highlight{global model} converge to a different neighborhood of the optimal of its centralized counterpart.
The maximum difference between their loss is also bounded, and such bound can be further adjusted to a preferably small range by tuning hyper parameters.
We formally prove that \short guarantees \highlight{privacy preservation} \baigd{better to be specific: what privacy standard} against an honest-but-curious adversarial.
Extensive experimental results on two real-world datasets demonstrate the accuracy performance of \short is comparable with the centralized learning.


The performance of machine learning largely relies on the availability of large and  representative datasets, which may contain sensitive information.
In this work, we propose \codename (\short) to address the privacy concerns arising from the federated learning.
It is different from the existing federated learning frameworks where participants jointly learn/share one and the same global model.
In \short, each participant  learns a different  global model  and these global models are also kept private, and confined  within the corresponding participants. \baigd{need to give insight how these global models are joined into the final global model}
We theoretically guarantees the convergence of \short optimization, i.e., each confined global model will converge to a different neighborhood of the optimal solution of centralized training.
The maximum difference between the loss of \short solution and the centralized solution is bounded, and such bound can be further adjusted to a preferably small range by tuning hyper parameters during \short optimization.
In addition, we formally prove that it guarantees privacy preservation in a honest-but-curious adversarial setting.
Extensive experimental results on two real-world datasets  demonstrate that \short can closely approach the performance of centralized learning (where all the data are collected centrally), \highlight{and significantly outperform the local training (trained only with a single participant's data).} \baigd{this is trivial, no need to mention in abstract}
\end{abstract}


==> chapters/abstract2.tex <==
\begin{abstract}

Despite designed to facilitate collaborative training without aggregating raw data,
federated learning is still found insufficient for strong privacy guarantees by recent studies.
The intermediate global model parameters that have to be shared during the gradient decent based optimization are susceptible to attacks such as model inversion and membership inference.
In this work, we propose \codename (\short) that boosts the privacy preservation of federated learning by eliminating the sharing of global model parameters.
\short exploits the fact that a gradient descent optimization can start with a colony of discrete points %\highlight{models} \baigd{points? to be balanced with minimum point} 
and converges to another colony at the neighborhood of the minimum point of the objective function.
It lets participants independently train on their local data, and securely share the sum of local gradients to benefit each other. %\add{to benefit each other}.
We formally prove that the loss of each global models against the centralized model is bounded. %\highlight{central model} \baigd{hasn't been defined. ``optimal model''} is bounded, \highlight{and the bound can be adjusted by tuning hyper parameters.} \baigd{If we don't bring out the trade-off, it is not worth mentioning it this here.} %to offer the privacy-utility trade-off.
%We formally prove that \short guarantees \highlight{privacy preservation} \baigd{better to be specific: what privacy standard} against an honest-but-curious adversarial.
Extensive experimental results on two real-world datasets demonstrate the accuracy performance of \short is comparable with the centralized learning.
\end{abstract}


==> chapters/abstract3.tex <==
\begin{abstract}

Despite it being designed to facilitate collaborative training without aggregating raw data,
recent studies have shown that federated learning is still insufficient for strong privacy guarantees.
The intermediate global model parameters shared during the gradient decent based optimization are susceptible to attacks such as model inversion and membership inference.
In this work, we propose \codename (\short), an approach that boosts the privacy of federated learning by eliminating the sharing of global model parameters.
\short exploits the fact that a gradient descent optimization can start with a colony of discrete points 
and converges to another colony at the neighborhood of the minimum point of the objective function.
It allows the participants independently train on their local data, and securely share the sum of local gradients to benefit each other. 
We formally prove that the loss of %\replace{each global models}{the proprietary models learned for each participant} 
the proprietary models learned for each participant against the centralized model is bounded. %\highlight{central model} \baigd{hasn't been defined. ``optimal model''} is bounded, \highlight{and the bound can be adjusted by tuning hyper parameters.} \baigd{If we don't bring out the trade-off, it is not worth mentioning it this here.} %to offer the privacy-utility trade-off.
%We formally prove that \short guarantees \highlight{privacy preservation} \baigd{better to be specific: what privacy standard} against an honest-but-curious adversarial.
Extensive experimental results on two real-world datasets demonstrate the % \remove{accuracy} 
performance of \short is comparable with the centralized learning, %\add{with a marginal difference on loss~(up to XXX) and accuracy~(up to 1.43\%)}.
with marginal differences on validation loss~(within  0.128) and  accuracy~(within 3.8\%), and outperforms state-of-art federated learning with differential privacy.
\end{abstract}



==> chapters/abstract4.tex <==
\begin{abstract}

%\replace{Despite designed to facilitate collaborative training without aggregating raw data,
%recent studies have shown that federated learning is still insufficient for strong privacy guarantees.}
%{Despite federated learning facilitates collaborative training without aggregating raw data,
%recent studies have shown that its privacy protection is insufficient.}
Despite federated learning facilitates collaborative training without aggregating raw data,
recent studies have shown that its privacy protection is insufficient.
Although the local gradients of its participants can be securely synthesized, the global model parameters that have to be shared for optimization are susceptible to attacks such as model inversion and membership inference.
In this work, we propose \codename (\short) that boosts the privacy preservation of federated learning by eliminating the sharing of global model parameters.
\short exploits the fact that a gradient descent optimization can start with a colony of discrete points
and converges to another colony at the neighborhood of the %\replace{minimum point}{global minimum}
global minimum of the objective function.
It lets the participants independently train on their local data, and securely share the sum of local gradients to benefit each other.
We formally prove that the loss of %\replace{each global models}{the proprietary models learned for each participant}
the proprietary models learned for each participant against the centralized model is bounded. %\highlight{central model} \baigd{hasn't been defined. ``optimal model''} is bounded, \highlight{and the bound can be adjusted by tuning hyper parameters.} \baigd{If we don't bring out the trade-off, it is not worth mentioning it this here.} %to offer the privacy-utility trade-off.
%We formally prove that \short guarantees \highlight{privacy preservation} \baigd{better to be specific: what privacy standard} against an honest-but-curious adversarial.
Extensive experimental results on two real-world datasets demonstrate the % \remove{accuracy}
performance of \short is comparable with the centralized learning, %\add{with a marginal difference on loss~(up to XXX) and accuracy~(up to 1.43\%)}.
with marginal differences on validation loss~(mostly within  0.05) and  accuracy~(mostly within  1\%). %\highlight{, and outperforms state-of-art federated learning with differential privacy.} \baigd{1. This sentence is incorrect, because the sentence before ``and'' has a subject of ``the performance of \short''. 2. state-of-the-art. 3. I am a bit reluctant to talk about the comparison here, as we don't have a thorough comparison, e.g, convergence rate etc.}
\end{abstract}





==> chapters/background.tex <==
\section{Background and Related Works}
\label{sec:related}
In this section, we review the existing applicable techniques for gradient updates in the federated learning setting.

\subsection{Stochastic gradient descent}
Stochastic gradient descent~(SGD)~\cite{robbins1951stochastic, bottou2018optimization}, in the context of minimizing a cost function $F$ and with parameters $w$, is defined by
\begin{equation}
	\label{equ:sgd}
	w_{k+1} \leftarrow w_k - \alpha_k \frac{1}{|\xi_{k}|} \nabla F(w_k, \xi_{k})
\end{equation}
where $w_k$ are the parameters after iteration $k$, $\xi_{k} \in \xi$ is a randomly selected subset of the training samples at $k^{th}$ iteration, and $\alpha_k$ is the learning rate. Equation \ref{equ:sgd} can generalize to mini-batch update when $1 < |\xi_{k}| < |\xi|$; and to batch update when $\xi_{k} = \xi$.

In the federated learning setting, each local participant $l \in \mathcal{L}$ holds a subset of the training samples $\xi_l$. To run SGD (or mini-batch update), for each iteration, a random subset $\xi_{l,k} \subseteq \xi_l$ %\baigd{$\subseteq$?} 
from a random participant $l$ is selected. The participant $l$ then computes the gradient with respect to $\xi_{l,k}$, which can be written as $\nabla F(w_k, \xi_{l,k})$, and shares the gradient with other participants (or a parameter server). All the participants (or the server) can thus take a gradient descent step by 
\begin{equation}
	\label{equ:fdsgd}
	w_{k+1} \leftarrow w_k - \alpha_k \frac{1}{|\xi_{l,k}|} \nabla F(w_k, \xi_{l,k}).
\end{equation}

However, the gradients, i.e., $\nabla F(w_k, \xi_{l,k})$, shared in plain text are subject to information leakage of the local training data. For example, model-inversion attacks~\cite{melis2019exploiting, fredrikson2015model, shokri2017membership} are able to restore training data from the parameters.

In the immediately following sections, we summarize the existing privacy-preserving methods for synthesizing the local gradients, which fall into two broad categories.
We refer to them as \emph{secure aggregation} and \emph{learning with differential privacy}.

\subsection{Secure aggregation}
\label{sec:HE/MPC}
Secure aggregation typically employ cryptographic mechanisms such as homomorphic encryption (HE)~\cite{chen2018privacy, marc2019privacy, sharma2019confidential} and/or secure multiparty computation (MPC)~\cite{ gascon2017privacy, gascon2016secure, liu2017oblivious, mohassel2017secureml, bonawitz2017practical, zhang2020privcoll} to securely evaluate the gradient $\nabla F(w_k, \xi_{l,k})$ without revealing either local data or parameters.
With $\nabla F(w_k, \xi_{l,k})$, all the participants can thus take a gradient descent step by Equation~\ref{equ:fdsgd}.
%Recently, several works propose variant models of HE/MPC and applied them to deep neural networks.
%A recent study propose a MPC-friendly alternative function which was specifically designed to replace non-linear functions (such as sigmoid and softmax) since division and exponentiation are expensive to compute on shared values.

For instances, Bonawitz et. al.~\cite{bonawitz2017practical} presents a secure aggregation protocol that allows a server to compute the sum of  user-held data vectors, which can be used to aggregate user-provided model updates for a deep neural network;
Mohassel et. al.~\cite{mohassel2017secureml} propose a secure two-party computation (2PC) protocol that supports secure arithmetic operations on shared decimal numbers for calculating the gradient updates using SGD.
%Aside from, earlier attempts also include, such as the approach proposed in ~\cite{liu2017oblivious} for transforming an existing neural network to an oblivious neural network supporting privacy-preserving predictions.

However, existing FL frameworks employing HE/MPC are based on federated SGD, where all the participants share and update one and the same global model, which is still subject to information leakage~\cite{nasr2019comprehensive}. 
%In addition, HE and MPC are known to be limited by the significant computational or communicational overheads, and thus may not scale well to large number of participants or large input size.

\subsection{Learning with differential privacy}
\label{sec:DP}
Another line of studies that approaches to privacy preserving machine learning is through differential privacy (DP) mechanism~\cite{zheng2019bdpl, hagestedt2019mbeacon, abadi2016deep, song2013stochastic, shokri2015privacy, dwork2014algorithmic, hu2019fdml, zhang2020differentially, geyer2017differentially}.
The common practice of achieving differential privacy is based on additive noise calibrated to $\nabla F$’s sensitivity $\mathcal{S}^2_{\nabla F}$. %, which is defined as the maximum of the absolute distance $|F(d)-F(d^\prime)|$ where $d$ and $d^\prime$ are adjacent inputs.
As such, one can achieve a differentially private learning framework by updating parameters with perturbed gradients at each iteration, for example, to update parameters as
\begin{equation}
	\label{equ:dp}
w_{k+1} \leftarrow w_k - \alpha_k \frac{1}{|\xi_{l,k}|} (\nabla F(w_k, \xi_{l,k})+ \mathcal{N}(0, \mathcal{S}^2_{\nabla F} \cdot \sigma^2))
\end{equation}
where $\mathcal{N}(0, \mathcal{S}^2_{\nabla F} \cdot \sigma^2)$ is the Gaussian distribution (a commonly used noise distribution in differentially private learning frameworks~\cite{dwork2014algorithmic}) with mean $0$ and standard deviation $\mathcal{S}_{\nabla F} \cdot \sigma$.

However, there is an inherent tradeoff between privacy and utility of the trained model. In addition, the privacy loss is accumulated (i.e., additional information about the sensitive data is released) with repeated access to the data during training epochs~\cite{abadi2016deep}.

In a summary, in all these approaches, the global model has to be shared with each participant, leading to the leakage of information and potential attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}.



==> chapters/case.tex <==
\section{Case study: \codename for a N-layer neural network}
	\label{sec:cgdnn}

In this section, we apply \short to a N-layer neural network (Algorithm \ref{alg:cgdnn}). 
We assume a centralized dataset $\xi$ is partitioned and distributed to $m$ participants where $m = (m^h \times m^v)$, i.e., number of horizontal partitions $\times$ number of vertical partitions.  
Each participant owns a private part of training dataset $\xi_{l_{(i,j)}}$ ($i \in m^h$, $j \in m^v$) as well as its respective confined global model parameters $w_k^{(1)l_{(i,j)}}$,...,$w_k^{(N)l_{(i,j)}}$. Since each participant owns different data and model, the training prediction $\widehat{y}^{(1)l_{(i,j)}}$  is also different and kept confined in its corresponding participant (shown in Figure \ref{fig:cgdnn}). 
%Algorithm \ref{alg:cgdnn} details the process of training. 

Each participant first randomly initialize its own confined model $w_1^{(1)l_{(i,j)}}$,...,$w_1^{(N)l_{(i,j)}}$ (line 3) (line number in Algorithm \ref{alg:cgdnn}). The size of the first layer model is $w^{(1)l_{(i,j)}} \in \mathbb{R}^{d_{l_j}\times H_1}$, where $d_{l_j}$ is the number of features in $\xi_{l_{(i,j)}}$, and the size of follow-up layers' models is $w^{(r)l_{(i,j)}} \in \mathbb{R}^{H_{r-1}\times H_r}$ ($r \in [2,N]$). 
We note that different participant may have different size of the first layer model $w^{(1)l_{(i,j)}}$ with respect to $d_{l_j}$, while the other follow-up layers' models $w^{(r)l_{(i,j)}}$ ($r \in [2,N]$) are kept same size in each participant.

In the following, we detail the process of training in each training iteration.

In the forward propagation, each participant computes $z_k^{(1)l_{(i,j)}} = \xi_{l_{(i,j)}} w_k^{(1)l_{(i,j)}}$ respectively (line 7). 
Then, the participants in each group $l_i = \{l_{(i,1)},...,l_{(i,m^v)}\}$ securely compute the sum on their $z_k^{(1)l_{(i,j)}}$ (via secret-sharing scheme) and produce the input to the first hidden layer $z_k^{(1)l_i} = \sum _{j=1}^{m^v} z_k^{(1)l_{(i,j)}}$ ($i \in m^h$) with respect to each horizontal partition (line 9 to 10). This step leverages the information from the vertical partitions within the group $l_i$ while preserves privacy for distributed features~\cite{zhang2020privcoll}.
Then each participant separately computes the output of each layer $a_k^{(1)l_{(i,j)}},...,a_k^{(N)l_{(i,j)}} $ based on its own confined models (line 12 to 18). 

In the backward propagation, each participant respectively computes the local gradient of each layer $g_k^{(N)l_{(i,j)}},...g_k^{(1)l_{(i,j)}}$ which is computed from its own private dataset and confined model (line 20 to 30). Then, they securely evaluate the sum of local gradients from the $N^{th}$ layer to the $2^{nd}$ layer (line 31 to 34). For the first layer gradient, since the size of $w^{(1)l_{(i,j)}}$ may be different with respect to $d_{l_j}$,  the sum of the local gradients $g_k^{(1)l_j}$ is therefore taken among the vertically partitioned participant groups $l_j = \{l_{(1,j)},...,l_{(m^h,j)}\}$ (line 36 to 38). 

In the descent, after choosing a learning rate $\alpha_k$ (line 40), the first layer model is updated by taking a descent step of $\alpha_k g_k^{(1)l_j}$ (line 41 to 44), and the rest of layer's models are updated by taking a descent step of $\alpha_k g_k^{(r)} $ ($r \in [2,N]$) (line 45 to 48). 

\begin{figure}[!t]
	\centering
	\includegraphics[width=2.5in]{fig/case.pdf}
	\caption{Confined data and model of a N-layer neural network in participant $l_{(i,j)}$ ($i \in m^h$, $j \in m^v$).}
	\label{fig:cgdnn}
\end{figure}

\begin{algorithm}[h]
	\caption{\codename of a N-layer fully-connected neural network for $m = (m^h \times m^v)$ participants}
	\label{alg:cgdnn}
	\begin{algorithmic}[1]
		\State{\textbf{Input:} Local training data $\xi_{l_{(i,j)}}$ ($i \in m^h$, $j \in m^v$), activation functions of $N$ layers: $\sigma^{(1)}...\sigma^{(N)}$, cost function $J$, the number of  training iterations $T$}
		\State{\textbf{Output:} Confined global model parameters of $N$ layers: $w_*^{(1)l_{(i,j)}}$,...,$w_*^{(N)l_{(i,j)}}$ ($i \in m^h$, $j \in m^v$) }
		\State{\textbf{Initialize:} $k\leftarrow 1$, each participant $l_{(i,j)}$ randomizes its own $w_1^{(1)l_{(i,j)}}$,...,$w_1^{(N)l_{(i,j)}}$}
		\While{$k \leq T$}
		\State{\textbf{Forward propagation} }
		\State{\quad\textbf{for all} participants $l_{(i,j)}$ \textbf{do in parallel}}
		\State{\qquad  $z_k^{(1)l_{(i,j)}} \leftarrow \xi_{l_{(i,j)}} w_k^{(1)l_{(i,j)}}$ }
		\State{\quad\textbf{end for}}
		\State{\quad\textbf{for all} groups $l_i = \{l_{(i,1)},...,l_{(i,m^v)}\}$ \textbf{do in parallel}}
		\State{\qquad  Securely evaluate the sum: $z_k^{(1)l_i} \leftarrow \sum _{j=1}^{m^v} z_k^{(1)l_{(i,j)}}$ }
		\State{\quad\textbf{end for}}
		\State\quad{\textbf{for all} participants $l_{(i,j)}$ \textbf{do in parallel}}
		\State{\qquad  $a_k^{(1)l_{(i,j)}} \leftarrow \sigma^{(1)}(z_k^{(1)l_i}) $ }
		\State{\qquad  $z_k^{(2)l_{(i,j)}} = a_k^{(1)l_{(i,j)}} w_k^{(2)l_{(i,j)}}$, $a_k^{(2)l_{(i,j)}} = \sigma^{(2)}( z_k^{(2)l_{(i,j)}})$ }
		%\State{\qquad  $a_k^{(2)l_{(i,j)}} \leftarrow \sigma^{(2)}( z_k^{(2)l_{(i,j)}}) $ }
		\State{\qquad  \qquad\qquad\qquad...... }
		\State{\qquad  $a_k^{(N)l_{(i,j)}} = \sigma^{(N)}( z_k^{(N)l_{(i,j)}})) $ }
		\State{\qquad  $\widehat{y}^{l_{(i,j)}} \leftarrow a_k^{(N)l_{(i,j)}} $ }			
		\State{\quad\textbf{end for}}
		\State{(to be continued in the next page)}
		\algstore{myalg}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\ContinuedFloat
	\caption{\codename of a N-layer neural network for $m = (m^h \times m^v)$ participants (continued)}
	\begin{algorithmic}
		\algrestore{myalg}
		\State{\textbf{Backward propagation} }
		\State\quad{\textbf{for all} participants $l_{(i,j)}$ \textbf{do in parallel}}
		\State{\qquad Compute the local gradient of the $N^{th}$ layer: \\\qquad\qquad\qquad $\delta_k^{(N)l_{(i,j)}} \leftarrow  \frac{\partial J(\widehat{y}^{l_{(i,j)}} , y^{l_{(i,j)}}) }{\partial a_k^{(N)l_{(i,j)}}} \frac{\partial a_k^{(N)l_{(i,j)}}}{\partial z_k^{(N)l_{(i,j)}}}$ \\\qquad\qquad\qquad $g_k^{(N)l_{(i,j)}} \leftarrow \delta_k^{(N)l_{(i,j)}} \frac{\partial  z_k^{(N)l_{(i,j)}}}{\partial w_k^{(N)l_{(i,j)}}}$ }
		%\State{\qquad Securely evaluate the sum of local gradients:  \\\qquad\qquad\qquad $g_k^{(N)} \leftarrow \sum_{i,j=1}^{m^h,m^v}g_k^{(N)l_{(i,j)}}$ }
		\State{\qquad Compute the local gradient of the $(N-1)^{th}$ layer:  \\\qquad\qquad\qquad $\delta_k^{(N-1)l_{(i,j)}} \leftarrow  \delta_k^{(N)l_{(i,j)}} \frac{\partial z_k^{(N)l_{(i,j)}}}{\partial a_k^{(N-1)l_{(i,j)}}} \frac{\partial a_k^{(N-1)l_{(i,j)}}}{\partial  z_k^{(N-1)l_{(i,j)}}}$ \\\qquad\qquad\qquad $g_k^{(N-1)l_{(i,j)}} \leftarrow \delta_k^{(N-1)l_{(i,j)}}  \frac{\partial  z_k^{(N-1)l_{(i,j)}}}{\partial w_k^{(N-1)l_{(i,j)}}}$ }
		\State{\qquad  \qquad\qquad\qquad...... }
		\State{\qquad Compute the local gradient of the $1^{st}$ layer:  \\\qquad\qquad\qquad $\delta_k^{(1)l_{(i,j)}} \leftarrow  \delta_k^{(2)l_{(i,j)}} \frac{\partial z_k^{(2)l_{(i,j)}}}{\partial a_k^{(1)l_{(i,j)}}} \frac{\partial a_k^{(1)l_{(i,j)}}}{\partial  z_k^{(1)l_{(i,j)}}}$ \\\qquad\qquad\qquad $g_k^{(1)l_{(i,j)}} \leftarrow \delta_k^{(1)l_{(i,j)}}  \frac{\partial  z_k^{(1)l_{(i,j)}}}{\partial w_k^{(1)l_{(i,j)}}}$ }
		\State{\qquad Securely evaluate the sum of local gradients:  \\\qquad\qquad\qquad $g_k^{(N)} \leftarrow \sum_{i,j=1}^{m^h,m^v}g_k^{(N)l_{(i,j)}}$ \\\qquad\qquad\qquad ...... \\\qquad\qquad\qquad $g_k^{(2)} \leftarrow \sum_{i,j=1}^{m^h,m^v}g_k^{(2)l_{(i,j)}}$ }
		%\State{\qquad  \qquad\qquad\qquad...... }
		\State{\quad\textbf{end for}}
		\State{\quad\textbf{for all} groups $l_j = \{l_{(1,j)},...,l_{(m^h,j)}\}$ \textbf{do in parallel}}
		\State{\qquad  Securely evaluate the sum: $g_k^{(1)l_j} \leftarrow \sum_{i=1}^{m^h}g_k^{(1)l_{(i,j)}}$ }
		\State{\quad\textbf{end for}}
		\State{\textbf{Descent} }
		\State{\quad Choose a stepsize: $\alpha_k$}
		\State{\quad\textbf{for all} groups $l_j = \{l_{(1,j)},...,l_{(m^h,j)}\}$ \textbf{do in parallel}}
		\State{\qquad Update the  $1^{st}$ layer's parameter as:\\\qquad\qquad\qquad $w_{k+1}^{(1)l_{(i,j)}} \leftarrow w_{k}^{(1)l_{(i,j)}} - \alpha_k g_k^{(1)l_j} $}
		\State{\quad\textbf{end for}}
		\State{\quad\textbf{for all} participants $l_{(i,j)}$ \textbf{do in parallel}}
		\State{\qquad Update the  rest of the layers' parameter as:\\\qquad\qquad\qquad $w_{k+1}^{(r)l_{(i,j)}} \leftarrow w_{k}^{(r)l_{(i,j)}} - \alpha_k g_k^{(r)} $, ($r \in [2,N]$)}
		\State{\quad\textbf{end for}}
		\State{$k \leftarrow k+1 $}		
		\EndWhile
	\end{algorithmic}
\end{algorithm}

==> chapters/convergence.tex <==
\section{Convergence Analysis}
\label{sec:convergence}
In this section, we theoretically demonstrate the bound of difference between any of $w_*^l$ learned by \short and the centralized optimal solution $w_*$. 
Inspired by~\cite{hu2019fdml, hsieh2017gaia, ho2013more}, we analyze the convergence property of \short by evaluating a \emph{regret} function $\mathcal{R}$, which is the difference between the loss of \short solution confined in any participant $l$ and the loss of the centralized optimal solution, defined as
\begin{equation}
	\label{equ:regret}
\mathcal{R} = \frac{1}{T} \sum_{k=1}^{T} (F(w_k^l) - F(w_*))
\end{equation}

%We prove that $\mathcal{R}$ is bounded by $\displaystyle \epsilon = m \|\mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$. 


\subsection{Assumptions}
Our approach for establishing convergence analysis for \short is built upon the following common assumptions on the loss function. (These assumptions are essential for convergence analyses of most gradient-based methods~\cite{bottou2018optimization}).

\begin{assumption}
	\label{assum:Lip}
(Lipschitz-continuous objective gradients). 
The loss function $F$: $\mathbb{R}^d \rightarrow \mathbb{R}$ is continuously differentiable and the gradient function of $F$, namely, $\nabla F$: $\mathbb{R}^d \rightarrow \mathbb{R}^d$, is Lipschitz continuous with Lipschitz constant $L > 0$, i.e.,
\begin{equation}
\|\nabla F(w) - \nabla F(\widehat{w})\|_2 \leq L\|w-\widehat{w}\|_2 \text{\quad for all } \{w,\widehat{w}\} \subset \mathbb{R}^d.
\end{equation}
\end{assumption}
%Any differentiable function whose gradient is Lipschitz continuous is a continuously differentiable function. 
Intuitively, this assumption ensures that the gradient of the loss function $F$ does not change arbitrarily quickly with respect to $w$, such that the gradient can be a useful indicator for decreasing $F$~\cite{bottou2018optimization}. %Such an assumption is essential for convergence analyses of most gradient-based methods; 
%Without it, the gradient would not provide a good indicator for how far to move to decrease F 

\begin{assumption}
	\label{assum:convex}
	(Strong convexity). 
	The loss function $F$: $\mathbb{R}^d \rightarrow \mathbb{R}$ is strongly convex such that 
	\begin{equation}
		F(\widehat{w}) \geq F(w) + \nabla F(w)^T(\widehat{w}-w)  \text{\quad for all } \{w,\widehat{w}\} \subset \mathbb{R}^d.
	\end{equation}
\end{assumption}

A useful fact from Assumption \ref{assum:convex} for our analysis is
\begin{equation}
	\label{equ:convex}
(F(w)-F(w_*)) \leq \langle w-w_*, \nabla F(w) \rangle  \text{\quad for all } w \subset \mathbb{R}^d,
\end{equation}
where $\langle\cdot{,}\cdot\rangle$ denotes inner product operation.

In addition, we adopt the same assumption on a bounded solution space used in related studies~\cite{bottou2018optimization, hu2019fdml}.
\begin{assumption}
	\label{assum:sol}
(Bounded solution space). The sequence of $\{w_k^l\}|_{k \in [1,T]}$ is contained in an open set over which $F$ is bounded below a scalar $F_{inf}$, such that
\begin{enumerate}[label=(\alph*)]
\item  There exists a $D>0$, s.t.,	$\|w_k^l-w_*\|_2^2 \leq D^2$ for all $k$ ~\label{assum:sola}
\item There exists a $G>0$, s.t., $\|g^l(w_k^l, \xi_l)\|_2^2 \leq G^2$ for all $w_k^l \subset \mathbb{R}^d$ ~\label{assum:solb}
\end{enumerate}
\end{assumption}

\subsection{Main Theorem} 

The following theorem demonstrates our main result on the converge rate of \short.
\begin{theorem}
	\label{theorem:main}
With Assumptions \ref{assum:Lip} - \ref{assum:sol}, and a learning rate of $\alpha_k = \frac{\alpha}{(k+\mu T)^2}$ ($0<\mu <1$), the regret $\mathcal{R}$ given by Algorithm \ref{alg:cgd} for \short optimization is
\begin{equation}
	\mathcal{R} = 
\begin{cases}
	O(\epsilon + \frac{1}{\mu T +1}), & \text{if } \mu \rightarrow 0 \vspace{0.3cm}\\ 
	O(\epsilon + \frac{\ln |\mu T +1|}{T}), & \text{if } \mu \rightarrow 1,
\end{cases}	
\end{equation}
where $\epsilon = m \| \displaystyle \mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$. %$ \|\sum_{j=1}^{m}(w_1^l-w_1^j)\| $.
%\yanjun{$m^h$?}
\end{theorem}
The theorem shows that, 
\begin{itemize}
	\item \textbf{Convergence rate.} $\mathcal{R}$ decreases as $\frac{1}{\mu T +1}$ or $\frac{\ln |\mu T +1|}{T}$ decreasing to $0$ with regard to $T$, meaning that the solution of \short will converge toward the optimal value. In addition, the convergence rate can be adjusted by the parameter $\mu$. (The choice of $\mu$ in practice will be discussed in Section \ref{sec:mu});
	\item \textbf{Bounded difference. } The maximum difference between  \short solution and the centralized optimal solution is bounded by $\epsilon$. 
	Here, we introduce the initialization parameter $\delta$, which decides the range of $w_1^l$   as
	\begin{equation}
		\label{equ:delta}
		w_1^l = \delta\cdot \mathit{Rand(d_{w_1^l })}  \text{\quad for all } l \in m,
	\end{equation}
	where $\mathit{Rand}$ is the initialization scheme and $d_{w_1^l }$ is the shape of $w_1^l$. 
	A default setting  is to apply  standard weight initialization scheme which returns random values sampling  from the Gaussian distribution of mean 0 and variance 1, with $\delta = 0.1$.
	%	(such as ``$\mathit{randn}$'' that returns random values sampling from the Gaussian distribution of mean 0 and variance 1), .	
	By tuning $\delta$, the gap between \short solution and the centralized optimal solution can be adjusted accordingly  (detailed in Section \ref{sec:init}) .
	
\end{itemize}
%Since every $w_1$ is initialized from the same distribution, we have $\displaystyle \|\mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$  exponentially small (theoretically reaches to $0$) with growth of $m$ . 
%(e.g., with randomization from uniform distribution, it decreases from $10^{-3}$ with $m = 10$ to $10^{-5}$ with $m = 100$).
%\yanjun{introduce initialization parameter $\delta$}
%Intuitively, 



\subsection{Proof of Theorem \ref{theorem:main}}
We start with the following lemma that is soon used in our proof. 
\begin{lemma}
	\label{lemma:inner}
	Let $S_{k+1} = \frac{1}{2} \|w_{k+1}^l - w_*\|_2^2$, and $S_{k} = \frac{1}{2} \|w_{k}^l - w_*\|_2^2$.  Let $\nabla F(\cdot) = \frac{1}{n} \sum_{i=1}^{n}  \nabla F(\cdot, \xi_{i})$.  %Because in Equation \ref{equ:regret}, the w_* is computed using \xi. Therefore, \nabla F(\cdot) should denote the gradient taken by batch update on $F$ with respect to $\xi$ as well, otherwise, we cannot derive inequality by Equation \ref{equ:convex}. 
	We have
	\begin{multline*}
		\langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle = 
		\frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 %first term
		- \frac{1}{\alpha_k} (S_{k+1}-S_k)\\ %second term
		- \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle. %third term
	\end{multline*}
\end{lemma}
%We give the proof in Appendix \ref{apx:lemma}.
\begin{proof}
	\begin{equation}
		\label{equ:lemma}
		\begin{aligned}
			& S_{k+1} - S_k = \frac{1}{2} \bigg( \|w_{k+1}^l - w_*\|_2^2 -  \|w_{k}^l - w_*\|_2^2 \bigg) \\
			&= \frac{1}{2} \bigg( \|w_k^l - \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)  - w_*\|_2^2 - \|w_{k}^l - w_*\|_2^2 \bigg) \\
			&= \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 - \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\rangle\\
			&= \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 \\
			& \qquad - \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) + \nabla F(w_k^l) - \nabla F(w_k^l) \rangle\\
			& = \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 -  \alpha_k \langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle\\
			& \qquad  \qquad \qquad- \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l) \rangle 
		\end{aligned}
	\end{equation}
	Dividing the above equation by $\alpha_k$, we can get the lemma. 
\end{proof}

In the following, we give the proof of Theorem \ref{theorem:main}.
\begin{proof}
	By the definition in Equation \ref{equ:regret}, we have
	\begin{equation}
		\label{equ:conv}
		\mathcal{R} = \frac{1}{T} \sum_{k=1}^{T} (F(w_k^l) - F(w_*)) \leq \frac{1}{T} \sum_{k=1}^{T} \langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle
	\end{equation}
	where Inequation \ref{equ:conv} is from Assumption \ref{assum:convex}, i.e., the convexity of the loss function.
	Inserting the result from Lemma \ref{lemma:inner} to Inequation \ref{equ:conv} and multiplying by $T$, we obtain
	\begin{equation}
		\label{equ:threeterms}
		\begin{aligned}
			T \cdot R & \leq  \sum_{k=1}^{T} \bigg( 	\frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 \\
			& \quad - \frac{1}{\alpha_k} (S_{k+1}-S_k)- \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \bigg) \\
			& \leq \sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 - \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k)\\
			&  \quad - \sum_{k=1}^{T}  \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle
		\end{aligned}
	\end{equation}
	We bound the three terms of Inequation \ref{equ:threeterms} in the following.
	
	For the first term, we have 
	\begin{align}
		\sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 & \leq \sum_{k=1}^{T} \frac{1}{2} \frac{\alpha}{(k+\mu T)^2} m^2 G^2 ~\label{equ:firstbound}\\
		&=\frac{\alpha m^2 G^2}{2} \sum_{k=1}^{T} \frac{1}{(k+\mu T)^2} < \alpha m^2 G^2 ~\label{equ:basel}
	\end{align}
	Inequation \ref{equ:firstbound} is from  Assumption \ref{assum:sol}\ref{assum:solb}, and Inequation \ref{equ:basel} is from the fact $\sum_{x=1}^{\infty} \frac{1}{x^2} \rightarrow 2$.
	
	For the second term, we have
	\begin{align}
		- \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k) & = \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_k-S_{k+1}) \\
		&= \sum_{k=1}^{T} \frac{1}{\alpha_k} \bigg( \frac{1}{2} \|w_{k}^l - w_*\|_2^2 - \frac{1}{2} \|w_{k+1}^l - w_*\|_2^2 \bigg)\\
		& \leq \sum_{k=1}^{T} \frac{1}{2\alpha_k}  \|(w_{k}^l - w_*)- (w_{k+1}^l - w_*)\|_2^2 ~\label{equ:reversetria}\\
		& = \sum_{k=1}^{T} \frac{1}{2\alpha_k} \|w_{k}^l - w_{k+1}^l \|_2^2 \\
		&=  \sum_{k=1}^{T} \frac{1}{2\alpha_k}  \|\alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2\\
		& = \sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 < \alpha m^2 G^2 ~\label{equ:second}
	\end{align}
	Inequation \ref{equ:reversetria} comes from reverse triangle inequality, and Inequation \ref{equ:second} is from the result of the first term. 
	
	
	For the third term, we have
	\mathleft
	\[- \sum_{k=1}^{T}\langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \]
	\mathcenter
	\begin{align}
		&=\langle w_{k}^l - w_*, \sum_{k=1}^{T} \big(\nabla F(w_k^l) - \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\big)\rangle \\
		&\leq \|w_{k}^l - w_*\|\cdot\|\sum_{k=1}^{T} \big(\nabla F(w_k^l) - \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\big)\| ~\label{equ:tria}\\
		&\leq \|w_{k}^l - w_*\|\cdot L \| \sum_{k=1}^{T} \sum_{j=1}^{m} (w_k^l -  w_k^j)\| ~\label{equ:lip}\\
		&\leq DL\|\sum_{j=1}^{m}(w_1^l-w_1^j) + ... +  \sum_{j=1}^{m}(w_T^l-w_T^j)\| ~\label{equ:assu3a}
	\end{align}
	\begin{equation}
		\begin{aligned}
			= DL \|&T\sum_{j=1}^{m}(w_1^l-w_1^j)  \\
			&-\sum_{k=1}^{T-1} \sum_{j=1}^{m} \alpha_{(T-k)} k \big(\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\big) \| ~\label{equ:rew}
		\end{aligned}
	\end{equation}
	\begin{equation}
		\begin{aligned}
			\leq  DL & \bigg(\|T\sum_{j=1}^{m}(w_1^l-w_1^j)\|  \\
			&+ \| \sum_{k=1}^{T-1} \sum_{j=1}^{m} \alpha_{(T-k)} k \big(\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\big) \| \bigg)~\label{equ:rewnorm}
		\end{aligned}
	\end{equation}
	\begin{align}
		&\leq  DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + DL\cdot2m^2G \sum_{k=1}^{T-1} \alpha_{(T-k)} k \quad \quad \quad \quad ~\label{equ:assu3b} \\
		& = DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL \sum_{k=1}^{T-1} \frac{k}{((1+\mu)T-k)^2}~\label{equ:insertalpha} \\
		& < DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{T}{\mu T +1} + \ln |\mu T +1|) ~\label{equ:integral}
	\end{align}
	
	Inequations \ref{equ:tria} and \ref{equ:rewnorm} are from triangle inequality. 
	Inequation \ref{equ:lip} is from the fact $\nabla F(w_k^l) = \frac{1}{n} \sum\limits_{i=1}^{n}  \nabla F(w_k^l, \xi_{i}) = \sum\limits_{j=1}^{m} g^j(w_k^l, \xi_j)$ and Assumption \ref{assum:Lip}'s blockwise Lipschitz-continuity. 
	Inequation \ref{equ:assu3a} is from Assumption \ref{assum:sol}\ref{assum:sola} and represents $\sum\limits_{k=1}^{T}(\cdot) $ by a summand sequence. 
	Equation \ref{equ:rew} comes from the fact
	\begin{multline*}
		w_k^l-w_k^j = (w_1^l - \alpha_1 \nabla F(w_1^l) - ... - \alpha_k \nabla F(w_k^l)) \\
		-(w_1^j - \alpha_1 \sum\limits_{j=1}^{m}g^j(w_1^j, \xi_j) - ... - \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j))\\
		= (w_1^l - w_1^j) - \alpha_1 (\nabla F(w_1^l) - \sum\limits_{j=1}^{m}g^j(w_1^j, \xi_j)) \\
		-...- \alpha_k(\nabla F(w_k^l) -  \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)).
	\end{multline*}
	Inequation \ref{equ:assu3b} is from Assumption \ref{assum:sol}\ref{assum:solb}, which gives $\|\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\| \leq 2mG$. 
	Equation \ref{equ:insertalpha} is obtained by inserting $\alpha_{(T-k)} = \frac{\alpha}{(T-k +\mu T)^2}$. 
	Inequation \ref{equ:integral} is from the following fact. Since
	\[\int_a^b \frac{k}{(c-k)^2}\, dk = \frac{b}{c-b} + \ln |c-b| - \frac{a}{c-a} - \ln |c-a|,\]
	we have
	\begin{align*}
		&\int_1^{T-1} \frac{k}{((1+\mu)T-k)^2}\, dk = \frac{T-1}{(1+\mu)T-(T-1)} \\
		&+ \ln |(1+\mu)T-(T-1)| - \frac{1}{(1+\mu)T-1} - \ln |(1+\mu)T-1|\\
		&<\frac{T-1}{(1+\mu)T-(T-1)}+ \ln |(1+\mu)T-(T-1)| \text{ \quad (with $T\geq2$). } \\
		&< \frac{T}{\mu T +1} + \ln |\mu T +1|
	\end{align*}	
	
	Combining Inequations \ref{equ:threeterms}, \ref{equ:basel}, \ref{equ:second} and \ref{equ:integral}, and dividing by T we obtain
	\begin{align*}
		\mathcal{R} &< \frac{2 \alpha m^2 G^2}{T} + DL \|\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{1}{\mu T +1} + \frac{\ln |\mu T +1|}{T}) \\
		& = 
		\begin{cases}
			O(\epsilon + \frac{1}{\mu T +1}), & \text{if } \mu \rightarrow 0 \vspace{0.3cm}\\ 
			O(\epsilon + \frac{\ln |\mu T +1|}{T}), & \text{if } \mu \rightarrow 1.
		\end{cases}	
	\end{align*}
\end{proof}


==> chapters/convergence1.tex <==
\section{Convergence Analysis}
\label{sec:convergence}

In this section, we conduct a formal convergence analysis on \short. 
Convergence analysis has been extensively used in the literature~\cite{hu2019fdml, hsieh2017gaia, ho2013more} to prove the correctness of optimization algorithms.
We demonstrate the bound of the distance between an arbitrary $w_*^l$ learned by \short and the centralized model $w_*$.
The analysis is centered around a \emph{regret} function $\mathcal{R}$, which is the difference between the \short's training loss %\highlight{confined in any participant $l$}\baigd{what does this mean?} 
and the loss of the centralized optimal solution, defined as
\begin{equation}
	\label{equ:regret}
\mathcal{R} = \frac{1}{T} \sum_{k=1}^{T} (F(w_k^l) - F(w_*))
\end{equation}

%We prove that $\mathcal{R}$ is bounded by $\displaystyle \epsilon = m \|\mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$.


\subsection{Assumptions}
We make the following three assumptions on the loss function $F$. 
They all are common assumptions in convergence analyses of most gradient-based methods, and satisfied in a variety of widely used cost functions, such as mean squared error (MSE), cross entropy, etc~\cite{bottou2018optimization}.
%\baigd{Also need a sentence to argue these assumptions will not introduce extra constraints to those loss functions used by existing learning algorithms. Give examples, citations to support}

\begin{assumption}
	\label{assum:Lip}
(Lipschitz continuity). %\baigd{objective gradients sounds weird}
The loss function $F$: $\mathbb{R}^d \rightarrow \mathbb{R}$ is continuously differentiable and the gradient function of $F$, namely, $\nabla F$: $\mathbb{R}^d \rightarrow \mathbb{R}^d$, is Lipschitz continuous with Lipschitz constant $L > 0$, i.e.,
\begin{equation}
\|\nabla F(w) - \nabla F(\widehat{w})\|_2 \leq L\|w-\widehat{w}\|_2 \text{\quad for all } \{w,\widehat{w}\} \subset \mathbb{R}^d.
\end{equation}
\end{assumption}
%Any differentiable function whose gradient is Lipschitz continuous is a continuously differentiable function.
Intuitively, this assumption ensures that the gradient of $F$ does not change arbitrarily %\replace{quickly with respect to $w$}{in the course of descending}
in the course of descending, such that the gradient can be a useful indicator %\replace{for decreasing $F$}{towards the optimal}
towards the optimal~\cite{bottou2018optimization}. %Such an assumption is essential for convergence analyses of most gradient-based methods;
%Without it, the gradient would not provide a good indicator for how far to move to decrease F

\begin{assumption}
	\label{assum:convex}
	(Strong convexity).
	The loss function $F$: $\mathbb{R}^d \rightarrow \mathbb{R}$ is strongly convex such that
	\begin{equation}
		F(\widehat{w}) \geq F(w) + \nabla F(w)^T(\widehat{w}-w)  \text{\quad for all } \{w,\widehat{w}\} \subset \mathbb{R}^d.
	\end{equation}
\end{assumption}

A useful fact from Assumption \ref{assum:convex} for our analysis is
\begin{equation}
	\label{equ:convex}
(F(w)-F(w_*)) \leq \langle w-w_*, \nabla F(w) \rangle  \text{\quad for all } w \subset \mathbb{R}^d,
\end{equation}
where $\langle\cdot{,}\cdot\rangle$ denotes the inner product operation.

In addition, we adopt the same assumption on a bounded solution space used in related studies~\cite{bottou2018optimization, hu2019fdml}.
\begin{assumption}
	\label{assum:sol}
(Bounded solution space). The set of $\{w_k^l\}|_{k \in [1,T]}$ %\baigd{this is a set. consider another way to denote sequence} 
is contained in an open set over which $F$ is bounded below a scalar $F_{inf}$, such that
\begin{enumerate}[label=(\alph*)]
\item  there exists a $D>0$, s.t.,	$\|w_k^l-w_*\|_2^2 \leq D^2$ for all $k$, and \label{assum:sola}
\item there exists a $G>0$, s.t., $\|g^l(w_k^l, \xi_l)\|_2^2 \leq G^2$ for all $w_k^l \subset \mathbb{R}^d$.  ~\label{assum:solb}
\end{enumerate}
\end{assumption}

\subsection{Main Theorem}

The following theorem demonstrates our main result on the converge rate of \short.
\begin{theorem}
	\label{theorem:main}
With Assumptions \ref{assum:Lip} - \ref{assum:sol}, and a learning rate of $\alpha_k = \frac{\alpha}{(k+\mu T)^2}$ ($0<\mu <1$), the regret $\mathcal{R}$ given by Algorithm \ref{alg:cgd} for \short optimization is
\begin{equation}
	\mathcal{R} =
\begin{cases}
	O(\epsilon + \frac{1}{\mu T +1}), & \text{if } \mu \rightarrow 0 \vspace{0.3cm}\\
	O(\epsilon + \frac{\ln |\mu T +1|}{T}), & \text{if } \mu \rightarrow 1,
\end{cases}	
\end{equation}
where $\epsilon = m \| \displaystyle \mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$. %$ \|\sum_{j=1}^{m}(w_1^l-w_1^j)\| $.
%\yanjun{$m^h$?}
\end{theorem}
The theorem implies the following two facts. 
\begin{itemize}
	\item \textbf{Convergence rate.} $\mathcal{R}$ decreases as $\frac{1}{\mu T +1}$ or $\frac{\ln |\mu T +1|}{T}$ decreasing to $0$ with regard to $T$, meaning that %\remove{the solution of} 
	\short will converge toward the optimum. %\remove{value}. 
	In addition, the convergence rate can be adjusted by the parameter $\mu$~(the choice of $\mu$ in practice will be discussed in Section \ref{sec:mu}). 
	\item \textbf{Bounded optimality gap. } %\replace{The maximum difference between short solution and the centralized optimal solution is bounded by $\epsilon$.}{When \short converges, the maximum difference the confined model and the central model is bounded by $\epsilon$.} \baigd{have a consideration on the terms. whether you want to look at it from a pure mathematical or FL perspective }
	When \short converges, the maximum gap between the confined model and the central model is bounded by $\epsilon$.
	Here, we introduce the initialization parameter $\delta$, which decides the range of $w_1^l$  in a way of
	\begin{equation}
		\label{equ:delta}
		w_1^l = \delta\cdot \mathit{Rand}  \text{\quad for all } l \in m,
	\end{equation}
	where $\mathit{Rand}$ is the initialization scheme. %and $d_{w_1^l }$ is the \highlight{shape} \baigd{what is shape?} of $w_1^l$.
	A default setting  is to apply  standard weight initialization scheme which returns random values sampling  from the Gaussian distribution of mean 0 and variance 1, with $\delta = 0.1$.
	%	(such as ``$\mathit{randn}$'' that returns random values sampling from the Gaussian distribution of mean 0 and variance 1), .	
	By tuning $\delta$, the gap between \short solution and the centralized optimal solution can be adjusted accordingly  (detailed in Section \ref{sec:init}) .
	
\end{itemize}
%Since every $w_1$ is initialized from the same distribution, we have $\displaystyle \|\mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$  exponentially small (theoretically reaches to $0$) with growth of $m$ .
%(e.g., with randomization from uniform distribution, it decreases from $10^{-3}$ with $m = 10$ to $10^{-5}$ with $m = 100$).
%\yanjun{introduce initialization parameter $\delta$}
%Intuitively,



\subsection{Proof of Theorem \ref{theorem:main}}
We start with the following lemma that is soon used in our proof.
\begin{lemma}
	\label{lemma:inner}
	Let $S_{k+1} = \frac{1}{2} \|w_{k+1}^l - w_*\|_2^2$, and $S_{k} = \frac{1}{2} \|w_{k}^l - w_*\|_2^2$.  Let $\nabla F(\cdot) = \frac{1}{n} \sum_{i=1}^{n}  \nabla F(\cdot, \xi_{i})$.  %Because in Equation \ref{equ:regret}, the w_* is computed using \xi. Therefore, \nabla F(\cdot) should denote the gradient taken by batch update on $F$ with respect to $\xi$ as well, otherwise, we cannot derive inequality by Equation \ref{equ:convex}.
	We have
	\begin{multline*}
		\langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle =
		\frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 %first term
		- \frac{1}{\alpha_k} (S_{k+1}-S_k)\\ %second term
		- \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle. %third term
	\end{multline*}
\end{lemma}
%We give the proof in Appendix \ref{apx:lemma}.
\begin{proof}
	\begin{equation}
		\label{equ:lemma}
		\begin{aligned}
			& S_{k+1} - S_k = \frac{1}{2} \bigg( \|w_{k+1}^l - w_*\|_2^2 -  \|w_{k}^l - w_*\|_2^2 \bigg) \\
			&= \frac{1}{2} \bigg( \|w_k^l - \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)  - w_*\|_2^2 - \|w_{k}^l - w_*\|_2^2 \bigg) \\
			&= \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 - \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\rangle\\
			&= \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 \\
			& \qquad - \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) + \nabla F(w_k^l) - \nabla F(w_k^l) \rangle\\
			& = \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 -  \alpha_k \langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle\\
			& \qquad  \qquad \qquad- \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l) \rangle
		\end{aligned}
	\end{equation}
	Dividing the above equation by $\alpha_k$, we can get the lemma.
\end{proof}

%\baigd{The proof of theorem 1 is not quite easy to follow. I think it would be better to give some semantics or meaning to each term. Look at the page 8 of this paper: A security framework for the analysis and design of software attestation. It shows a good. It shows a very good example to break a long formula into terms }
In the following, we give the proof of Theorem \ref{theorem:main}.
\begin{proof}
	By the definition in Equation \ref{equ:regret}, we have
	\begin{equation}
		\label{equ:conv}
		\mathcal{R} = \frac{1}{T} \sum_{k=1}^{T} (F(w_k^l) - F(w_*)) \leq \frac{1}{T} \sum_{k=1}^{T} \langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle
	\end{equation}
	It follows from Assumption \ref{assum:convex}'s Equation \ref{equ:convex}. %, \baigd{this sentence is ambiguous}i.e., the convexity of the loss function.
	Inserting the result from Lemma \ref{lemma:inner} to Inequation \ref{equ:conv} and multiplying by $T$, we obtain
	\begin{equation}
		\label{equ:threeterms}
		\begin{aligned}
			T \cdot R & \leq  \sum_{k=1}^{T} \bigg( 	\frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 \\
			& \quad - \frac{1}{\alpha_k} (S_{k+1}-S_k)- \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \bigg) \\
			& \leq \sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 - \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k)\\
			&  \quad - \sum_{k=1}^{T}  \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle
		\end{aligned}
	\end{equation}
	%There are three terms . 
	Semantically, the first term  in Inequation \ref{equ:threeterms}, i.e., $\sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2$ indicates the range of solution space; 
	the second term $-\sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k)$ sums up the model updates throughout the training iterations, which in essence indicates the range of solution space as well; 
	and the third term $- \sum_{k=1}^{T}  \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle$ measures the gap of the gradient between  \short and the centralized training. 
	
	We now bound the three terms individually in the following. 	
	For the first term, we have
	\begin{align}
		\sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 & \leq \sum_{k=1}^{T} \frac{1}{2} \frac{\alpha}{(k+\mu T)^2} m^2 G^2 ~\label{equ:firstbound}\\
		&=\frac{\alpha m^2 G^2}{2} \sum_{k=1}^{T} \frac{1}{(k+\mu T)^2} < \alpha m^2 G^2 ~\label{equ:basel}
	\end{align}
	Inequation \ref{equ:firstbound} is from  Assumption \ref{assum:sol}\ref{assum:solb}, and Inequation \ref{equ:basel} is from the fact $\sum_{x=1}^{\infty} \frac{1}{x^2} \rightarrow 2$.
	
	For the second term, we have
	\begin{align}
		- \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k) & = \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_k-S_{k+1}) \\
		&= \sum_{k=1}^{T} \frac{1}{\alpha_k} \bigg( \frac{1}{2} \|w_{k}^l - w_*\|_2^2 - \frac{1}{2} \|w_{k+1}^l - w_*\|_2^2 \bigg)\\
		& \leq \sum_{k=1}^{T} \frac{1}{2\alpha_k}  \|(w_{k}^l - w_*)- (w_{k+1}^l - w_*)\|_2^2 ~\label{equ:reversetria}\\
		& = \sum_{k=1}^{T} \frac{1}{2\alpha_k} \|w_{k}^l - w_{k+1}^l \|_2^2 \\
		&=  \sum_{k=1}^{T} \frac{1}{2\alpha_k}  \|\alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2\\
		& = \sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 < \alpha m^2 G^2 ~\label{equ:second}
	\end{align}
	Inequation \ref{equ:reversetria} comes from reverse triangle inequality, and Inequation \ref{equ:second} is from the result of the first term.
	
	For the final term, we use the following claim, which we prove afterwards.
	\begin{claim}
		\label{claim:term3}
		\begin{equation}
		\begin{aligned}
	&- \sum_{k=1}^{T}\langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \\
	&< DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{T}{\mu T +1} + \ln |\mu T +1|)
\end{aligned}
		\end{equation}
	\end{claim}

	Combining Inequations \ref{equ:threeterms}, \ref{equ:basel}, \ref{equ:second} and Claim \ref{claim:term3}, and dividing by T we obtain
\begin{align*}
	\mathcal{R} &< \frac{2 \alpha m^2 G^2}{T} + DL \|\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{1}{\mu T +1} + \frac{\ln |\mu T +1|}{T}) \\
	& =
	\begin{cases}
		O(\epsilon + \frac{1}{\mu T +1}), & \text{if } \mu \rightarrow 0 \vspace{0.3cm}\\
		O(\epsilon + \frac{\ln |\mu T +1|}{T}), & \text{if } \mu \rightarrow 1
	\end{cases}	
\end{align*}
concluding the proof.
\end{proof}

	%For the third term, we have
\paragraph{Proof of Claim \ref{claim:term3}}
	\begin{proof}
	\mathleft
\[- \sum_{k=1}^{T}\langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \]
\mathcenter
\begin{align}
	&=\langle w_{k}^l - w_*, \sum_{k=1}^{T} \big(\nabla F(w_k^l) - \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\big)\rangle \\
	&\leq \|w_{k}^l - w_*\|\cdot\|\sum_{k=1}^{T} \big(\nabla F(w_k^l) - \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\big)\| ~\label{equ:tria}\\
	&\leq \|w_{k}^l - w_*\|\cdot L \| \sum_{k=1}^{T} \sum_{j=1}^{m} (w_k^l -  w_k^j)\| ~\label{equ:lip}\\
	&\leq DL\|\sum_{j=1}^{m}(w_1^l-w_1^j) + ... +  \sum_{j=1}^{m}(w_T^l-w_T^j)\| ~\label{equ:assu3a}
\end{align}
\begin{equation}
	\begin{aligned}
		= DL \|&T\sum_{j=1}^{m}(w_1^l-w_1^j)  \\
		&-\sum_{k=1}^{T-1} \sum_{j=1}^{m} \alpha_{(T-k)} k \big(\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\big) \| ~\label{equ:rew}
	\end{aligned}
\end{equation}
\begin{equation}
	\begin{aligned}
		\leq  DL & \bigg(\|T\sum_{j=1}^{m}(w_1^l-w_1^j)\|  \\
		&+ \| \sum_{k=1}^{T-1} \sum_{j=1}^{m} \alpha_{(T-k)} k \big(\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\big) \| \bigg)~\label{equ:rewnorm}
	\end{aligned}
\end{equation}
\begin{align}
	&\leq  DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + DL\cdot2m^2G \sum_{k=1}^{T-1} \alpha_{(T-k)} k \quad \quad \quad \quad ~\label{equ:assu3b} \\
	& = DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL \sum_{k=1}^{T-1} \frac{k}{((1+\mu)T-k)^2}~\label{equ:insertalpha} \\
	& < DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{T}{\mu T +1} + \ln |\mu T +1|) ~\label{equ:integral}
\end{align}

Inequations \ref{equ:tria} and \ref{equ:rewnorm} are from triangle inequality.
Inequation \ref{equ:lip} is from the fact $\nabla F(w_k^l) = \frac{1}{n} \sum\limits_{i=1}^{n}  \nabla F(w_k^l, \xi_{i}) = \sum\limits_{j=1}^{m} g^j(w_k^l, \xi_j)$ and Assumption \ref{assum:Lip}'s blockwise Lipschitz-continuity.
Inequation \ref{equ:assu3a} is from Assumption \ref{assum:sol}\ref{assum:sola} and represents $\sum\limits_{k=1}^{T}(\cdot) $ by a summand sequence.
Equation \ref{equ:rew} comes from the fact
\begin{multline*}
	w_k^l-w_k^j = (w_1^l - \alpha_1 \nabla F(w_1^l) - ... - \alpha_k \nabla F(w_k^l)) \\
	-(w_1^j - \alpha_1 \sum\limits_{j=1}^{m}g^j(w_1^j, \xi_j) - ... - \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j))\\
	= (w_1^l - w_1^j) - \alpha_1 (\nabla F(w_1^l) - \sum\limits_{j=1}^{m}g^j(w_1^j, \xi_j)) \\
	-...- \alpha_k(\nabla F(w_k^l) -  \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)).
\end{multline*}
Inequation \ref{equ:assu3b} is from Assumption \ref{assum:sol}\ref{assum:solb}, which gives $\|\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\| \leq 2mG$.
Equation \ref{equ:insertalpha} is obtained by inserting $\alpha_{(T-k)} = \frac{\alpha}{(T-k +\mu T)^2}$.
Inequation \ref{equ:integral} is from the following fact. Since
\[\int_a^b \frac{k}{(c-k)^2}\, dk = \frac{b}{c-b} + \ln |c-b| - \frac{a}{c-a} - \ln |c-a|,\]
we have
\begin{align*}
	&\int_1^{T-1} \frac{k}{((1+\mu)T-k)^2}\, dk = \frac{T-1}{(1+\mu)T-(T-1)} \\
	&+ \ln |(1+\mu)T-(T-1)| - \frac{1}{(1+\mu)T-1} - \ln |(1+\mu)T-1|\\
	&<\frac{T-1}{(1+\mu)T-(T-1)}+ \ln |(1+\mu)T-(T-1)| \text{ \quad (with $T\geq2$). } \\
	&< \frac{T}{\mu T +1} + \ln |\mu T +1|
\end{align*}	
	\end{proof}
	


==> chapters/convergence2.tex <==
\section{Convergence Analysis}
\label{sec:convergence}

In this section, we conduct a formal convergence analysis on \short.
Convergence analysis has been extensively used in the literature~\cite{hu2019fdml, hsieh2017gaia, ho2013more} to prove the correctness of optimization algorithms.
We demonstrate the bound of the distance between an arbitrary $w_*^l$ learned by \short and the centralized model $w_*$.
The analysis is centered around a \emph{regret} function $\mathcal{R}$, which is the difference between the \short's training loss %\highlight{confined in any participant $l$}\baigd{what does this mean?}
and the loss of the %\highlight{centralized optimum}\baigd{can we see centralized model?}
centralized model, defined as
\begin{equation}
	\label{equ:regret}
\mathcal{R} = \frac{1}{T} \sum_{k=1}^{T} (F(w_k^l) - F(w_*))
\end{equation}

%We prove that $\mathcal{R}$ is bounded by $\displaystyle \epsilon = m \|\mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$.


\subsection{Assumptions}
We make the following  assumptions on the loss function $F$.
They all are common assumptions in convergence analyses of most gradient-based methods, and satisfied in a variety of widely used cost functions~\cite{bottou2018optimization}, such as mean squared error (MSE) and cross entropy.
%\baigd{Also need a sentence to argue these assumptions will not introduce extra constraints to those loss functions used by existing learning algorithms. Give examples, citations to support}

\begin{assumption}
	\label{assum:Lip}
(Lipschitz continuity). %\baigd{objective gradients sounds weird}
The loss function $F$: $\mathbb{R}^d \rightarrow \mathbb{R}$ is continuously differentiable and the gradient function of $F$, namely, $\nabla F$: $\mathbb{R}^d \rightarrow \mathbb{R}^d$, is Lipschitz continuous with Lipschitz constant $L > 0$, %i.e.,
\begin{equation}
\|\nabla F(w) - \nabla F(\widehat{w})\|_2 \leq L\|w-\widehat{w}\|_2 \text{\quad for all } \{w,\widehat{w}\} \subset \mathbb{R}^d.
\end{equation}
\end{assumption}
%Any differentiable function whose gradient is Lipschitz continuous is a continuously differentiable function.
Intuitively, this assumption ensures that the gradient of $F$ does not change arbitrarily %\replace{quickly with respect to $w$}{in the course of descending}
in the course of descending, such that the gradient can be a useful indicator %\replace{for decreasing $F$}{towards the optimal}
towards the optimum~\cite{bottou2018optimization}. %Such an assumption is essential for convergence analyses of most gradient-based methods;
%Without it, the gradient would not provide a good indicator for how far to move to decrease F

\begin{assumption}
	\label{assum:convex}
	(Strong convexity).
	The loss function $F$: $\mathbb{R}^d \rightarrow \mathbb{R}$ is strongly convex such that
	\begin{equation}
		F(\widehat{w}) \geq F(w) + \nabla F(w)^T(\widehat{w}-w)  \text{\quad for all } \{w,\widehat{w}\} \subset \mathbb{R}^d.
	\end{equation}
\end{assumption}

A useful fact from Assumption \ref{assum:convex} for our analysis is
\begin{equation}
	\label{equ:convex}
(F(w)-F(w_*)) \leq \langle w-w_*, \nabla F(w) \rangle  \text{\quad for all } w \subset \mathbb{R}^d,
\end{equation}
where $\langle\cdot{,}\cdot\rangle$ denotes the inner product operation.

In addition, we adopt the same assumption on a bounded solution space used in related studies~\cite{bottou2018optimization, hu2019fdml}.
\begin{assumption}
	\label{assum:sol}
(Bounded solution space). The set of $\{w_k^l\}|_{k \in [1,T]}$ %\baigd{this is a set. consider another way to denote sequence}
is contained in an open set over which $F$ is bounded below a scalar $F_{inf}$, such that
\begin{enumerate}[label=(\alph*)]
\item  there exists a $D>0$, s.t.,	$\|w_k^l-w_*\|_2^2 \leq D^2$ for all $k$, and \label{assum:sola}
\item there exists a $G>0$, s.t., $\|g^l(w_k^l, \xi_l)\|_2^2 \leq G^2$ for all $w_k^l \subset \mathbb{R}^d$.  ~\label{assum:solb} %\baigd{why need square?}
\end{enumerate}
\end{assumption}

\subsection{Main Theorem}

The following theorem demonstrates our main result on the converge rate of \short.
\begin{theorem}
	\label{theorem:main}
With Assumptions \ref{assum:Lip} - \ref{assum:sol}, and a learning rate of $\alpha_k = \frac{\alpha}{(k+\mu T)^2}$ ($0<\mu <1$), the regret $\mathcal{R}$ given by Algorithm \ref{alg:cgd} for \short optimization is
\begin{equation}
	\mathcal{R} =O(\epsilon + \frac{1}{\mu T +1}+ \frac{\ln |\mu T +1|}{T})
%\begin{cases}
%	O(\epsilon + \frac{1}{\mu T +1}), & \text{if } \mu \rightarrow 0 \vspace{0.3cm}\\
%	O(\epsilon + \frac{\ln |\mu T +1|}{T}), & \text{if } \mu \rightarrow 1,
%\end{cases}	
\end{equation}%\baigd{what do $\mu \rightarrow 0$ and $\mu \rightarrow 1$ mean?}
where $\epsilon = m \| \displaystyle \mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$. %$ \|\sum_{j=1}^{m}(w_1^l-w_1^j)\| $.
%\yanjun{$m^h$?}
\end{theorem}
The theorem implies the following two remarks. %\replace{facts}{remarks}.
\begin{itemize}
	\item \textbf{Convergence rate.} %\replace{$\mathcal{R}$ decreases as $\frac{1}{\mu T +1}$ or $\frac{\ln |\mu T +1|}{T}$ decreasing to $0$ with regard to $T$}{Both $\frac{1}{\mu T +1}$ and $\frac{\ln |\mu T +1|}{T}$ approach 0 as $T$ increases}, \baigd{sounds weird} \replace{meaning}{implying} that %\remove{the solution of}
	Both $\frac{1}{\mu T +1}$ and $\frac{\ln |\mu T +1|}{T}$ approach 0 as $T$ increases,  implying that
	\short will converge toward the optimum. %\remove{value}.
%\baigd{We need to check this term throughout the paper: optimal, optimality or optimum? What is used in literature?}
	%\remove{In addition,} 
	The convergence rate can be adjusted by the parameter $\mu$~(%\replace{the choice of}{determining} 
	the effect of $\mu$ in practice will be discussed in Section \ref{sec:mu}).
	%\item \textbf{Bounded \highlight{optimality} gap. } \baigd{gap sounds weird. distance?} %\replace{The maximum difference between short solution and the centralized optimal solution is bounded by $\epsilon$.}{When \short converges, the maximum difference the confined model and the central model is bounded by $\epsilon$.} \baigd{have a consideration on the terms. whether you want to look at it from a pure mathematical or FL perspective }
	\item \textbf{Bounded optimality gap. }
	When \short converges, the maximum %\highlight{gap}
	gap between the confined model and the centralized model is bounded by $\epsilon$.
	%\replace{Here, we introduce}{\short uses} 
	\short uses the initialization parameter $\delta^l$ %\replace{, which decides}{to determine} 
	to determine the range of $w_1^l$  in the way of 
	\begin{equation}
		\label{equ:delta}
		w_1^l = \delta^l\cdot \mathit{Rand}^l  \text{\quad for all } l \in (1, m),
	\end{equation}
	where $\mathit{Rand}$ is the initialization scheme. A standard $\mathit{Rand}$ used in machine learning is to apply random sampling from the Gaussian distribution of mean 0 and the variance 1, and a standard $\delta$ is $\frac{1}{\sqrt n}$ (where $n$ is the sample size)~\cite{glorot2010understanding}. %and $d_{w_1^l }$ is the \highlight{shape} \baigd{what is shape?} of $w_1^l$.
%\baigd{need to brief what initialization parameter and initialization scheme are. Also, reviewers may think why there are two, what are the roles for either of them}
	In \short, each participant %\replace{confines}{determines} 
	determines its own $\mathit{Rand}^l$ and $\delta^l$ %\baigd{should they become $\mathit{Rand^l}$ and $\delta^l$} 
	independently to avoid leaking the average distance among the confined models.
	Our experiment finds that \short keeps robust~(in terms of %\baigd{what accuracy} 
	validation accuracy) %\add{even when its participants select their $\delta$s}
	even when the participants select their $\delta^l$s uniformly at random in a range of $(\frac{10}{\sqrt n}, \frac{0.1}{\sqrt n})$ (cf. Section \ref{sec:init}). %by  \baigd{do you mean two orders. 100 orders means $10^{100}$}orders with regards to $\delta$ .
		
	%A default setting  is to apply %\baigd{a or the}
	%a standard weight initialization scheme which %\replace{returns random values sampling}{generates random values sampled}
	%generates random values sampled  from the Gaussian distribution of mean 0 and variance 1, with $\delta = 0.1$.
	 %initialization of the confined models.
	%By tuning $\delta$, the gap between \short solution and the centralized optimum can be adjusted accordingly  (detailed in Section \ref{sec:init}) .
\end{itemize}
%Since every $w_1$ is initialized from the same distribution, we have $\displaystyle \|\mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$  exponentially small (theoretically reaches to $0$) with growth of $m$ .
%(e.g., with randomization from uniform distribution, it decreases from $10^{-3}$ with $m = 10$ to $10^{-5}$ with $m = 100$).
%\yanjun{introduce initialization parameter $\delta$}
%Intuitively,



\subsection{Proof of Theorem \ref{theorem:main}}
%We first introduce the following lemma that is used in our proof. %for decomposing the upper bound of  $\mathcal{R}$.

We are interested in an upper bound of  $\mathcal{R}$. %, which has an upper bound of $\langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle$ by the convexity of the cost function. 
To this end, we consider the trend of the distance from the confined model $w_{k}^l$ and the final optimum $w_*$ during the iterations. 
We define the distance as  $S_{k} = \frac{1}{2} \|w_{k}^l - w_*\|_2^2$,  
which is related to the deviation  between $\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)$ (i.e., the descent in  \short)  and $\nabla F$ (i.e., the descent in the centralized training). 
We first introduce the following lemma which describes the relationship between such deviation and the trend of $S_{k}$. %by taking the difference of $S_{k+1}$ and $S_{k}$. %, and illustrates the contribution of the gap to the upper bound of $\mathcal{R}$.
%To represent the gap, 

% By defining the distance $S_{k}$ from $w_{k}^l$ to $w_*$, and taking the difference of $S_{k+1}$ and $S_{k}$,  
%\baigd{If possible add one sentence to introduce the lemma, like ``It describes the trend of the distance between the confined model and the final optimum during the iterations.''}

%We start with the following lemma that is soon used in our proof.
%\baigd{fix the index. No lemma 1}
\begin{lemma}
	\label{lemma:inner}
	Let $S_{k+1} = \frac{1}{2} \|w_{k+1}^l - w_*\|_2^2$ and $S_{k} = \frac{1}{2} \|w_{k}^l - w_*\|_2^2$.  Let $\nabla F(\cdot) = \frac{1}{n} \sum_{i=1}^{n}  \nabla F(\cdot, \xi_{i})$.  %Because in Equation \ref{equ:regret}, the w_* is computed using \xi. Therefore, \nabla F(\cdot) should denote the gradient taken by batch update on $F$ with respect to $\xi$ as well, otherwise, we cannot derive inequality by Equation \ref{equ:convex}.
	We have
	%\vspace{-0.1cm}
	\begin{multline*}
		\langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle =
		\frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 %first term
		- \frac{1}{\alpha_k} (S_{k+1}-S_k)\\ %second term
		- \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle. %third term
	\end{multline*}
	%\vspace{-0.5cm}
\end{lemma}
%We give the proof in Appendix \ref{apx:lemma}.

%By defining the distance $S_{k}$ from $w_{k}^l$ to $w_*$, and taking the difference of $S_{k+1}$ and $S_{k}$, we are able to introduce the measurement of the difference between the gradient

%\baigd{Give some intuition about the lemma here to facilitate reading, so the reader knows what its use without reading the formula.}
\begin{proof}
	%\vspace{-0.5cm}
	\begin{equation}
		\label{equ:lemma}
		\begin{aligned}
			& S_{k+1} - S_k = \frac{1}{2} \bigg( \|w_{k+1}^l - w_*\|_2^2 -  \|w_{k}^l - w_*\|_2^2 \bigg) \\
			&= \frac{1}{2} \bigg( \|w_k^l - \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)  - w_*\|_2^2 - \|w_{k}^l - w_*\|_2^2 \bigg) \\
			&= \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 - \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\rangle\\
			&= \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 \\
			& \qquad - \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) + \nabla F(w_k^l) - \nabla F(w_k^l) \rangle\\
			& = \frac{1}{2} \| \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 -  \alpha_k \langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle\\
			& \qquad  \qquad \qquad- \alpha_k \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l) \rangle
		\end{aligned}
	\end{equation}
	Dividing the above equation by $\alpha_k$, we can %\replace{get}{prove}
	prove the lemma.
\end{proof}

%\baigd{The proof of theorem 1 is not quite easy to follow. I think it would be better to give some semantics or meaning to each term. Look at the page 8 of this paper: A security framework for the analysis and design of software attestation. It shows a good. It shows a very good example to break a long formula into terms }
In the following, we give the proof of Theorem \ref{theorem:main}.
Our proof starts with utilizing the convexity of the objective function to obtain the upper bound of  $\mathcal{R}$.
The bound can be decomposed into three terms based on Lemma \ref{lemma:inner}.
We then explore the boundedness of each term, and taking these bounds together concludes the proof.

%\baigd{If possible, brief introduce the proof schema rather than throwing the proof to the readers, so that they can appreciate how you solve this problem}
\begin{proof}
	By the definition %\add{of the regret function}
	of the regret function~(Equation \ref{equ:regret}) and Assumption \ref{assum:convex}'s Equation \ref{equ:convex}, %\baigd{this is actually based on assumption 2, isn't it?}
	we have
	\begin{equation}
		\label{equ:conv}
		\mathcal{R} = \frac{1}{T} \sum_{k=1}^{T} (F(w_k^l) - F(w_*)) \leq \frac{1}{T} \sum_{k=1}^{T} \langle w_{k}^l - w_*, \nabla F(w_k^l) \rangle
	\end{equation}
	%It follows from Assumption \ref{assum:convex}'s Equation \ref{equ:convex}. %, \baigd{this sentence is ambiguous}i.e., the convexity of the loss function.
	%\highlight{Inserting} \baigd{it seems Chinese. ``Applying Lemma 2''?} \remove{the result from}
	Applying Lemma \ref{lemma:inner} to Inequation \ref{equ:conv} and multiplying by $T$, we obtain
	\begin{equation}
		\label{equ:threeterms}
		\begin{aligned}
			T \cdot R & \leq  \sum_{k=1}^{T} \bigg( 	\frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 \\
			& \quad - \frac{1}{\alpha_k} (S_{k+1}-S_k)- \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \bigg) \\
			& \leq \sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 - \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k)\\
			&  \quad - \sum_{k=1}^{T}  \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle
		\end{aligned}
	\end{equation}
	%There are three terms .
	%\remove{Semantically,} t
	Inequation \ref{equ:threeterms} can be decomposed into three terms.
  The first term $\sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2$ indicates the range of solution space;
	the second term $-\sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k)$ sums up the model updates throughout the training iterations, which indicates the range of solution space; 
	%\highlight{in essence indicates the range of solution space as well}; \baigd{not quite clear. ``which affects the rance of solution space''?}
	the third term $- \sum_{k=1}^{T}  \langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle$ measures the gap of the gradient between  \short and the centralized training.
	
	Next, we %\replace{bound the three terms individually}{explore the boundedness of each term}
	explore the boundedness of each term. 	
	For the first term, we have
	\begin{align}
		\sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 & \leq \sum_{k=1}^{T} \frac{1}{2} \frac{\alpha}{(k+\mu T)^2} m^2 G^2 ~\label{equ:firstbound}\\
		&=\frac{\alpha m^2 G^2}{2} \sum_{k=1}^{T} \frac{1}{(k+\mu T)^2} < \alpha m^2 G^2 ~\label{equ:basel}.
	\end{align}
	Inequation \ref{equ:firstbound} is from  Assumption \ref{assum:sol}\ref{assum:solb}, and Inequation \ref{equ:basel} is from the fact $\sum_{x=1}^{\infty} \frac{1}{x^2} \rightarrow 2$.
	
	For the second term, we have
	\begin{align}
		- \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_{k+1}-S_k) & = \sum_{k=1}^{T} \frac{1}{\alpha_k} (S_k-S_{k+1}) \\
		&= \sum_{k=1}^{T} \frac{1}{\alpha_k} \bigg( \frac{1}{2} \|w_{k}^l - w_*\|_2^2 - \frac{1}{2} \|w_{k+1}^l - w_*\|_2^2 \bigg)\\
		& \leq \sum_{k=1}^{T} \frac{1}{2\alpha_k}  \|(w_{k}^l - w_*)- (w_{k+1}^l - w_*)\|_2^2 ~\label{equ:reversetria}\\
		& = \sum_{k=1}^{T} \frac{1}{2\alpha_k} \|w_{k}^l - w_{k+1}^l \|_2^2 
		=  \sum_{k=1}^{T} \frac{1}{2\alpha_k}  \|\alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2\\
		& = \sum_{k=1}^{T} \frac{1}{2} \alpha_k \|\sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\|_2^2 < \alpha m^2 G^2 ~\label{equ:second}
	\end{align}
	Inequation \ref{equ:reversetria} follows reverse triangle inequality, and Inequation \ref{equ:second} reuses the result of the first term (cf. Equation \ref{equ:basel}).
	
	%\replace{For the final term, we use the following claim, which we prove afterwards.}{Determining the bound of the third term is slightly complex. We list is as the following claim, and prove it soon after the proof of Theorem~\ref{theorem:main}.}
	Determining the bound of the third term is slightly complex. We list it as the following claim, and prove it soon after the proof of Theorem~\ref{theorem:main}.
	\begin{claim}
		\label{claim:term3}
		\begin{equation}
		\begin{aligned}
	&- \sum_{k=1}^{T}\langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \\
	&< DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{T}{\mu T +1} + \ln |\mu T +1|)
\end{aligned}
		\end{equation}
	\end{claim}

	Combining Inequations \ref{equ:threeterms}, \ref{equ:basel}, \ref{equ:second} and Claim \ref{claim:term3}, and dividing by T we obtain
\begin{align*}
	\mathcal{R} &< \frac{2 \alpha m^2 G^2}{T} + DL \|\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{1}{\mu T +1} + \frac{\ln |\mu T +1|}{T}) \\
	& = O(\epsilon + \frac{1}{\mu T +1}+ \frac{\ln |\mu T +1|}{T}), \text{concluding the proof.}
	%\begin{cases}
	%	O(\epsilon + \frac{1}{\mu T +1}), & \text{if } \mu \rightarrow 0 \vspace{0.3cm}\\
	%	O(\epsilon + \frac{\ln |\mu T +1|}{T}), & \text{if } \mu \rightarrow 1
	%\end{cases}	
\end{align*}
\end{proof}

	%For the third term, we have
\paragraph{Proof of Claim \ref{claim:term3}}
	\begin{proof}
	\mathleft
\[- \sum_{k=1}^{T}\langle w_{k}^l - w_*, \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j) - \nabla F(w_k^l)\rangle \]
\mathcenter
%\vspace{-0.7cm}
\begin{align}
	&=\langle w_{k}^l - w_*, \sum_{k=1}^{T} \big(\nabla F(w_k^l) - \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\big)\rangle \\
	&\leq \|w_{k}^l - w_*\|\cdot\|\sum_{k=1}^{T} \big(\nabla F(w_k^l) - \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)\big)\| ~\label{equ:tria}\\
	&\leq \|w_{k}^l - w_*\|\cdot L \| \sum_{k=1}^{T} \sum_{j=1}^{m} (w_k^l -  w_k^j)\| ~\label{equ:lip}\\
	&\leq DL\|\sum_{j=1}^{m}(w_1^l-w_1^j) + ... +  \sum_{j=1}^{m}(w_T^l-w_T^j)\| ~\label{equ:assu3a}
\end{align}
\begin{equation}
%\vspace{-0.3cm}
	\begin{aligned}
		= DL \|&T\sum_{j=1}^{m}(w_1^l-w_1^j)  \\
		&-\sum_{k=1}^{T-1} \sum_{j=1}^{m} \alpha_{(T-k)} k \big(\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\big) \| ~\label{equ:rew}
	\end{aligned}
\end{equation}
\begin{equation}
	\begin{aligned}
		\leq  DL & \bigg(\|T\sum_{j=1}^{m}(w_1^l-w_1^j)\|  \\
		&+ \| \sum_{k=1}^{T-1} \sum_{j=1}^{m} \alpha_{(T-k)} k \big(\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\big) \| \bigg)~\label{equ:rewnorm}
	\end{aligned}
\end{equation}
\begin{align}
	&\leq  DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + DL\cdot2m^2G \sum_{k=1}^{T-1} \alpha_{(T-k)} k \quad \quad \quad \quad ~\label{equ:assu3b} \\
	& = DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL \sum_{k=1}^{T-1} \frac{k}{((1+\mu)T-k)^2}~\label{equ:insertalpha} \\
	& < DL \|T\sum_{j=1}^{m}(w_1^l-w_1^j)\| + 2m^2GDL(\frac{T}{\mu T +1} + \ln |\mu T +1|) ~\label{equ:integral}
\end{align}

Inequations \ref{equ:tria} and \ref{equ:rewnorm} are from triangle inequality.
Inequation \ref{equ:lip} is from the fact $\nabla F(w_k^l) = \frac{1}{n} \sum\limits_{i=1}^{n}  \nabla F(w_k^l, \xi_{i}) = \sum\limits_{j=1}^{m} g^j(w_k^l, \xi_j)$ and Assumption \ref{assum:Lip}'s blockwise Lipschitz-continuity.
Inequation \ref{equ:assu3a} is from Assumption \ref{assum:sol}\ref{assum:sola} and represents $\sum\limits_{k=1}^{T}(\cdot) $ by a summand sequence.
Equation \ref{equ:rew} comes from the fact
\begin{multline*}
	w_k^l-w_k^j = (w_1^l - \alpha_1 \nabla F(w_1^l) - ... - \alpha_k \nabla F(w_k^l)) \\
	-(w_1^j - \alpha_1 \sum\limits_{j=1}^{m}g^j(w_1^j, \xi_j) - ... - \alpha_k \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j))\\
	= (w_1^l - w_1^j) - \alpha_1 (\nabla F(w_1^l) - \sum\limits_{j=1}^{m}g^j(w_1^j, \xi_j)) \\
	-...- \alpha_k(\nabla F(w_k^l) -  \sum\limits_{j=1}^{m}g^j(w_k^j, \xi_j)).
\end{multline*}
Inequation \ref{equ:assu3b} follows Assumption \ref{assum:sol}\ref{assum:solb} from which we obtain $\|\nabla F(w_{(T-k)}^l) -  \sum\limits_{j=1}^{m}g^j(w_{(T-k)}^j, \xi_j)\| \leq 2mG$.
Equation \ref{equ:insertalpha} is obtained by %\replace{inserting}{applying} 
applying $\alpha_{(T-k)} = \frac{\alpha}{(T-k +\mu T)^2}$.
Inequation \ref{equ:integral} is from the following fact. 

Since\[\int_a^b \frac{k}{(c-k)^2}\, dk = \frac{b}{c-b} + \ln |c-b| - \frac{a}{c-a} - \ln |c-a|,\]
we have
\begin{align*}
	&\int_1^{T-1} \frac{k}{((1+\mu)T-k)^2}\, dk = \frac{T-1}{(1+\mu)T-(T-1)} \\
	&+ \ln |(1+\mu)T-(T-1)| - \frac{1}{(1+\mu)T-1} - \ln |(1+\mu)T-1|\\
	&<\frac{T-1}{(1+\mu)T-(T-1)}+ \ln |(1+\mu)T-(T-1)| \text{ \quad (with $T\geq2$) } \\
	&< \frac{T}{\mu T +1} + \ln |\mu T +1|
\end{align*}	
%\baigd{what is (with $T\geq2$).?}
	\end{proof}
	


==> chapters/design.tex <==
\section{\codename}

%\baigd{This should be moved to 3.2. Discuss it together with Table 1}
%\baigd{An important information missing: when is the local gradients shared, in each iteration or only once in the end?}

%We propose \codename (\short), which is an optimization method for confined global models. Our approach makes it straightforward to achieve the property of privacy-preservation, while at the same time, theoretically guarantees the convergence of the optimization, i.e., each $w^l_{k}$ will converge to the neighborhoods of the optimal solution of centralized training.

In this section, we describe the formal problem statements (Section \ref{sec:problem}); and the process of \short optimization (Section \ref{sec:optimization}).


\subsection{Problem formulation}
\label{sec:problem}
Consider a centralized dataset $\xi = \{(x_i, y_i)\}^n_{i=1}$, consisting of $n$ training samples.
The goal of machine learning is to find a model $h(w,x)$ with parameter $w$ that given input $x$, can predict its label $y$ by minimizing the loss between the model prediction $h(w,x_i)$ and its corresponding label $y_i$ over all training samples $i$. In general, the model is trained by solving the following problem
%\baigd{argmin}
\begin{equation}
	argmin_w \frac{1}{n} \sum_{i=1}^{n} F (w;\xi) + \lambda z(w),
\end{equation}
where $F(w;\xi)$ is the loss function, and $z(w)$ is the regularizer for $w$. We use $w_*$ to denote the optimal solution of centralized training.

In the federated learning setting, we have a system of $m$ local participants, each participant holding a private set $\xi_l \subseteq \xi $ $(l \in [1,m])$ %\baigd{$\subseteq$?}
consisting of a part of training samples with a part of features (may have common entries with others). % in a way that $\xi$ can be partitioned horizontally (by samples), vertically (by features), or in a mixed manner (by both).
Let $w^l_{k}$ denote the %\highlight{confined model}
confined model belonging to the participant $l$ at $k^{th}$ iteration, where $k \in [1,T]$ and $T$ is the total number of iterations. We let
\begin{equation}
	\label{equ:gl}
g^l(w^l_{k}, \xi_l)=\frac{1}{|\xi_{l}|}  \nabla F(w^l_{k}, \xi_{l}),
\end{equation} %\baigd{Where are $n_l$ and $\xi_{l,i}$ defined? }
which represents the local gradient with respect to $\xi_l$. We use $w^l_*$ to denote the solution of the federated learning using \short.

The objective of \short is to make $w^l_*$ converge to a neighborhood of the centralized optimal value $w_*$ within a bounded difference.

\subsection{\short optimization}
%\yanjun{whether we need to detail the horizontal/vertical partitions in the following algorithm?}
\label{sec:optimization}

Figure \ref{fig:differ} illustrates the architecture of \short (Figure \ref{fig:cgd}) compared with the centralized training  (Figure \ref{fig:central}) and traditional  FL (Figure \ref{fig:existing}). In the centralized training, the datasets are collect centrally for training one centralized model. In the traditional FL , every participant owns its local training dataset, and updates the \emph{same} global model $w_{k}$ (usually via a parameter server) using its local model/gradients. In this paradigm, the local gradients $\nabla F(w_k, \xi_{l,k})$ can be protected via either secure aggregation or differential privacy mechanisms. In \short , each participant learns and confines its own global model (represented by different colors), i.e., each $w_{k}$ with respect to participant $l$, denoted by $w^l_{k}$, is \emph{different and private}.

%In addition, in the traditional FL architecture, the global model, in each iteration, is usually updated by the local gradients pushed by a single participant; while in \short, the confined model is  updated by the \emph{sum} of all the local gradients in each iteration.
In addition, in \short, the model update embraces the information from all the training samples by summing up the local gradients (Figure \ref{fig:cgd}), while in federated SGD/mini-batch (Figure \ref{fig:existing}), the iterate is taken with respect to a subset of training samples $\xi_k$ only.
\short is also clearly different to the batch gradient descent in the centralized training in which the sum is taken over the gradients computed from the same $w_k$ (c.f. Equation \ref{equ:sgd} where $\xi_k = \xi$).

A summary of differences between the traditional FL, i.e., federated SGD/mini-batch\footnote{We refer federated SGD/mini-batch to SGD/mini-batch optimization in the federated learning setting, including plain SGD/mini-batch in which the local gradient/model is shared in plaintext, and  privacy-preserving SGD/mini-batch via secure aggregation or differential privacy mechanisms.}, and \short is given in Table \ref{tab:differ}. By designing the \short algorithm, we theoretically guarantee that each confined model will converge towards the centralized optimal solution to ensure the model accuracy (column 5 in Table \ref{tab:differ} and detailed in Section \ref{sec:convergence}), and also achieve the desired privacy preservation compared to the traditional FL framework (column 6 in Table \ref{tab:differ} and detailed in Section \ref{sec:privacy}).



\begin{figure}
		\centering
	\subfloat[Centralized Training]{{\includegraphics[width=5.8cm]{fig/central.pdf} \label{fig:central}}}%
\qquad
	\subfloat[Traditional Federated Learning]{{\includegraphics[width=8cm]{fig/existing.pdf} \label{fig:existing}}}%
	\qquad
	\subfloat[\short ]{{\includegraphics[width=8cm]{fig/cgd.pdf} \label{fig:cgd}}}%
	\caption{Architectural comparison of the centralized training, traditional federated learning, and \short.}%
\label{fig:differ}	
\end{figure}

\begin{table*}[ht]
	\centering
	\resizebox{1\textwidth}{!}{
		\begin{tabular}{|p{0.11\linewidth} | p{0.15\linewidth} |p{0.11\linewidth} | p{0.16\linewidth} |p{0.22\linewidth} |p{0.22\linewidth}|}
			\hline
			\multicolumn{2}{|c|}{\multirow{2}{*}{Technique}}                                         & \multicolumn{2}{c|}{Methodology}                                                                                                                                                                     & \multicolumn{2}{c|}{Desired properties}                                                                                                                                                                                                                                                                                                                           \\ \cline{3-6}
			\multicolumn{2}{|c|}{}                                                                   & Architecture                                                                       & Model update                                                                                            & Model Accuracy                                                                                                                                                                                                      & Privacy                                                                                                                                     \\ \hline
			%\multicolumn{2}{|l|}{Centralized training via batch-GD}                    & All the data are collected centrally to produce the model.                         & Compute the gradient using all the training samples to update the model in each iteration.                      & N/A                                                                                                                                                                                                         & Theoretically guaranteed convergence.                                                                                                               \\ \hline
			\multirow{3}{*}{\shortstack[l]{Federated \\ SGD/mini-batch  }} & Plain federated SGD/mini-batch~\cite{robbins1951stochastic, bottou2018optimization}                         & \multirow{3}{*}{\shortstack[l]{All the particip-\\ants  jointly  \\learn one and \\ the same  global \\ model.}} & \multirow{3}{*}{\shortstack[l]{Update the model  \\ using  the gradient \\ computed on a subset \\ of  training samples  in \\ each  iteration.}} & Theoretically guaranteed convergence~\cite{robbins1951stochastic, bottou2018optimization}.                                                                                    & The plain sharing of local parameters/gradients is subject to model inversion attack~\cite{melis2019exploiting, fredrikson2015model, shokri2017membership} .                                                                            \\ \cline{2-2} \cline{5-6}
			& Preserving privacy with secure aggregation~\cite{bonawitz2017practical, mohassel2017secureml, zhang2020privcoll,  marc2019privacy, sharma2019confidential, liu2017oblivious}  &                                                                                    &                                                                                                                 & As above, since the mechanism guarantees that the computation result from ciphertext is the same from plaintext~\cite{bonawitz2017practical,mohassel2017secureml}.& The sharing of one and the same global model (even though the local gradients are protected) is still subject to information leakage of original dataset (refer to~\cite{nasr2019comprehensive} and Section \ref{sec:privacy}). \\ \cline{2-2} \cline{5-6}
			& Preserving privacy with differential privacy~\cite{abadi2016deep, song2013stochastic, shokri2015privacy, dwork2014algorithmic, hu2019fdml, zhang2020differentially}  &                                                                                    &                                                                                                                 & Additive noise (in most cases) affects the model accuracy~\cite{dwork2014algorithmic}.                                                                                                    &  The privacy cost is accumulated with repeated accesses to the dataset~\cite{abadi2016deep}.                                                      \\ \hline
			\multicolumn{2}{|l|}{\codename}                                           & Each participant learns and confines a different global model.                     & The model update in each  iteration embraces the information from all the training samples by summing up the local gradients.            & Theoretically guaranteed convergence with bounded difference to the centralized optimal solution.                                                                                                                         & Ensured privacy preservation based on the guarantee of the secure addition operation.                                                   \\ \hline
		\end{tabular}
	}	
	\caption{A summary of differences between the traditional federated learning, i.e., federated SGD/mini-batch, and \short.}
	%{A summary of differences between the traditional federated learning, i.e., federated SGD/mini-batch\protect\footnotemark, and \short.}	
	\label{tab:differ}
\end{table*}
%\footnotetext{We refer federated SGD/mini-batch to SGD/mini-batch optimization in the federated learning setting, including plain SGD/mini-batch in which the local gradient/model is shared in plaintext, and  privacy-preserving SGD/mini-batch via secure aggregation or differential privacy mechanisms.}


Algorithm \ref{alg:cgd} outlines \short optimization for training with confined model parameters $w_k^l$.
In general, the optimization process consists of the following  steps.
\begin{itemize}
\item \textbf{Initialization. } Each  participant $l$ randomizes its own $w_1^l$.
\item \textbf{Step 1. } At each iteration $k$, every participant computes the local gradient $g^l(w^l_{k}, \xi_l)$  with respect to its own private dataset $\xi_l$ using Equation \ref{equ:gl}. %\baigd{this needs equation 4, so what are $n_l$ and $\xi_{l,i}$ w.r.t a participant?}
\item \textbf{Step 2. } Securely compute $\sum\limits_{l=1}^m g^l(w^l_{k}, \xi_l)$ which is later used for iterate update (double lines in Figure \ref{fig:cgd}).

%Here, we remark an important difference of model update between \short and SGD/mini-batch. (column 4 in Table \ref{tab:differ}).
%\baigd{this still needs to be synched. How is it different from the synch in FL, and why is it good? Explaining this clearly is the key of this paper. The ``remark'' below should focus on this}

This step presumes that computational tools exist for securely evaluating the sum of a set of secret values to avoid direct release of plain local gradient $g^l(w^l_{k}, \xi_l)$. (We refer to Section \ref{sec:privacy} for more detail).
\item \textbf{Step 3. } A scalar stepsize $\alpha_k > 0$ is chosen given an iteration number $k\in[1,T]$.
\item \textbf{Step 4. } Every participant takes a descent step on its own $w_k^l$ with $\alpha_k \sum\limits_{l=1}^m g^l(w^l_{k}, \xi_l)$.

\end{itemize}

%At each step of the SGD, we compute the gradient  for a random subset of examples, clip the l2 norm of each gradient, compute the average, add noise in order to protect privacy, and take a step in the opposite direction of this average noisy gradient. At the end, in addition to out- putting the model, we will also need to compute the privacy loss of the mechanism based on the information maintained by the privacy accountant.



\begin{algorithm}
	\caption{\codename Optimization}
	\label{alg:cgd}
	\begin{algorithmic}[1]
		\State{\textbf{Input:} Local training data $\xi_l$ ($l \in [1, m]$), }
		\State{\qquad number of training iterations $T$}
		\State{\textbf{Output:} Confined global model parameters $w_*^l$ ($l \in [1, m]$) }
		\State{\textbf{Initialize:} $k\leftarrow 1$, each participant $l$ randomizes its own $w_1^l$}
		\While{$k \leq T$}
		\State{\textbf{for all} participants $l \in [1, m]$ \textbf{do in parallel}}
		\State{\qquad Compute the local gradient: $g^l(w^l_{k}, \xi_l)$ }
		\State{\qquad Securely evaluate the sum: $\sum\limits_{l=1}^{m}g^l(w^l_{k}, \xi_l)$ }
		\State{\qquad Choose a stepsize: $\alpha_k$}
		\State{\qquad Set the new iterate as: $w_{k+1}^l \leftarrow w^l_{k} - \alpha_k \sum\limits_{l=1}^{m}g^l(w^l_{k}, \xi_l)$}
		\State{\textbf{end for}}
		\State{$k \leftarrow k+1 $}		
		\EndWhile
	\end{algorithmic}
\end{algorithm}

%\paragraph{Remark} Table \ref{tab:differ} summarizes the differences between the traditional federated learning, i.e., \emph{federated SGD/mini-batch}, and our proposed \emph{\short}. We refer \emph{federated SGD/mini-batch} to SGD/mini-batch optimization in the federated learning setting, including plain SGD/mini-batch in which the local gradient/model is shared in plaintext, and  privacy-preserving SGD/mini-batch via secure aggregation or differential privacy mechanisms.

%In addition to the architectural difference as aforementioned, the way of model update also differs.
%\short also differs to the federated SGD/mini-batch
%The differences lie in two aspects.
%(1) In federated SGD, every participant shares/updates the same $w_k$, while  in \short, the global models $w_k^l$ are different, and confined within their corresponding participants $l$. (2)


%The theoretical guarantee of convergence including the bound of difference between \short solution and the centralized solution is discussed in Section \ref{sec:convergence}, and the privacy preservation property achieved by \short is presented in Section \ref{sec:privacy} .

In Section \ref{sec:cgdnn}, we will apply \short optimization, i.e.,  Algorithm \ref{alg:cgd}, to a N-layer neural network. %, with the number of participants $m$ decomposed into $m = (m^h \times m^v)$ (i.e., number of horizontal partitions $\times$ number of vertical partitions).



==> chapters/design1.tex <==
\section{\codename}

\short optimizes an objective function in FL with multiple local datasets.
It starts with a colony of discrete points and uses the combination of their gradients to lead the optimization to another colony of points at the neighborhood of 
the global optimum. %\replace{the optimum of the objective function}{the global optimum}.
%\add{In this section, } 
In this section, we formalize this problem and present the %\replace{process}{workflow}
workflow of \short optimization.


\subsection{Problem formulation}
\label{sec:problem}
Consider a centralized dataset $\xi = \{(x_i, y_i)\}^n_{i=1}$ consisting of $n$ training samples.
%\highlight{The goal of machine learning is to find a model $h(w,x)$ with parameter $w$ that given input $x$, can predict its label $y$ by minimizing the loss between the model prediction $h(w,x_i)$ and its corresponding label $y_i$ over all training samples $i$.}
%baigd{I don't think this is correct}
%\add{The goal of machine learning is to find a model parameter $w$ such that the overall loss, which is measured by the distance between model prediction $h(w,x_i)$ and label $y_i$ for each $(x_i,y_i) \in \xi$, is minimized.}
The goal of machine learning is to find a model parameter $w$ such that the overall loss, which is measured by the distance between the model prediction $h(w,x_i)$ and the label $y_i$ for each $(x_i,y_i) \in \xi$, is minimized.
%\replace{In general, the model is trained by}{This is reduced to }
This is reduced to solving the following problem
%\baigd{argmin}
\begin{equation}
	\arg \min_w \frac{1}{n} \sum_{i=1}^{n} F (w;\xi) + \lambda z(w),
\end{equation}
where $F(w;\xi)$ is the loss function, and $z(w)$ is the regularizer for $w$. We use $w_*$ to denote the optimal solution of centralized training~(i.e., the centralized model).

In the context of FL, we have a system of $m$ local participants, each of which holds a private dataset $\xi_l \subseteq \xi $ $(l \in [1,m])$ %\baigd{$\subseteq$?}
consisting of a part of the training dataset.
The part could be a part of training samples, a part of features that have common entries, or both.
Assume the training takes $T$ iterations, and let $w^l_{k}$ denote the
confined model of participant $l$ at the $k^{th}$ iteration, where $k \in [1,T]$.
Let
\begin{equation}
	\label{equ:gl}
g^l(w^l_{k}, \xi_l)=\frac{1}{|\xi_{l}|}  \nabla F(w^l_{k}, \xi_{l})
\end{equation}
represent the local gradient with respect to $\xi_l$.
We use $w^l_*$ to denote the final confined model of participant $l$ when \short converges.
The objective of \short is to make $w^l_*$ located at a neighborhood of the centralized model $w_*$ within a bounded gap. %\highlight{difference}. \baigd{difference or gap. Unify this throughout the paper}%\baigd{it is the algorithm, not the model, that converges }

\subsection{\short optimization}
%\yanjun{whether we need to detail the horizontal/vertical partitions in the following algorithm?}
\label{sec:optimization}

Figure \ref{fig:differ} illustrates the architecture of \short (Figure \ref{fig:cgd}), with a comparison to the centralized training~(Figure \ref{fig:central}) and traditional FL~(Figure \ref{fig:existing}).
In the centralized training, the datasets of all participants are gathered for training a single model.
In the traditional FL, every participant owns its local training dataset, and updates the \emph{same} global model $w_{k}$ via a parameter server using its local model/gradients.
The local gradients $\nabla F(w_k, \xi_{l,k})$ can be protected via either secure aggregation~\cite{bonawitz2017practical, mohassel2017secureml, zhang2020privcoll,  marc2019privacy, sharma2019confidential, liu2017oblivious} or differential privacy mechanisms~\cite{abadi2016deep, song2013stochastic, shokri2015privacy, dwork2014algorithmic, hu2019fdml, zhang2020differentially}. %\baigd{citations}
This process can be decentralized by replacing the parameter server with a peer-to-peer communication mechanism~\cite{kim2019blockchained, roy2019braintorrent}. %\baigd{citations}
In \short, each participant learns its own confined model~(represented by different colors), i.e., each $w^l_{k}$ %\remove{with respect to participant $l$, denoted by $w^l_{k}$,}\baigd{$w_{k}$ has been defined}
is \emph{different and private}.
The model updating in \short synthesizes the information from all training samples by summing up the local gradients, %allowing each participant to benefit from all other ones,
while in federated SGD~(Figure \ref{fig:existing}), each iteration takes into account only a subset of training samples.

%\baigd{I don't get the footnote here. Too much information. See my writing below this paragraph }
%A summary of differences between the traditional FL, i.e., federated SGD/mini-batch\footnote{We refer federated SGD/mini-batch to SGD/mini-batch optimization in the federated learning setting, including plain SGD/mini-batch in which the local gradient/model is shared in plaintext, and  privacy-preserving SGD/mini-batch via secure aggregation or differential privacy mechanisms.}, and \short is given in Table \ref{tab:differ}. By designing the \short algorithm, we theoretically guarantee that each confined model will converge towards the centralized optimal solution to ensure the model accuracy (column 5 in Table \ref{tab:differ} and detailed in Section \ref{sec:convergence}), and also achieve the desired privacy preservation compared to the traditional FL framework (column 6 in Table \ref{tab:differ} and detailed in Section \ref{sec:privacy}).

To better position \short, we summarize the related studies in the literature in Table~\ref{tab:differ}.
We use federated SGD to represent the SGD or its mini-batch mode %\highlight{mini-batch mode of SGD} \baigd{confirm this, make it consistent with in the intro}
in the FL, including both the plain SGD in which the local gradient/model is shared in plaintext,
and privacy-preserving SGD via secure aggregation or differential privacy mechanisms. %\baigd{if the term is correct, update it in the table}
\short guarantees that each confined model, when \short converges, is at the neighborhood of the centralized model, retaining the model accuracy (column 5 in Table \ref{tab:differ} and proved in Section \ref{sec:convergence}).
It also achieves desired privacy preservation compared to the traditional FL (column 6 in Table \ref{tab:differ} and detailed in Section \ref{sec:privacy}).


%\begin{figure*}[]
%	\begin{minipage}{0.48\textwidth}
%		\centering
%		\subfloat[Centralized Training]{\includegraphics[width=0.5\columnwidth]{fig/central.pdf}\label{fig:central}}
%		\\[3mm]
%		\subfloat[Traditional Federated Learning]{\includegraphics[width=0.9\columnwidth]{fig/existing.pdf}\label{fig:existing}}
%	\end{minipage}
%	\begin{minipage}{0.48\textwidth}
%		\subfloat[\short ]{\includegraphics[width=\columnwidth]{fig/cgd.pdf}\label{fig:cgd}}
%	\end{minipage}
%\label{fig:differ}	
%\caption{Architectural comparison of the centralized training, traditional federated learning, and \short.}
%\end{figure*}


\begin{figure}
		\centering
	\subfloat[Centralized Training]{{\includegraphics[width=5.5cm]{fig/central.pdf} \label{fig:central}}}%
\qquad
	\subfloat[Traditional Federated Learning]{{\includegraphics[width=8cm]{fig/existing.pdf} \label{fig:existing}}}%
	\qquad
	\subfloat[\short ]{{\includegraphics[width=8cm]{fig/cgd.pdf} \label{fig:cgd}}}%
	\caption{Architectural comparison of the centralized training, traditional federated learning, and \short.}%
\label{fig:differ}	
\end{figure}

\begin{table*}[ht]
	\centering
	\resizebox{1\textwidth}{!}{
		\begin{tabular}{|p{0.07\linewidth} | p{0.17\linewidth} | p{0.13\linewidth} | p{0.23\linewidth} |p{0.22\linewidth} |p{0.24\linewidth}|}
			\hline
			\multicolumn{2}{|c|}{\multirow{2}{*}{Technique}}                                         & \multicolumn{2}{c|}{Methodology}                                                                                                                                                                     & \multicolumn{2}{c|}{Desired properties}                                                                                                                                                                                                                                                                                                                           \\ \cline{3-6}
			\multicolumn{2}{|c|}{}                                                                   & Architecture                                                                       & Model update                                                                                            & Model Accuracy                                                                                                                                                                                                      & Privacy                                                                                                                                     \\ \hline
			%\multicolumn{2}{|l|}{Centralized training via batch-GD}                    & All the data are collected centrally to produce the model.                         & Compute the gradient using all the training samples to update the model in each iteration.                      & N/A                                                                                                                                                                                                         & Theoretically guaranteed convergence.                                                                                                               \\ \hline
			\multirow{3}{*}{\shortstack[l]{Federated \\ SGD  }} & Plain SGD~\cite{robbins1951stochastic, bottou2018optimization}                         & \multirow{3}{*}{\shortstack[l]{All the particip-\\ants  jointly  learn\\ one and the same \\ global  model.}} & \multirow{3}{*}{\shortstack[l]{Update the model  using  the \\ gradient  computed on a subset \\ of  training samples  in  each \\ iteration.}} & Theoretically guaranteed convergence~\cite{robbins1951stochastic, bottou2018optimization}.                                                                                    & The sharing of local parameters/gradients is subject to model inversion attack~\cite{melis2019exploiting, fredrikson2015model, shokri2017membership} .                                                                            \\ \cline{2-2} \cline{5-6}
			& Privacy-preserving SGD via secure aggregation~\cite{bonawitz2017practical, mohassel2017secureml, zhang2020privcoll,  marc2019privacy, sharma2019confidential, liu2017oblivious}  &                                                                                    &                                                                                                                 & As above, since the mechanism guarantees that the computation result from ciphertext is the same from plaintext~\cite{bonawitz2017practical,mohassel2017secureml}.& The sharing of one and the same global model (even though the local gradients are protected) is still subject to information leakage (refer to~\cite{nasr2019comprehensive} and Section \ref{sec:privacy}). \\ \cline{2-2} \cline{5-6}
			& Privacy-preserving SGD via differential privacy~\cite{abadi2016deep, song2013stochastic, shokri2015privacy, dwork2014algorithmic, hu2019fdml, zhang2020differentially}  &                                                                                    &                                                                                                                 & Additive noise (in most cases) affects the model accuracy~\cite{dwork2014algorithmic}.                                                                                                    &  The privacy cost is accumulated with repeated accesses to the dataset~\cite{abadi2016deep}.                                                      \\ \hline
			\multicolumn{2}{|l|}{\codename}                                           & Each participant learns and confines a different global model.                     & The model update in each  iteration embraces the information from all the training samples by summing up the local gradients.            & Theoretically guaranteed convergence with bounded gap to the centralized model.                                                                                                                         & Boosted privacy preservation by eliminating the sharing of the global model.                                                    \\ \hline
		\end{tabular}
	}	
	\caption{A summary of differences between the federated SGD and \short.}
	%{A summary of differences between the traditional federated learning, i.e., federated SGD/mini-batch\protect\footnotemark, and \short.}	
	\label{tab:differ}
\end{table*}
%\footnotetext{We refer federated SGD/mini-batch to SGD/mini-batch optimization in the federated learning setting, including plain SGD/mini-batch in which the local gradient/model is shared in plaintext, and  privacy-preserving SGD/mini-batch via secure aggregation or differential privacy mechanisms.}


Algorithm \ref{alg:cgd} outlines \short optimization for training with the confined model $w_k^l$.
In general, the optimization process consists of the following  steps.
\begin{itemize}
\item \textbf{Initialization. } Each  participant $l$ randomizes its own $w_1^l$.
\item \textbf{Step 1. } At each iteration $k$, every participant computes the local gradient $g^l(w^l_{k}, \xi_l)$  with respect to its current confined model $w^l_{k}$ and %\add{current confined model $w^l_{k}$ and} own \remove{private}
own dataset $\xi_l$ using Equation \ref{equ:gl}. %\baigd{this needs equation 4, so what are $n_l$ and $\xi_{l,i}$ w.r.t a participant?}
\item \textbf{Step 2. } Securely compute $\sum\limits_{l=1}^m g^l(w^l_{k}, \xi_l)$ which is later used for %\replace{iterate update}{calculating $w^l_{k+1}$}
calculating $w^l_{k+1}$ (double lines in Figure \ref{fig:cgd}).

%Here, we remark an important difference of model update between \short and SGD/mini-batch. (column 4 in Table \ref{tab:differ}).
%\baigd{this still needs to be synched. How is it different from the synch in FL, and why is it good? Explaining this clearly is the key of this paper. The ``remark'' below should focus on this}

This step presumes that computational tools exist for securely evaluating the sum of a set of secret values to avoid direct release of plain local gradient $g^l(w^l_{k}, \xi_l)$.
We refer to Section \ref{sec:privacy} for more detail.
\item \textbf{Step 3. } A scalar stepsize $\alpha_k > 0$ is chosen given an iteration number $k\in[1,T]$.
\item \textbf{Step 4. } Every participant takes a descent step on its own $w_k^l$ with $\alpha_k \sum\limits_{l=1}^m g^l(w^l_{k}, \xi_l)$, %\add{, i.e., $w_{k+1}^l \leftarrow w_k^l - \alpha_k \sum\limits_{l=1}^m g^l(w^l_{k}, \xi_l)$}.
i.e., $w_{k+1}^l \leftarrow w_k^l - \alpha_k \sum\limits_{l=1}^m g^l(w^l_{k}, \xi_l)$.

\end{itemize}

%At each step of the SGD, we compute the gradient  for a random subset of examples, clip the l2 norm of each gradient, compute the average, add noise in order to protect privacy, and take a step in the opposite direction of this average noisy gradient. At the end, in addition to out- putting the model, we will also need to compute the privacy loss of the mechanism based on the information maintained by the privacy accountant.



\begin{algorithm}
	\caption{\codename Optimization}
	\label{alg:cgd}
	\begin{algorithmic}[1]
		\State{\textbf{Input:} Local training data $\xi_l$ ($l \in [1, m]$), }
		\State{\qquad number of training iterations $T$}
		\State{\textbf{Output:} Confined global model parameters $w_*^l$ ($l \in [1, m]$) }
		\State{\textbf{Initialize:} $k\leftarrow 1$, each participant $l$ randomizes its own $w_1^l$}
		\While{$k \leq T$}
		\State{\textbf{for all} participants $l \in [1, m]$ \textbf{do in parallel}}
		\State{\qquad Compute the local gradient: $g^l(w^l_{k}, \xi_l)$ }
		\State{\qquad Securely evaluate the sum: $\sum\limits_{l=1}^{m}g^l(w^l_{k}, \xi_l)$ }
		\State{\qquad Choose a stepsize: $\alpha_k$}
		\State{\qquad Set the new iterate as: $w_{k+1}^l \leftarrow w^l_{k} - \alpha_k \sum\limits_{l=1}^{m}g^l(w^l_{k}, \xi_l)$}
		\State{\textbf{end for}}
		\State{$k \leftarrow k+1 $}		
		\EndWhile
	\end{algorithmic}
\end{algorithm}

%\paragraph{Remark} Table \ref{tab:differ} summarizes the differences between the traditional federated learning, i.e., \emph{federated SGD/mini-batch}, and our proposed \emph{\short}. We refer \emph{federated SGD/mini-batch} to SGD/mini-batch optimization in the federated learning setting, including plain SGD/mini-batch in which the local gradient/model is shared in plaintext, and  privacy-preserving SGD/mini-batch via secure aggregation or differential privacy mechanisms.

%In addition to the architectural difference as aforementioned, the way of model update also differs.
%\short also differs to the federated SGD/mini-batch
%The differences lie in two aspects.
%(1) In federated SGD, every participant shares/updates the same $w_k$, while  in \short, the global models $w_k^l$ are different, and confined within their corresponding participants $l$. (2)


%The theoretical guarantee of convergence including the bound of difference between \short solution and the centralized solution is discussed in Section \ref{sec:convergence}, and the privacy preservation property achieved by \short is presented in Section \ref{sec:privacy} .

%In Section \ref{sec:cgdnn}, we will apply \short optimization to a N-layer neural network.
%, with the number of participants $m$ decomposed into $m = (m^h \times m^v)$ (i.e., number of horizontal partitions $\times$ number of vertical partitions).

%\baigd{It could be moved here} \yanjun{Let me think about it...}



==> chapters/experiment.tex <==
\section{Experiments}
\label{sec:experiment}
We implement \short algorithms in C++. 
We use Eigen library \cite{eigenweb} to handle matrix operations, and use ZeroMQ library \cite{hintjens2013zeromq} to implement the distributed messaging.
We employ additive  secret sharing scheme~\cite{bogdanov2008sharemind} for securely computing the sum of local gradients. 

We examine the performance of \emph{\short training} compared with \emph{centralized training} and \emph{local training}.
\begin{itemize}
	\item \textbf{\short training.} The model is trained using Algorithm \ref{alg:cgd} on the dataset which is partitioned and distributed to $m$ participants, where $m = (m^h \times m^v)$ (number of horizontal partitions $\times$ number of vertical partitions). %\yanjun{need to explain why $m^v$ is set to 2.} 
	The performance results are then evaluated by a randomly selected participant's confined model on the validation set. 
	\item \textbf{Centralized training (baseline).} We use the performance of centralized training as the baseline. In this setting, the model is trained on the entire dataset using batch update.
	\item \textbf{Local training.} In this setting,  the data and model is also separately owned by $m$ participants, but without using the proposed \short mechanism. That is, each participant separately trains their local models based on their own data partition. %, %(i.e.,  the models are updated using the local gradients only), 
	%and evaluates the model's performance on the validation set.
\end{itemize}

In the following, we report on our evaluation results on two popular datasets: MNIST~ \cite{lecun-mnisthandwrittendigit-2010} and CIFAR-10~\cite{krizhevsky2009learning}.


\subsection{MNIST}
We conduct experiments on the standard MNIST dataset for handwritten digit recognition. 
The dataset has $60,000$ training samples and $10,000$ test samples, each with $784$ features representing $28 \times 28$ pixels in the image. 
We use a  FNN %with 1 hidden layer 
with ReLU of $256$ units and softmax of 10 classes (corresponding to the 10 digits) with cross-entropy loss.

%In the following, we conduct three sets of experiments: the first one uses 
%\paragraph{Baseline}
%Our baseline  model of centralized training reaches  accuracy of $98.30\%$  in $2000$ iterations. 

\subsubsection{\short Optimization with default settings} \hfill\\
\indent Our first set of experiments is conducted to examine the performance of \short training compared with centralized/local training in default settings. 
We set $\mu = 0$ (meaning a fixed learning rate $\alpha$), and
we use  standard weight initialization scheme which sampling from the Gaussian distribution of mean 0 and variance 1 with a default initialization parameter $\delta = 0.1$ (c.f. Equation \ref{equ:delta}). 
The number of training iterations is set to  $T=2000$.

%These three methods are implemented with the same fixed learning rate $\alpha$ (i.e., not diminishes as the iteration increases), and the same training iteration $T=2000$.

\paragraph{Results}
Figure \ref{fig:fixrate}  summarizes the performance for different number of participants. Generally, the results on the validation loss and accuracy of \short stays near to the centralized baseline when the number of participants is growing, and significantly outperforms the local training. 

For example, when $m = (1000 \times 112)$, i.e., each participant owns a different part of dataset that consists of $60$ samples with $7$ features, \short achieves $0.209$ and $93.74\%$ in validation loss and accuracy respectively, which is still near to - $0.081$ and $97.54\%$ - in the centralized baseline, whereas in the local training without \short mechanism, the loss is $2.348$ and the accuracy is merely $11.64\%$ (detailed in Table \ref{tab:fixrate}).

\begin{figure*}[]%
	\centering
	\subfloat[$m=(10 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_10x1_loss.pdf} \label{fig:fixrate_10*1_loss}}}%
	\subfloat[$m=(100 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_100x1_loss.pdf} \label{fig:fixrate_100*1_loss}}}%
	\subfloat[$m=(1000 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x1_loss.pdf} \label{fig:fixrate_1000*1_loss}}}%
\quad
	\subfloat[$m=(10 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_10x1_acc.pdf} \label{fig:fixrate_10*1_acc}}}%
	\subfloat[$m=(100 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_100x1_acc.pdf} \label{fig:fixrate_100*1_acc}}}%
	\subfloat[$m=(1000 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x1_acc.pdf} \label{fig:fixrate_1000*1_acc}}}%
\quad
	\subfloat[$m=(10 \times 7)$]{{\includegraphics[width=5cm]{fig/fixrate_10x7_loss.pdf} \label{fig:fixrate_10*7_loss}}}%
	\subfloat[$m=(100 \times 49)$]{{\includegraphics[width=5cm]{fig/fixrate_100x49_loss.pdf} \label{fig:fixrate_100*49_loss}}}%
	\subfloat[$m=(1000 \times 112)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x112_loss.pdf} \label{fig:fixrate_1000*112_loss}}}%
\quad
	\subfloat[$m=(10 \times 7)$]{{\includegraphics[width=5cm]{fig/fixrate_10x7_acc.pdf} \label{fig:fixrate_10*7_acc}}}%
	\subfloat[$m=(100 \times 49)$]{{\includegraphics[width=5cm]{fig/fixrate_100x49_acc.pdf} \label{fig:fixrate_100*49_acc}}}%
	\subfloat[$m=(1000 \times 112)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x112_acc.pdf} \label{fig:fixrate_1000*112_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for different number of participants on the MNIST dataset.}%
	\label{fig:fixrate}
\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\begin{table}[H]
%	\caption{Performance with default settings.}
%	\label{tab:fixrate}
%	\begin{tabular}{|l|l|l|l|l|}
%		\hline
%		\multirow{2}{*}{}                & \multicolumn{2}{l|}{Validation loss}   & \multicolumn{2}{l|}{Validation accuracy} \\ \cline{2-5} 
%		& \short  & Local training & \short  & Local training  \\ \hline
%		m=($10 \times 2$)   & 0.143                 & 0.278          & 95.6\%                  & 92\%            \\ \hline
%		m=($100 \times 2$)  & 0.188                 & 0.549          & 94.22\%                 & 82.89\%          \\ \hline
%		m=($1000 \times 2$) & 0.208                 & 1.566     & 93.76\%                 & 50.11\%          \\ \hline
%	\end{tabular}
%\end{table}

\begin{table}[H]
	\caption{Performance comparison on MNIST with default settings.}
	\label{tab:fixrate}
\begin{tabular}{|l|l|l|l|l|}
	\hline
	& \multicolumn{2}{c|}{Validation loss} & \multicolumn{2}{c|}{Validation accuracy} \\ \hline
	Centralized        & \multicolumn{2}{c|}{0.081}           & \multicolumn{2}{c|}{97.54\%}             \\ \hline \hline
	& \short             & Local training           & \short               & Local training              \\ \hline
	m=($10 \times 1$)   & 0.143             & 0.278            & 95.6\%              & 92\%               \\ \hline
	m=($10 \times 7$)   & 0.143             & 1.283            & 95.6\%              & 54.39\%               \\ \hline
	m=($100 \times 1$)  & 0.188             & 0.549            & 94.22\%             & 82.89\%            \\ \hline
	m=($100 \times 49$)  & 0.189             & 2.076            & 94.21\%             & 23.53\%            \\ \hline
	m=($1000 \times 1$) & 0.208             & 1.566            & 93.76\%             & 50.11\%            \\ \hline
	m=($1000 \times 112$) & 0.209             & 2.348            & 93.74\%             & 11.64\%            \\ \hline
\end{tabular}
\end{table}


\subsubsection{Role of the initialization}\hfill\\
\label{sec:init}
\indent According to Theorem \ref{theorem:main}, the maximum gap between \short solution and the centralized optimum is bounded by  $\epsilon = m \| \displaystyle \mathop{\mathbb{E}}_{j\in m^h}(w_1^l-w_1^j)\|$, and the range of each  $w_1^l$ is decided by $\delta$ in Equation \ref{equ:delta}. Therefore, in this set of experiment, we investigate how different initialization settings affect the \short performance. 

To demonstrate the effects of initialization, we manipulate the parameter $\delta$ individually, and keep the other settings as default (i.e., $\mu = 0$ and $T=2000$). 

In our first setting, we let all participants use the same $\delta$ in $(0.1, 0.06, 0.01, 0.001)$, to investigate the impact of this parameter on the model accuracy. 
Then, in our second setting, we let each participant confine the parameter and randomly select its own $\delta$ based on the uniform distribution within the range from $0.001$ to $0.1$.

\paragraph{Results}
Figure \ref{fig:init} shows the results of our first setting. Generally, by decreasing $\delta$ appropriately (which reducing the value of $ \| \displaystyle \mathop{\mathbb{E}}_{j\in m^h}(w_1^l-w_1^j)\|$), \short achieves better performance (meaning that it is further approaching to the centralized optimum). 
For example, with $m = (1000 \times 112)$ participants, the validation accuracy and loss achieves $97.08\%$ and $0.096$ with $\delta = 0.01$ which outperforms $93.74\%$ and $0.209$  in the default setting of $\delta = 0.1$, and very close to the centralized optimum in which the validation accuracy and loss are $97.61\%$ and $0.078$ respectively. 

However, one cannot set $\delta$ too small as the choice of initialization can be crucial for maintaining numerical stability in neural network~\cite{glorot2010understanding}. For example, if we depress $\delta$ to $0.001$, as shown in the last column of Table \ref{tab:init},  the overall performance is decreased even though the gap between the centralized optimum and \short solution is further closer.

Figure \ref{fig:initrandom} shows the results of our second setting. 
The performance of \short in this setting still closely approaches the centralized optimum with $\delta$ selected uniformly at random by each participant. 
For example,  with $m = (1000 \times 112)$ participants, \short achieves $95.82\%$ and $0.136$ in the validation accuracy and loss respectively. 

The detail report of performance with different setting of $\delta$ for different number of participants is given in Table \ref{tab:init}.

\begin{figure}[]%
	\centering
	\subfloat[Validation loss]{{\includegraphics[width=4.5cm]{fig/Init_1000_loss.pdf} \label{fig:Init_1000_loss}}}%
	\subfloat[Validation accuracy]{{\includegraphics[width=4.5cm]{fig/Init_1000_acc.pdf} \label{fig:Init_1000_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for different initialization parameter $\delta$ with $m = (1000 \times 112)$ on the MNIST dataset.}%
	\label{fig:init}
\end{figure}

\begin{figure}[]%
	\centering
	\subfloat[Validation loss]{{\includegraphics[width=4.5cm]{fig/Init_random_loss.pdf} \label{fig:Init_random_loss}}}%
	\subfloat[Validation accuracy]{{\includegraphics[width=4.5cm]{fig/Init_random_acc.pdf} \label{fig:Init_random_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for various number of participants with $\delta$ selected uniformly at random on the MNIST dataset.}%
	\label{fig:initrandom}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
	\centering
	\caption{Performance with different initialization parameter $\delta$ for different number of participants on the MNIST dataset.}
	\label{tab:init}
	\resizebox{0.51\textwidth}{!}{
	\begin{tabular}{|l|l|l|l|l||l|}
		\hline
		\multicolumn{6}{|c|}{Validation loss}                                                            \\ \hline
		& $\delta=0.1$   & $\delta=0.06$  & $\delta=0.01$  & $\delta=0.001$     & \multirow{2}{*}{Random}                      \\ \cline{1-5}
		Centralized & 0.080 & 0.074  & 0.078  & 0.111      &                    \\ \hline
		m=($10 \times 7$)    & 0.143 & 0.106 & 0.092 & 0.121      & 0.110                   \\ \hline
		m=($100 \times 49$)   & 0.188 & 0.125 & 0.094 & 0.129     & 0.124                    \\ \hline
		m=($1000 \times 112$)   & 0.209 & 0.132 & 0.096 & 0.117 & 0.136\\ \hline\hline
		\multicolumn{6}{|c|}{Validation accuracy}                                                        \\ \hline
		& $\delta=0.1$   & $\delta=0.06$  & $\delta=0.01$  & $\delta=0.001$     & \multirow{2}{*}{Random}                      \\ \cline{1-5}
		Centralized & 97.54\%    & 97.79\%    & 97.61\%    & 96.69\%      &                       \\ \hline
		m=($10 \times 7$)    & 95.60\%    & 96.72\%    & 97.21\%    & 96.38\%       & 96.59\%                     \\ \hline
		m=($100 \times 49$)   & 94.22\%    & 96.05\%    & 97.15\%    & 96.19\%     & 96.13\%                       \\ \hline
		m=($1000 \times 112$)   & 93.74\%    & 95.91\%    & 97.08\%    & 96.59\%     & 95.82\%                       \\ \hline
	\end{tabular}
}
\end{table}


\subsubsection{Effect of the parameter $\mu$}\hfill\\
\label{sec:mu}
\indent Our third set of experiments is conducted to demonstrate the effect of parameter $\mu$, which affects the convergence speed.
In this experiment, we adjust the parameter $\mu$ individually, and keep $\delta$ fixed as default (i.e., $ \delta = 0.1$).

As each time the stepsize is diminished, more the number of iterations are required. Therefore, for practical purpose, we  begin by running \short with a fixed $\alpha$ until it (approximately) reaches a preferred point, and starting with $\alpha_1=\alpha$.

\paragraph{Results}
Figure \ref{fig:mu} demonstrates heuristic results with different $\mu$ for ($100 \times 49$) and ($1000 \times 112$) participants. We run the first $6000$ iterations with a fixed $\alpha$, and  then diminish $\alpha_k$ in each of the following $8000$ iterations. 

As shown in Figure \ref{fig:mu_100_acc}, for training with ($100 \times 49$) participants, $\mu \geq 0.01$ gives a faster speed which reaches the optimal solution with validation accuracy $95.9\%$ at $11401^{th}$ iteration, $2500$ iterations faster than training with $\mu < 0.01$. For ($1000 \times 112$) participants (Figure \ref{fig:mu_1000_acc}), empirical results show that training with $\mu > 0.05$ reaches the highest validation accuracy of $95.68\%$ at $11821^{th}$ iteration, which is $2140$ iterations faster than training with $\mu \leq 0.05$.

 
\begin{figure}[]%
	\centering
	\subfloat[m=($100 \times 49$)]{{\includegraphics[width=5cm]{fig/mu_100_acc.pdf} \label{fig:mu_100_acc}}}%
	\subfloat[m=($1000 \times 112$)]{{\includegraphics[width=4.5cm]{fig/mu_1000_acc.pdf} \label{fig:mu_1000_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Validation accuracy with different parameter $\mu$ for different number of participants on the MNIST dataset.}%
	\label{fig:mu}
\end{figure}

\subsection{CIFAR-10}
\begin{figure*}[]%
	\centering
	\subfloat[$m=(10 \times 2)$]{{\includegraphics[width=5cm]{fig/cifar_10_loss.pdf} \label{fig:cifar_10_loss}}}%
	\subfloat[$m=(100 \times 16)$]{{\includegraphics[width=5cm]{fig/cifar_100_loss.pdf} \label{fig:cifar_100_loss}}}%
	\subfloat[$m=(1000 \times 32)$]{{\includegraphics[width=5cm]{fig/cifar_1000_loss.pdf} \label{fig:cifar_1000_loss}}}%
	\quad
	\subfloat[$m=(10 \times 2)$]{{\includegraphics[width=5cm]{fig/cifar_10_acc.pdf} \label{fig:cifar_10_acc}}}%
	\subfloat[$m=(100\times 16)$]{{\includegraphics[width=5cm]{fig/cifar_100_acc.pdf} \label{fig:cifar_100_acc}}}%
	\subfloat[$m=(1000 \times 32)$]{{\includegraphics[width=5cm]{fig/cifar_1000_acc.pdf} \label{fig:cifar_1000_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for different number of participants on the CIFAR-10 dataset.}%
	\label{fig:cifar}
\end{figure*}

We also conduct experiments on the CIFAR-10 dataset, which consists of 60000 $32 \times 32$ colour images in 10 classes (e.g., airplane, bird, cat, etc), with 6000 images per class. There are 50000 training images and 10000 test images. The CIFAR-100 dataset is just like the CIFAR-10, except it has 100 classes containing 600 images each. There are 500 training images and 100 testing images per class. 

We use the ResNet-56 architecture proposed by He, et al.~\cite{he2016deep}. The network inputs are $32 \times 32$ images, with the per-pixel mean subtracted. The first layer is $3 \times 3$ convolutions. Then a stack of $3 \times 18$ layers is used, with $3 \times 3$ convolutions of filter sizes $\{32, 16, 8\}$ respectively, and $18$ layers for each size. The numbers of filters are $\{16, 32, 64\}$ respectively. The network ends with an  average pooling layer, a fully-connected (FC) layer with $1024$ units, and softmax.

The training data augumentation in our implementation follows the setting in~\cite{he2016deep}. For each training image, we generate a new distorted image by randomly flipping the image horizontally with probability $0.5$, and adding 4 amounts of padding to all sides before cropping the image to $32 \times 32$.

Since our focus is on the behaviors of proposed \short, but not on pushing the state-of-the-art results on CIFAR-10, we follow the experiment setting of the related work~\cite{abadi2016deep} which utilizes the transferability~\footnote{By transfer learning, one can take a model trained on one dataset and transfer it to another one without retraining~\cite{shin2016deep}.} of convolutional layers to save the computational overhead of computing per-example gradients.                        
We treat the CIFAR-10 as the private dataset and CIFAR-100 as a public dataset. 
We use CIFAR-100 to train a network with the aforementioned network architecture. 
We then freeze the model parameters of early convolutional layers  learned from CIFAR-100 and retrain only the last FC layer  on CIFAR-10 with the same architecture.  
Training on the entire dataset with batch update gives us $75.75\%$ validation accuracy, which is our centralized training baseline\footnote{We should note that by making the network deeper or using other advanced techniques, significantly better accuracy can be obtained, with the state-of-the-art being about 99.37\%~\cite{kolesnikov2019big}.}.

For the \short training, every participant solely feeds the pre-trained convolutional layers with their private data partitions, generates the input features of the FC layer, and randomly initializes the confined model parameters of the FC layer. Then, treating  the input features of the FC layer as the private local training data $\xi_l$ and training with Algorithm \ref{alg:cgd} with $\delta = 0.01$ and $T=6000$ gives the  results of \short optimization.



\paragraph{Results}
Figure \ref{fig:cifar} and Table \ref{tab:cifar}  summarizes the performance on CIFAR-10. The results on the validation loss and accuracy of \short on CIFAR-10 are consistent to the MNIST dataset. 

For example, when $m = (1000 \times 32)$, \short achieves $0.724$ and $74.29\%$ in validation loss and accuracy respectively, which is relatively near to - $0.675$ and $75.72\%$ - in the centralized baseline, whereas in the local training, the loss is $2.434$ and the accuracy is  $16.19\%$ .


\begin{table}[H]
	\caption{Performance comparison on CIFAR-10.}
	\label{tab:cifar}
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		& \multicolumn{2}{c|}{Validation loss} & \multicolumn{2}{c|}{Validation accuracy} \\ \hline
		Centralized         & \multicolumn{2}{c|}{0.675}           & \multicolumn{2}{c|}{75.72\%}             \\ \hline \hline
		& \short             & Local training           & \short               & Local training              \\ \hline
		m=($10 \times 2$)   & 0.720             & 0.980            & 74.79\%              & 65.3\%               \\ \hline
		m=($100 \times 16$)  & 0.723             & 2.008            & 74.42\%             & 26.25\%            \\ \hline
		m=($1000 \times 32$) & 0.724             & 2.434            & 74.29\%             & 16.19\%            \\ \hline
	\end{tabular}
\end{table}



==> chapters/experiment1.tex <==
\section{Experiments} \label{sec:experiment}

We implement \short and evaluate its performance in terms of XXX  on two popular benchmark datasets: MNIST~ \cite{lecun-mnisthandwrittendigit-2010} and CIFAR-10~\cite{krizhevsky2009learning}.
We use C++ in our implementation, and use Eigen library \cite{eigenweb} to handle matrix operations and ZeroMQ library \cite{hintjens2013zeromq} for distributed messaging.
%\highlight{We employ additive secret sharing scheme~\cite{bogdanov2008sharemind} for securely computing the sum of local gradients.} \baigd{This has been given in the design section. No need to mention it again here unless you want to talk about implementation issues like which library is used.}

We compare the performance of \short with the training on aggregated data~(referred to as the \emph{centralized training}) and the training on merely each participant's local data~(referred to as the \emph{local training}).
\short is expected to significantly outperform the local training, and approach the performance of the centralized training. 
The settings of all trainings are listed below.
\begin{itemize}
	\item \textbf{\short training.} The model is trained using Algorithm \ref{alg:cgd} on the dataset which is partitioned and distributed to $m$ participants, where $m = (m^h \times m^v)$ (number of horizontal partitions multiplied by number of vertical partitions). %\yanjun{need to explain why $m^v$ is set to 2.}
	\highlight{The performance results are then evaluated by a randomly selected participant's confined model on the validation set.} \baigd{only one confined model is selected? If so, try ``Due to symmetricity, the reported performance data in this section is collected from one randomly selected participant.''}
	\item \textbf{Centralized training}~(the baseline). We take the performance of centralized training as the baseline. In this setting, the training is on the entire dataset using the batch update.
	\item \textbf{Local training.} In this setting, the data and model are distributed to $m$ participants in the same way as in \short. 
 Each participant separately trains their local models from their local data, without sharing the gradients. 
\end{itemize}


\subsection{MNIST}
Our first set of experiments are conducted on the standard MNIST dataset which is a benchmark for handwritten digit recognition.
It has $60,000$ training samples and $10,000$ test samples, each with $784$ features representing $28 \times 28$ pixels in the image.
We use a fully-connect neural network (FNN) %\baigd{full name} %with 1 hidden layer
with ReLU of $256$ units and softmax of 10 classes (corresponding to the 10 digits) with cross-entropy loss.

In the following, we first conduct our experiment in the default settings (Section \ref{sec:default}). We set $\mu = 0$ (meaning a fixed learning rate $\alpha$), and
use the standard weight initialization scheme based on the Gaussian distribution of mean 0 and variance 1 with a default initialization parameter $\delta = 0.1$ (cf. Equation \ref{equ:delta}).
The number of training iterations is set to  $T=2000$.
Then, we investigate the effects of hyper-parameters in \short in Section \ref{sec:init} and Section \ref{sec:mu}. A comparison of the performance of \short and the traditional FL via differential privacy in given in Section \ref{sec:comparedp}.
%In the following, we conduct three sets of experiments: the first one uses
%\paragraph{Baseline}
%Our baseline  model of centralized training reaches  accuracy of $98.30\%$  in $2000$ iterations.

\subsubsection{\short with default settings}  \label{sec:default}
%\baigd{I don't think the default setting has been introduced} 
We first examine the performance of \short against both centralized and local trainings in default settings.


%These three methods are implemented with the same fixed learning rate $\alpha$ (i.e., not diminishes as the iteration increases), and the same training iteration $T=2000$.

%\paragraph{Results}
Figure \ref{fig:fixrate}  summarizes the performance when the number of participants varies. 
In general, \short stays close to the centralized baseline in both validation loss and accuracy, and as expected, significantly outperforms the local training.
%\replace{For example, in the case of $m = (1000 \times 112)$}{In the worst case of $m = (1000 \times 112)$ when \short contains the greatest number of participants}, i.e., \replace{each participant owns a different part of the dataset that consists of $60$ samples with $7$ features}{each participant owns a small proportion consisting of $60$ samples with $7$ features},\baigd{ambiguous} \short \add{still} 
In the worst case of $m = (1000 \times 112)$ when \short contains the greatest number of participants, i.e.,  each participant owns a small proportion consisting of $60$ samples with $7$ features, \short still achieves $0.209$ and $93.74\%$ in validation loss and accuracy respectively, close to $0.081$ and $97.54\%$ of the centralized baseline.  In contrast, the performance of local training declines to $2.348$ and $11.64\%$. In Table \ref{tab:fixrate}, we list the detailed performance comparison.

\begin{figure*}[]%
	\centering
	\subfloat[$m=(10 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_10x1_loss.pdf} \label{fig:fixrate_10*1_loss}}}%
	\subfloat[$m=(100 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_100x1_loss.pdf} \label{fig:fixrate_100*1_loss}}}%
	\subfloat[$m=(1000 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x1_loss.pdf} \label{fig:fixrate_1000*1_loss}}}%
\quad
	\subfloat[$m=(10 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_10x1_acc.pdf} \label{fig:fixrate_10*1_acc}}}%
	\subfloat[$m=(100 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_100x1_acc.pdf} \label{fig:fixrate_100*1_acc}}}%
	\subfloat[$m=(1000 \times 1)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x1_acc.pdf} \label{fig:fixrate_1000*1_acc}}}%
\quad
	\subfloat[$m=(10 \times 7)$]{{\includegraphics[width=5cm]{fig/fixrate_10x7_loss.pdf} \label{fig:fixrate_10*7_loss}}}%
	\subfloat[$m=(100 \times 49)$]{{\includegraphics[width=5cm]{fig/fixrate_100x49_loss.pdf} \label{fig:fixrate_100*49_loss}}}%
	\subfloat[$m=(1000 \times 112)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x112_loss.pdf} \label{fig:fixrate_1000*112_loss}}}%
\quad
	\subfloat[$m=(10 \times 7)$]{{\includegraphics[width=5cm]{fig/fixrate_10x7_acc.pdf} \label{fig:fixrate_10*7_acc}}}%
	\subfloat[$m=(100 \times 49)$]{{\includegraphics[width=5cm]{fig/fixrate_100x49_acc.pdf} \label{fig:fixrate_100*49_acc}}}%
	\subfloat[$m=(1000 \times 112)$]{{\includegraphics[width=5cm]{fig/fixrate_1000x112_acc.pdf} \label{fig:fixrate_1000*112_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for different number of participants on the MNIST dataset.}%
	\label{fig:fixrate}
\end{figure*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\begin{table}[H]
%	\caption{Performance with default settings.}
%	\label{tab:fixrate}
%	\begin{tabular}{|l|l|l|l|l|}
%		\hline
%		\multirow{2}{*}{}                & \multicolumn{2}{l|}{Validation loss}   & \multicolumn{2}{l|}{Validation accuracy} \\ \cline{2-5}
%		& \short  & Local training & \short  & Local training  \\ \hline
%		m=($10 \times 2$)   & 0.143                 & 0.278          & 95.6\%                  & 92\%            \\ \hline
%		m=($100 \times 2$)  & 0.188                 & 0.549          & 94.22\%                 & 82.89\%          \\ \hline
%		m=($1000 \times 2$) & 0.208                 & 1.566     & 93.76\%                 & 50.11\%          \\ \hline
%	\end{tabular}
%\end{table}

\begin{table}[t]
	\caption{Performance comparison on MNIST with default settings.}
	\label{tab:fixrate}
\begin{tabular}{|l|l|l|l|l|}
	\hline
	& \multicolumn{2}{c|}{Validation loss} & \multicolumn{2}{c|}{Validation accuracy} \\ \hline
	Centralized        & \multicolumn{2}{c|}{0.081}           & \multicolumn{2}{c|}{97.54\%}             \\ \hline \hline
	& \short             & Local training           & \short               & Local training              \\ \hline
	m=($10 \times 1$)   & 0.143             & 0.278            & 95.6\%              & 92\%               \\ \hline
	m=($10 \times 7$)   & 0.143             & 1.283            & 95.6\%              & 54.39\%               \\ \hline
	m=($100 \times 1$)  & 0.188             & 0.549            & 94.22\%             & 82.89\%            \\ \hline
	m=($100 \times 49$)  & 0.189             & 2.076            & 94.21\%             & 23.53\%            \\ \hline
	m=($1000 \times 1$) & 0.208             & 1.566            & 93.76\%             & 50.11\%            \\ \hline
	m=($1000 \times 112$) & 0.209             & 2.348            & 93.74\%             & 11.64\%            \\ \hline
\end{tabular}
\end{table}


\subsubsection{Role of the initialization} \label{sec:init} 
According to Theorem \ref{theorem:main}, the maximum gap between \short solution and the centralized model %\highlight{centralized optimum}\baigd{centralized model?} 
is bounded by  $\epsilon = m \| \displaystyle \mathop{\mathbb{E}}_{j\in m}(w_1^l-w_1^j)\|$, %\baigd{I just noticed this: what is $j$? Basically what does $j\in m^h$ mean? Also check it in Theorem 1.} 
where the scale %\baigd{what does range mean here?} 
of each  $w_1^l$ is decided by $\delta$ in Equation \ref{equ:delta}. Therefore, we investigate how the initialization setting affects \short's performance.

To this end, we conduct two experiments in which we mutate parameter $\delta$ while keeping other settings unchanging~(i.e., $\mu = 0$ and $T=2000$). 
In the first experiment, we let all participants use the same $\delta$ in $\{0.1, 0.06, 0.01, 0.001\}$, as they are  within a reasonable range around $\frac{1}{\sqrt 60000}$. %(where $n$ is the sample size of $60000$) which is the  commonly used to calibrate the scale of initial weights.  %used in \baigd{which are the setting commonly used in existing ...} 
In the other experiment, we let each participant randomly select its own $\delta$ based on the uniform distribution within the range from $0.001$ to $0.1$.

The results of our first experiment are shown in Figure~\ref{fig:init} and the first five columns in Table~\ref{tab:init}. 
In general, as $\delta$ decreases, \short achieves better performance. 
This confirms our expectation: decreasing $\delta$ would reduce the value of $ \| \displaystyle \mathop{\mathbb{E}}_{j\in m^h}(w_1^l-w_1^j)\|$, such that the confined models are closer to the centralized optimum.
We have not observed significant difference from $\delta=0.1$, $0.06$ and $0.01$. 
In the case of $m = (1000 \times 112)$, the validation accuracy and loss achieves $97.08\%$ and $0.096$ with $\delta = 0.01$ which outperforms $93.74\%$ and $0.209$ in the setting of $\delta = 0.1$, but both are close to the centralized model whose validation accuracy and loss are $97.61\%$ and $0.078$ respectively.
However, $\delta$ cannot be set too small, in order to maintain numerical stability in neural network~\cite{glorot2010understanding}. 
For example, when we lower $\delta$ to $0.001$, the performance starts decreasing.  


The results of our second experiment are shown in Figure \ref{fig:initrandom} and the last column in Table~\ref{tab:init}.
We find that when the participants uniformly randomize their $\delta$s from $0.001$ to $0.1$, 
the performance of \short is still comparable with the centralized mode. 
For example, with $m = (1000 \times 112)$ participants, \short achieves $95.82\%$ and $0.136$ in the validation accuracy and loss respectively.
This suggests that \short keeps robust when the $\delta$s of its participants differ by two orders of magnitude. 

\begin{figure}[]%
	\centering
	\subfloat[Validation loss]{{\includegraphics[width=4.5cm]{fig/Init_1000_loss.pdf} \label{fig:Init_1000_loss}}}%
	\subfloat[Validation accuracy]{{\includegraphics[width=4.5cm]{fig/Init_1000_acc.pdf} \label{fig:Init_1000_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for different initialization parameter $\delta$ with $m = (1000 \times 112)$ on the MNIST dataset.}%
	\label{fig:init}
\end{figure}

\begin{figure}[]%
	\centering
	\subfloat[Validation loss]{{\includegraphics[width=4.5cm]{fig/Init_random_loss.pdf} \label{fig:Init_random_loss}}}%
	\subfloat[Validation accuracy]{{\includegraphics[width=4.5cm]{fig/Init_random_acc.pdf} \label{fig:Init_random_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for various number of participants with $\delta$ selected uniformly at random on the MNIST dataset.}%
	\label{fig:initrandom}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
	\centering
	\caption{Performance with different initialization parameter $\delta$ for different number of participants on the MNIST dataset.}
	\label{tab:init}
	\resizebox{0.51\textwidth}{!}{
	\begin{tabular}{|l|l|l|l|l||l|}
		\hline
		\multicolumn{6}{|c|}{Validation loss}                                                            \\ \hline
		& $\delta=0.1$   & $\delta=0.06$  & $\delta=0.01$  & $\delta=0.001$     & \multirow{2}{*}{Random}                      \\ \cline{1-5}
		Centralized & 0.080 & 0.074  & 0.078  & 0.111      &                    \\ \hline
		m=($10 \times 7$)    & 0.143 & 0.106 & 0.092 & 0.121      & 0.110                   \\ \hline
		m=($100 \times 49$)   & 0.188 & 0.125 & 0.094 & 0.129     & 0.124                    \\ \hline
		m=($1000 \times 112$)   & 0.209 & 0.132 & 0.096 & 0.117 & 0.136\\ \hline\hline
		\multicolumn{6}{|c|}{Validation accuracy}                                                        \\ \hline
		& $\delta=0.1$   & $\delta=0.06$  & $\delta=0.01$  & $\delta=0.001$     & \multirow{2}{*}{Random}                      \\ \cline{1-5}
		Centralized & 97.54\%    & 97.79\%    & 97.61\%    & 96.69\%      &                       \\ \hline
		m=($10 \times 7$)    & 95.60\%    & 96.72\%    & 97.21\%    & 96.38\%       & 96.59\%                     \\ \hline
		m=($100 \times 49$)   & 94.22\%    & 96.05\%    & 97.15\%    & 96.19\%     & 96.13\%                       \\ \hline
		m=($1000 \times 112$)   & 93.74\%    & 95.91\%    & 97.08\%    & 96.59\%     & 95.82\%                       \\ \hline
	\end{tabular}
}
\end{table}


\subsubsection{Effect of the parameter $\mu$} \label{sec:mu}
According to Theorem \ref{theorem:main}, the convergence speed of \short is affected by the parameter $\mu$. 
We thus conduct an experiment to investigate this relation. 
In this experiment, we adjust $\mu$ while keeping $\delta$ fixed as $0.1$ as our previous experiments show that \short performs the best in this setting~(cf. Table \ref{tab:init}).
For the stepsize~($\alpha_k$), we run \short with a fixed $\alpha$ till it (approximately) reaches a preferred point, and then continue our experiment with $\alpha_1=\alpha$.
This is to keep \short practical, as each time the stepsize is diminished, more iterations are required. 
Therefore, the first $6000$ iterations is run with $\alpha= 0.01$, %\baigd{put a concrete value}, 
and then diminish $\alpha_k$ in each of the following $8000$ iterations.


%As each time the stepsize is diminished, more the number of iterations are required. Therefore, for practical purpose, we  begin by running \short with a fixed $\alpha$ until it (approximately) reaches a preferred point, and starting with $\alpha_1=\alpha$.

%We enumerate $\mu$ from $0.01$ to $0.9$. 
Figure \ref{fig:mu} demonstrates the results with varying $\mu$ for $m=(100 \times 49)$ and $m=(1000 \times 112)$. 
For the case of $m=(100 \times 49)$, $\mu \geq 0.01$ gives a faster speed. 
\short converges with validation accuracy $95.9\%$ at $11401^{th}$ iteration, $2500$ iterations faster than training with $\mu < 0.01$.  
For the case of $m=1000 \times 112)$, $\mu > 0.05$ gives a faster speed. 
\short converges with validation accuracy $95.68\%$ at $11821^{th}$ iteration, $2140$ iterations faster than training with $\mu \leq 0.05$.

We note that although one can adjust convergence speed by tuning $\mu$, its effect in practice is relatively limited. The gain of the validation accuracy is only within $0.2\%$ in the cost of around $2000$ iterations.  

%Nevertheless, \short will converge to has limited effect for \short used in practice. 
%\baigd{two concerns: 1) where are the boundaries 0.01 and 0.05 from; 2) what implications by this result}

\begin{figure}[]%
	\centering
	\subfloat[m=($100 \times 49$)]{{\includegraphics[width=5cm]{fig/mu_100_acc.pdf} \label{fig:mu_100_acc}}}%
	\subfloat[m=($1000 \times 112$)]{{\includegraphics[width=4.5cm]{fig/mu_1000_acc.pdf} \label{fig:mu_1000_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Validation accuracy with different parameter $\mu$ for different number of participants on the MNIST dataset.}%
	\label{fig:mu}
\end{figure}
\subsubsection{Comparison with the traditional FL via differential privacy} \label{sec:comparedp}
Table \ref{tab:dpmnist} summarizes the performance comparison between \short and the traditional FL via differential privacy mechanism on the MNIST dataset~\cite{abadi2016deep}.
Due to the different setting of network architecture and hyper-parameters, the centralized baseline in our work is slightly different to ~\cite{abadi2016deep}\footnote{The centralized baseline of validation accuracy on the MNIST in ~\cite{abadi2016deep} is 98.3\%.}. Therefore, we use the difference of validation  accuracy to the centralized baseline as the comparison metric.
\short's performance in the comparison is from the results of second experiment in Section \ref{sec:init}, where the $\delta$s of its participants differ by two orders of magnitude, as this setting avoids the leaking about the average distance among the confined models which is recommended in practice for boosted privacy preservation.

\short outperforms the traditional FL as is shown. In the worst case of $m = (1000 \times 112)$, the  difference of validation  accuracy to the centralized baseline in \short is $1.72\%$, while in the traditional FL, such difference in the setting of large noise level is $8.3\%$.
\begin{table}
	\centering
\caption{Comparison between \short and traditional FL via differential privacy in terms of the difference of validation  accuracy to the centralized baseline on MNIST.}
\label{tab:dpmnist}
	\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
	\hline
	\multicolumn{2}{|c|}{\short}               & \multicolumn{2}{c|}{Traditional FL via DP~\cite{abadi2016deep}}             \\ \hline
	Participants & \shortstack[l]{Difference \\to the baseline} & Noise levels                                & \shortstack[l]{Difference \\to the baseline} \\ \hline
	m=($10 \times 7$)            & 0.95\%                     & $\epsilon = 8$ (small noise)   & 1.3\%                      \\ \hline
	m=($100 \times 49$)           & 1.41\%                     & $\epsilon = 2$ (medium noise)  & 3.3\%                      \\ \hline
	m=($1000 \times 112$)            & 1.72\%                     & $\epsilon = 0.5$ (large noise) & 8.3\%                      \\ \hline
\end{tabular}
}
\end{table}

\subsection{CIFAR-10}
\begin{figure*}[]%
	\centering
	\subfloat[$m=(10 \times 2)$]{{\includegraphics[width=5cm]{fig/cifar_10_loss.pdf} \label{fig:cifar_10_loss}}}%
	\subfloat[$m=(100 \times 16)$]{{\includegraphics[width=5cm]{fig/cifar_100_loss.pdf} \label{fig:cifar_100_loss}}}%
	\subfloat[$m=(1000 \times 32)$]{{\includegraphics[width=5cm]{fig/cifar_1000_loss.pdf} \label{fig:cifar_1000_loss}}}%
	\quad
	\subfloat[$m=(10 \times 2)$]{{\includegraphics[width=5cm]{fig/cifar_10_acc.pdf} \label{fig:cifar_10_acc}}}%
	\subfloat[$m=(100\times 16)$]{{\includegraphics[width=5cm]{fig/cifar_100_acc.pdf} \label{fig:cifar_100_acc}}}%
	\subfloat[$m=(1000 \times 32)$]{{\includegraphics[width=5cm]{fig/cifar_1000_acc.pdf} \label{fig:cifar_1000_acc}}}%
	%
	%\vspace{-10pt}
	\caption{Results on the validation loss and accuracy for different number of participants on the CIFAR-10 dataset.}%
	\label{fig:cifar}
\end{figure*}

We also conduct experiments on the CIFAR-10 dataset. 
It consists of 60000 $32 \times 32$ colour images in 10 classes (e.g., airplane, bird, and cat), with 6000 images per class. 
The images are divided into 50000 training images and 10000 test images. 

We use the ResNet-56 architecture proposed by He et al.~\cite{he2016deep}.
It takes as input images of size $32 \times 32$, with the per-pixel mean subtracted. 
Its first layer is $3 \times 3$ convolutions, and then a stack of $3 \times 18$ layers is used, with $3 \times 3$ convolutions of filter sizes $\{32, 16, 8\}$ respectively, and $18$ layers for each filter size.
The numbers of filters are $\{16, 32, 64\}$ in each stack. %\highlight{The numbers of filters are $\{16, 32, 64\}$ respectively. } \baigd{I don't get this sentence}
The network ends with an  average pooling layer, a fully-connected (FC) layer with $1024$ units, and softmax.

Our training data augmentation follows the setting in~\cite{he2016deep}. 
For each training image, we generate a new distorted image by randomly flipping the image horizontally with probability $0.5$, and adding 4 amounts of padding %\highlight{4 amounts of padding}{4 paddings?} 
to all sides before cropping the image to the size of $32 \times 32$.

Since our focus is on evaluating the proposed \short, rather than enhancing the state-of-the-art analysis on CIFAR-10,
we utilize the transferability\footnote{Transfer learning allows the analyst to take a model trained on one dataset and transfer it to another without retraining~\cite{shin2016deep}.} of convolutional layers to save the computational cost of computing per-example gradients.
We follow the experiment setting of Abadi et al.,~\cite{abadi2016deep}, which treats the CIFAR-10 as the private dataset and CIFAR-100 as a public dataset.
CIFAR-100 has the same image types as CIFAR-10, and it has 100 classes containing 600 images each. 
We use CIFAR-100 to train a network with the aforementioned network architecture, and then freeze the model parameters of the %\highlight{early} \baigd{what does early mean here? early is about time} 
convolutional layers and retrain only the last FC layer on CIFAR-10.

Training on the entire dataset with batch update reaches the validation accuracy of $75.75\%$, which is taken as our centralized training baseline\footnote{We note that by making the network deeper or using other advanced techniques, significantly better accuracy can be obtained, with the state-of-the-art being about 99.37\%~\cite{kolesnikov2019big}.}.
For the \short training, each participant feeds the pre-trained convolutional layers with their private data partitions, generates the input features of the FC layer, and randomly initializes the confined model parameters of the FC layer. 
They then take the input %features \baigd{what does input feature mean} 
to the FC layer as the private local training data, and train a model using Algorithm \ref{alg:cgd} with $\delta = 0.01$ and $T=6000$. 

Figure \ref{fig:cifar} and Table \ref{tab:cifar} summarize our experimental results on CIFAR-10. 
The results on the validation loss and accuracy are generally inline with that on the MNIST dataset.
In the worst case of $m = (1000 \times 32)$, \short achieves $0.724$ and $74.29\%$ in validation loss and accuracy respectively, which are relatively near to
the centralized baseline~($0.675$ and $75.72\%$). 

\begin{table}
	\caption{Performance comparison on CIFAR-10.}
	\label{tab:cifar}
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		& \multicolumn{2}{c|}{Validation loss} & \multicolumn{2}{c|}{Validation accuracy} \\ \hline
		Centralized         & \multicolumn{2}{c|}{0.675}           & \multicolumn{2}{c|}{75.72\%}             \\ \hline \hline
		& \short             & Local training           & \short               & Local training              \\ \hline
		m=($10 \times 2$)   & 0.720             & 0.980            & 74.79\%              & 65.3\%               \\ \hline
		m=($100 \times 16$)  & 0.723             & 2.008            & 74.42\%             & 26.25\%            \\ \hline
		m=($1000 \times 32$) & 0.724             & 2.434            & 74.29\%             & 16.19\%            \\ \hline
	\end{tabular}
\end{table}

We also compare the performance of \short  and the traditional FL~\cite{abadi2016deep}\footnote{The centralized baseline of validation accuracy on the CIFAR-10 in ~\cite{abadi2016deep} is 80\%.} on CIFAR-10 (Table \ref{tab:dpcifar}). Similar to the results on MNIST, the accuracy difference to the centralized baseline in \short is largely smaller than that in the traditional FL. 

\begin{table}
	\centering
	\caption{Comparison between \short and the traditional FL on CIFAR-10.}
	\label{tab:dpcifar}
	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{|l|l|l|l|}
			\hline
			\multicolumn{2}{|c|}{\short}               & \multicolumn{2}{c|}{Traditional FL via DP~\cite{abadi2016deep}}             \\ \hline
			Participants & \shortstack[l]{Difference \\to the baseline} & Noise levels                                & \shortstack[l]{Difference \\to the baseline} \\ \hline
			m=($10 \times 7$)            & 0.93\%                     & $\epsilon = 8$ (small noise)   & 7\%                      \\ \hline
			m=($100 \times 49$)           & 1.30\%                     & $\epsilon = 4$ (medium noise)  & 10\%                      \\ \hline
			m=($1000 \times 112$)            & 1.43\%                     & $\epsilon = 2$ (large noise) & 13\%                      \\ \hline
		\end{tabular}
	}
\end{table}




==> chapters/intro.tex <==
\section{Introduction}

Wile machine learning techniques based on gradient descent optimization have achieved remarkable success across a wide range of tasks~\cite{krizhevsky2017imagenet, he2016deep, devlin2018bert}, the performance of a learning model largely relies on the availability of  datasets. \baigd{``while'' implicitly implies contrast, but there is no here}
To take advantage of massive data owned by multiple entities, the federated learning has been proposed to enable multiple data owners to construct a global model~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
\baigd{need to specifically point out the threat this work is against. I don't think DP, HE, MPC are the main threat? Keep the main threat in your story, and put others in related work}
To address the privacy concerns arising from federated learning, privacy-preserving techniques, including differential privacy (DP) mechanisms~\cite{abadi2016deep, dwork2014algorithmic, shokri2015privacy} and cryptographic mechanisms, such as homomorphic encryption (HE)~\cite{chen2018privacy, marc2019privacy, sharma2019confidential} and secure multiparty computation (MPC)~\cite{ liu2017oblivious, mohassel2017secureml, bonawitz2017practical}, can be employed to provide data locality as well as  privacy-preserving sharing of the local models to synthesize the global model .

In this work, we explore the privacy-preserving federated learning based on another motivation.
It is different from the existing frameworks where participants jointly learn/share \emph{one and the same} global model.
In our framework, \emph{each participant  learns a different  global model  and these global models are also kept private, and confined  within the corresponding participants}.

In particular, we aim to achieve the following challenging goals in this work.
\begin{itemize}
\item The prediction made by any confined global model belonging to any participants should  greatly outperform the local model trained only with a single participant's data\baigd{This shouldn't be in your main goal, or the very beginning of your goals. Training on single participant's data is not your main competitor. You can have it in evaluation, but remove it from your story, otherwise it will pollute your story}, and the performance of the confined global model should approach the centralized training where all the data are collected centrally.
\item The framework should ensure the privacy in a way that each confined global model is always kept with its corresponding owner. Neither should any of the owner's local data or any intermediate results compute on its local data be leaked to other parties or a third aggregator in plaintext.
\item The framework should be practical and scalable in the presence of large scale datasets.
\end{itemize}
\baigd{Compared to the above goals, the insights how you solve the problem of privacy-preserving federated learning are more attractive. Consider talking about how the idea stems from SGD mini-batch mode (if so?). People will appreciate it}
\baigd{Need to highlight your insights. What is it? Is my understanding below correct?\\ 
Despite distributing the calculation of gradients, FL's parallelization of GD optimization in essence is an application of SGD batch model [[cite first FL paper here]], such that participants still have to jointly work the same intermediate model synchronously [[citation]] or asynchronously [[citation]].
CGD explores to further decrease the dependency by letting the participants ''}



To solve the above challenges, in this paper, we design, implement and evaluate \codename (\short) - an optimization method of learning confined global models for preserving privacy in the federated learning settings.

In \short, each participant first randomly initializes its own confined model respectively.
During each training iteration, every party solely computes the local gradients using its  private dataset and the \highlight{confined model}; \baigd{this idea hasn't been introduced yet}
collaboratively evaluates the \emph{sum} of the local gradient in a secure way (i.e., construct the addition result on a set of secret values  without revealing any  addends to each other or a third party);
and  updates its own confined model using the addition result.
We remark the difference between the \short and previous privacy-preserving federated learning frameworks~\cite{smith2017federated, bonawitz2017practical, hu2019fdml}. %\yanjun{cite NIPS' work from Guangdong}
In existing works, local gradients are also protected (via DP or HE/MPC), however, they are computed based on the same global model, and are used to update the same global model as well (usually via a third-party parameter server).
Whereas, in \short, local gradients are computed based on different confined models respectively, and using the sum of them for iterate update gives different final solution of confined models (as each model is initialized differently).
\baigd{need to be more concise} 
In addition, it is not necessarily to have a third-party aggregator in \short, depending on the choice of computational tool for secure addition operation.


A highlight of our framework is that we theoretically guarantees the convergence of \short optimization, i.e., each global model will converge to a different neighborhood of the optimal solution of centralized training. The maximum difference between the loss of \short solution and the centralized solution is bounded, and such bound can be further adjusted to a preferably small range by tuning hyper parameters in the \short optimization.

By confining the global models, we are able to achieve privacy preservation. The randomness introduced in the initialization of confined global models - which also decides their respective final locations - can be regarded as random masks to ensure privacy.
In addition, in contrast to additive noise based differentially private learning frameworks, in which the privacy loss is accumulated with the growth of training epochs (meaning that privacy can be breached if the privacy parameter reaches to an unacceptable value), in \short, the only information shared among the participants  is the \emph{sum} of the local gradients, which hides the local information including both the private data and the confined model, as long as the underlying cryptographic primitives (secure addition operation)  are not broken.

Moreover, our approach can enable privacy preservation to be achieved in a relatively cost-saving way compared to traditional HE/MPC-based mechanisms. The extra computation/communication cost in \short only lies in the secure addition operation, which is far more efficient than the secure multiplication operations and non-linear functions on ciphertext~\cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}.



\subsection{Contribution}

We summarize the main contributions of this paper as follows:

\begin{itemize}
	\item \textbf{A New Privacy-preserving Federated Learning Framework.}
	We propose a new optimization method \short for privacy-preserving federated learning.
	In \short, each participant learns and confines a different global model.
	It preserves privacy while enabling a wide range of machine learning algorithms that use gradient descent for optimization.
	
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short optimization under certain assumptions on the loss function (such as convexity).
	We prove the solution of \short will converge toward the optimal solution of centralized training with regard to the number of iterations.
	The maximum gap between  \short solution and the centralized optimal solution is bounded, and can be tuned by the hyper-parameter setting.
	%That is, each  global model converges to a different neighborhood of the optimal solution of centralized training

	\item \textbf{Provable Privacy Preservation.}
	We prove the privacy preservation of \short, demonstrating that given only the \emph{sum} of the local gradients which are computed on different confined model, an  \emph{honest-but-curious} adversary who may control $t$ out of $m$ participants (where $t \leq m-2$), including the aggregator for secure addition operation (if there is any), can learn ``nothing more” than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Experimental Evaluations.} We implement \short and conduct experiments on both the MNIST dataset and the CIFAR-10 dataset.
	Extensive experimental results have demonstrated that \short can closely approach the performance of centralized learning with respect to validation loss and accuracy, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro1.tex <==
\section{Introduction}
\yanjun{new version, start here}

The performance of machine learning largely relies on the availability of large and representative datasets, which may contain private information. 
To take advantage of massive data owned by multiple entities, the federated learning (FL) has been proposed to enable multiple data owners to construct a \highlight{global model}  without sharing the datasets by distributing the calculation of gradients onto data owners~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.~\yanjun{we may use global model, as the term appears in related works such as CCS'15 Shokri and Shmatikov, and CCS'17 Bonawitz.}

Despite this, FL's parallelization of gradient descent optimization in essence is an application of stochastic gradient descent (SGD)/mini-batch model~\cite{konevcny2016federated}, such that participants still have to jointly work the same intermediate \highlight{global} model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml} via a coordinating server. %, and the learning process is usually coordinated by a parameter server.
However, such sharing of the same global model makes existing FL susceptible to information leakage. Even though the local gradients can be securely synthesized via a variety of privacy preserving techniques~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep, shokri2015privacy}, the global model parameter that have to be shared during the training iteration still can be used to infer the information of original dataset. 
%\yanjun{Actually, the insufficiency of privacy guarantees of existing methods is different with regards to the differenct privacy-preserving techniques. For MPC/HE, it is the update of the same global model during iterations that leaks the information about the original dataset; For DP, the model itself is projected (via additive noise), however, the privacy cost is accumulated with repeated access to the training sample. Those insufficiencies with respect to differenct techniques are detailed in related works and summerized in Table \ref{tab:differ}. I was wondering if we shall mention MPC/HE and DP in the intro here? Or it might be a bit tedious? How would you think?}

\yanjun{Guangdong, I received Surya's comments today and he has some notes in this part: Surya--``I think we can say something about the architecture here. Note that the federated machine learning works is not a fully decentralised; a central server coordinates the learning process; whereas your architecture is fully decentralised and the learning works in a peer-peer model. I think we need to highlight the architectural aspects. In such architecture, we can use HE/MPC to gurantee privacy, but it raises a new challenge - how do you know learned model in each party converges? (Similar to blockchain model). "} \yanjun{ How would you think? Do we need to mention the decentralization here, like ``This work explores a different FL architecture towards the decentralization, or fully decentralised FL, bla bla''?} 

This work explores to further decrease the dependency by letting \emph{each participant learn a different  global model, and these global models are also kept private, and confined  within the corresponding participants}. 
%, we propose \codename (\short)  to further decrease the dependency during the learning process. In \short, \emph{each participant learns a different  global model and these global models are also kept private, and confined  within the corresponding participants}. 
We name these global models as \emph{confined models}.

In particular, we aim to achieve the following two main goals in this work.
\begin{itemize}
	\item \textbf{Convergence.} The prediction capability of any confined global model belonging to any participants should approach that in the centralized training where all the data are collected centrally. That is, these confined models should converge to the near neighborhoods of the centralized optimal solution. 
	\item \textbf{Privacy.} The framework should ensure the privacy in a way that each confined global model is different and always kept with its corresponding owner. Neither should any intermediate results during the training iterations leak any information of the owner's local data or the confined model.  That is, all model learning and updates happen locally. 
	%any intermediate results compute on its local data be leaked to other parties or a third aggregator in plaintext.
	%\item The framework should be practical and scalable in the presence of large scale datasets.
\end{itemize}

To solve the above challenges, in this paper, we design, implement and evaluate \codename (\short) - an optimization method of learning confined global models for preserving privacy in the federated learning settings.

In \short, each participant first randomly initializes its own confined model privately.
During each training iteration, every participant solely computes the local gradients from its private datasets and the corresponding confined model; %based on its  private dataset and its corresponding confined model; %and the \highlight{confined model}; \baigd{this idea hasn't been introduced yet}
then collaboratively evaluates the \emph{sum} of the local gradient in a secure way (i.e., construct the addition result on a set of secret values  without revealing any  addends to each other or a third party);
and then updates its own confined model using the addition result.
As the randomness which is separately introduced in the initialization makes each confined model initially different, it also results in the final model to be different via \short's iterate update mechanism. 
We also note that our framework does not require a third-party parameter server for synthesizing the global mode as the existing FL frameworks do, as each participant is in charge of updating its own confined global model, (but there might be an addition aggregator though, depending on the choice of computational tool for secure addition operation).


\yanjun{new version, end here}

\yanjun{old version, start here}

Wile machine learning techniques based on gradient descent optimization have achieved remarkable success across a wide range of tasks~\cite{krizhevsky2017imagenet, he2016deep, devlin2018bert}, the performance of a learning model largely relies on the availability of  datasets. \baigd{``while'' implicitly implies contrast, but there is no here}
To take advantage of massive data owned by multiple entities, the federated learning has been proposed to enable multiple data owners to construct a global model~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
\baigd{need to specifically point out the threat this work is against. I don't think DP, HE, MPC are the main threat? Keep the main threat in your story, and put others in related work}
To address the privacy concerns arising from federated learning, privacy-preserving techniques, including differential privacy (DP) mechanisms~\cite{abadi2016deep, dwork2014algorithmic, shokri2015privacy} and cryptographic mechanisms, such as homomorphic encryption (HE)~\cite{chen2018privacy, marc2019privacy, sharma2019confidential} and secure multiparty computation (MPC)~\cite{ liu2017oblivious, mohassel2017secureml, bonawitz2017practical}, can be employed to provide data locality as well as  privacy-preserving sharing of the local models to synthesize the global model .

In this work, we explore the privacy-preserving federated learning based on another motivation.
It is different from the existing frameworks where participants jointly learn/share \emph{one and the same} global model.
In our framework, \emph{each participant  learns a different  global model  and these global models are also kept private, and confined  within the corresponding participants}.

In particular, we aim to achieve the following challenging goals in this work.
\begin{itemize}
\item The prediction made by any confined global model belonging to any participants should  greatly outperform the local model trained only with a single participant's data\baigd{This shouldn't be in your main goal, or the very beginning of your goals. Training on single participant's data is not your main competitor. You can have it in evaluation, but remove it from your story, otherwise it will pollute your story}, and the performance of the confined global model should approach the centralized training where all the data are collected centrally.
\item The framework should ensure the privacy in a way that each confined global model is always kept with its corresponding owner. Neither should any of the owner's local data or any intermediate results compute on its local data be leaked to other parties or a third aggregator in plaintext.
\item The framework should be practical and scalable in the presence of large scale datasets.
\end{itemize}
\baigd{Compared to the above goals, the insights how you solve the problem of privacy-preserving federated learning are more attractive. Consider talking about how the idea stems from SGD mini-batch mode (if so?). People will appreciate it}
\baigd{Need to highlight your insights. What is it? Is my understanding below correct?\\ 
Despite distributing the calculation of gradients, FL's parallelization of GD optimization in essence is an application of SGD batch model [[cite first FL paper here]], such that participants still have to jointly work the same intermediate model synchronously [[citation]] or asynchronously [[citation]].
CGD explores to further decrease the dependency by letting the participants ''}



To solve the above challenges, in this paper, we design, implement and evaluate \codename (\short) - an optimization method of learning confined global models for preserving privacy in the federated learning settings.

In \short, each participant first randomly initializes its own confined model respectively.
During each training iteration, every party solely computes the local gradients using its  private dataset and the \highlight{confined model}; \baigd{this idea hasn't been introduced yet}
collaboratively evaluates the \emph{sum} of the local gradient in a secure way (i.e., construct the addition result on a set of secret values  without revealing any  addends to each other or a third party);
and  updates its own confined model using the addition result.
We remark the difference between the \short and previous privacy-preserving federated learning frameworks~\cite{smith2017federated, bonawitz2017practical, hu2019fdml}. %\yanjun{cite NIPS' work from Guangdong}
In existing works, local gradients are also protected (via DP or HE/MPC), however, they are computed based on the same global model, and are used to update the same global model as well (usually via a third-party parameter server).
Whereas, in \short, local gradients are computed based on different confined models respectively, and using the sum of them for iterate update gives different final solution of confined models (as each model is initialized differently).
\baigd{need to be more concise} 
In addition, it is not necessarily to have a third-party aggregator in \short, depending on the choice of computational tool for secure addition operation.

\yanjun{old version, end here}

A highlight of our framework is that we theoretically guarantees the convergence of \short optimization, i.e., each global model will converge to a different neighborhood of the optimal solution of centralized training. The maximum difference between the loss of \short solution and the centralized solution is bounded, and such bound can be further adjusted to a preferably small range by tuning hyper parameters in the \short optimization.

By confining the global models, we are able to achieve privacy preservation. The randomness introduced in the initialization of confined global models - which also decides their respective final locations - can be regarded as random masks to ensure privacy.
In addition, in contrast to additive noise based differentially private learning frameworks, in which the privacy loss is accumulated with the growth of training epochs (meaning that privacy can be breached if the privacy parameter reaches to an unacceptable value), in \short, the only information shared among the participants  is the \emph{sum} of the local gradients, which hides the local information including both the private data and the confined model, as long as the underlying cryptographic primitives (secure addition operation)  are not broken.

Moreover, our approach can be practical and scalable in the presence of large scale datasets, as the extra computation/communication cost in \short only lies in the secure addition operation, which is far more efficient than the secure multiplication operations and non-linear functions on ciphertext~\cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}.



\subsection{Contribution}
\yanjun{Here is the comments from Surya: ``The contributions should be framed as:
- Fully decentralised FL 
- Convergence of model 
- Provable privacy 
- Performance:"} \yanjun{How would you think of his point regarding the ``decentralization"? }

We summarize the main contributions of this paper as follows:

\begin{itemize}
	\item \textbf{A New Privacy-preserving Federated Learning Framework.}
	We propose a new optimization method \short for privacy-preserving federated learning.
	In \short, each participant learns and confines a different global model.
	It preserves privacy while enabling a wide range of machine learning algorithms that use gradient descent for optimization.
	
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short optimization under certain assumptions on the loss function (such as convexity).
	We prove the solution of \short will converge toward the optimal solution of centralized training with regard to the number of iterations.
	The maximum gap between  \short solution and the centralized optimal solution is bounded, and can be tuned by the hyper-parameter setting.
	%That is, each  global model converges to a different neighborhood of the optimal solution of centralized training

	\item \textbf{Provable Privacy Preservation.}
	We prove the privacy preservation of \short, demonstrating that given only the \emph{sum} of the local gradients which are computed on different confined model, an  \emph{honest-but-curious} adversary who may control $t$ out of $m$ participants (where $t \leq m-2$), including the aggregator for secure addition operation (if there is any), can learn ``nothing more” than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Experimental Evaluations.} We implement \short and conduct experiments on both the MNIST dataset and the CIFAR-10 dataset.
	Extensive experimental results have demonstrated that \short can closely approach the performance of centralized learning with respect to validation loss and accuracy, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro2.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities.
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}. \baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow and PyTorch, and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(the mini-batch model in precise)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in centralized FL) or a peer-to-peer communication scheme~(in decentralized FL).
Each of them obtains the current model parameters, works out a local gradient based on the local data, and shares it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy~\cite{nasr2019comprehensive}: 
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy, secure multi-party communication, and homomorphic encryption~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep, shokri2015privacy}, \baigd{separate the citations}
the global model parameters that have to be shared still can be used to infer information about the raw datasets~\cite{nasr2019comprehensive}.

This work explores to further decrease the dependency by \emph{letting each participant learn a different global model}.
Each of them maintains their own global models locally, which are strictly confined within themselves throughout the training process.
We thus name these localized global models as \emph{confined models}, to differentiate them from the global models in traditional FL.
We propose a new optimization algorithm named \codename (\short) for training confined models.
\short is designated to converge to a model parameter adjacent to the global model learned from aggregated data~(referred to as \emph{centralized model}), so as to
retain the merits of FL while providing privacy preservation.
This adjacency is proved to be bounded~(cf. Section~\ref{}), and thus we call the convergence a \emph{bounded convergence}.

%\short is designated to satisfy the following two properties, so as to retain the merits of FL while providing privacy preservation.
%\begin{itemize}
%	\item \textbf{Convergence.} The prediction capability of any confined model should approach that of the global model learned from aggregated data~(referred to as \emph{centralized model}).
%That is, \emph{\short should converge to a model parameter adjacent to the centralized model}.
%We require the adjacency to be bounded~(cf. Section~\ref{}), and thus we call this convergence a \emph{bounded convergence}.
%%	\item \textbf{Information Confinement.} The confined models differ from each other in a way that any of them cannot be derived by knowing all of the rest. \baigd{we need to discuss this. I don't think it is necessary to be underivable, but it was ``each confined global model is differen'', which is vague.} \baigd{This point is about whether the deviations on confined models are possible to leak information, which is different from the following point. Move to be with convergence - but converge to a different model parameter?}
%\item \textbf{Information Confinement.} Any shared intermediate result should be immune to \highlight{what attack?}~\cite{}.
%In addition, although finally become adjacent to the centralized model when the training process completes, the intermediate confined models during the training iterations are sufficiently different from each other that \highlight{model reversion attack}~\cite{} \baigd{check this} could be defeated.
%\end{itemize}

\short let each participant arbitrarily~\baigd{is this to strong?} initialize their own confined models.
In a training iteration, each of them independently computes the local gradient from its current confined model and local data.
All of them then jointly work out the \emph{sum} of all local gradients in a secure way and use it to update their confined models locally.
Collaboratively calculating the sum of a set of secret values without revealing any addends has proved to be feasible~\cite{cite secure additive}, and has been applied to achieve decentralization in FL~\cite{zhang2020privcoll}.
The proposed algorithm eliminates the necessity of sharing the same global model in either centralized or decentralized way, alleviating the threat of the model reversion attack~\cite{}. 


\baigd{up to here}

\begin{figure*}[!t]
	\centering
	\includegraphics[width=6in]{fig/confined.pdf}
	\caption{Confined .}
	\label{fig:confined}
\end{figure*}


In addition, although finally become adjacent to the centralized model when the training process completes, the intermediate confined models during the training iterations are sufficiently different from each other that \highlight{model reversion attack}~\cite{} \baigd{check this} could be defeated.


\highlight{As the randomness which is separately introduced in the initialization makes each confined model initially different, it also results in the final model to be different via \short's iterate update mechanism.} \baigd{random initialization cannot guarantee different result, SGD is an example}



\short is demonstrated to guarantee the convergence, both theoretically and experimentally.


By confining the global models, we are able to achieve privacy preservation. The randomness introduced in the initialization of confined global models - which also decides their respective final locations - can be regarded as random masks to ensure privacy.
In addition, in contrast to additive noise based differentially private learning frameworks, in which the privacy loss is accumulated with the growth of training epochs (meaning that privacy can be breached if the privacy parameter reaches to an unacceptable value), in \short, the only information shared among the participants  is the \emph{sum} of the local gradients, which hides the local information including both the private data and the confined model, as long as the underlying cryptographic primitives (secure addition operation)  are not broken.

Moreover, our approach can be practical and scalable in the presence of large scale datasets, as the extra computation/communication cost in \short only lies in the secure addition operation, which is far more efficient than the secure multiplication operations and non-linear functions on ciphertext~\cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}.



\subsection{Contribution}
\yanjun{Here is the comments from Surya: ``The contributions should be framed as:
- Fully decentralised FL
- Convergence of model
- Provable privacy
- Performance:"} \yanjun{How would you think of his point regarding the ``decentralization"? }

We summarize the main contributions of this paper as follows:

\begin{itemize}
	\item \textbf{A New Privacy-preserving Federated Learning Framework.}
	We propose a new optimization method \short for privacy-preserving federated learning.
	In \short, each participant learns and confines a different global model.
	It preserves privacy while enabling a wide range of machine learning algorithms that use gradient descent for optimization.
	
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short optimization under certain assumptions on the loss function (such as convexity).
	We prove the solution of \short will converge toward the optimal solution of centralized training with regard to the number of iterations.
	The maximum gap between  \short solution and the centralized optimal solution is bounded, and can be tuned by the hyper-parameter setting.
	%That is, each  global model converges to a different neighborhood of the optimal solution of centralized training

	\item \textbf{Provable Privacy Preservation.}
	We prove the privacy preservation of \short, demonstrating that given only the \emph{sum} of the local gradients which are computed on different confined model, an  \emph{honest-but-curious} adversary who may control $t$ out of $m$ participants (where $t \leq m-2$), including the aggregator for secure addition operation (if there is any), can learn ``nothing more” than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Experimental Evaluations.} We implement \short and conduct experiments on both the MNIST dataset and the CIFAR-10 dataset.
	Extensive experimental results have demonstrated that \short can closely approach the performance of centralized learning with respect to validation loss and accuracy, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro3.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities.
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow and PyTorch, and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or the mini-batch model)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in centralized FL) or a peer-to-peer communication scheme~(in decentralized FL).
Each of them obtains the current model parameters, works out a local gradient based on the local data, and shares it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy~\cite{nasr2019comprehensive}:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared still can be used to infer information about the raw datasets (illustrated in Figure \ref{fig:fl}).

This work further decreases the dependency among FL participants by approaching the ambition of \emph{eliminating the explicit sharing of the central global model} which is the root cause of the model inversion attack~\cite{fredrikson2015model, nasr2019comprehensive}.
We propose a new optimization algorithm named \codename (\short) that enables each FL participant to learn a proprietary global model.
Each of them maintains their own global models locally, which are strictly confined within themselves from the very beginning of and throughout the whole training process (Figure \ref{fig:confined}).
We name these localized global models as \emph{confined models}, to differentiate them from the global model in traditional FL.


\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$. Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and the results of $iter_{FL}$ which is in essence a composite function of $w$ and  $\xi_a, \xi_b, \xi_c$, a curious adversary is able to derive information about the raw datasets from the FL.]{{\includegraphics[width=7.2cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
	\subfloat[\codename. Each participant strictly confines their own global models locally from the very beginning of $w_0^a, w_0^b, w_0^c$ to their respective optimal points $w_*^a, w_*^b, w_*^c$. The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data. The distance between any two confined models in the colony keeps same throughout the training process, meaning that $w_*^a, w_*^b, w_*^b$ will not become closer to each other to the end of the optimization which ensures privacy, 
	while they will simultaneously  converge to a ``almost flat land" near the centralized optimal point where the loss is close to minimun.]{{\includegraphics[width=6.7cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Gradient descent in  traditional federated learning and \short, where $w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration, and $iter_{FL}$, $iter_{\short}$  are the abstractions for model updates going through all training iterations.}
	\label{fig:compgd}
\end{figure*}


The key idea that inspires \short's solution is that, the gradient descent algorithm $\mathcal{A}$, when applied on a convex objective function $F$, could start with a colony of %proximate 
nearby points. Iteratively descending using the joint gradient of the colony would lead $\mathcal{A}$ to another colony at the neighborhood of the optimal of $F$.
%Our idea is inspired by ... \baigd{observation? theorem? any mathematical theorem to support something like ``in a convex objective function f, the optimization algorithm could start with multiple discrete points, and the sum of the gradient at those points lead the algorithm to a neighborhood of the optimal of f"}
In the \short optimization, the algorithm first lets each participant randomly initialize the starting point of their own confined model.
A default setting is to let each of them solely apply random sampling from the Gaussian distribution of mean 0 and variance 1, which is the standard weight initialization scheme used in machine learning.
%\short lets each participant arbitrarily~\baigd{is this to strong?} initialize their own confined models.
Then, in every training iteration, each participant independently computes the local gradient from its current confined model and local data.
All of them then jointly work out the \emph{sum} of all local gradients in a secure way and use it to update their confined models.
In this way, \short is guaranteed to converge to a model parameter adjacent to the global model learned from aggregated data~(referred to as \emph{centralized model}).
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}), and thus we call the convergence a \emph{bounded convergence}.

The privacy preservation of \short (illustrated in Figure \ref{fig:confined}) relies on collaboratively calculating the sum of a set of secret values without revealing any addends.
This has been proved to be feasible~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}, and has been applied to achieve decentralization in FL~\cite{zhang2020privcoll}.
While providing privacy preservation, \short retains the merits of FL such as algorithm independence and asynchronicity. %\baigd{I may be wrong with these two, but need to talk about the implications of \short, both good and bad. If any bad one, better to discuss here before reviewers point it out, initialization scheme }

\short is demonstrated to guarantee the bounded convergence, both theoretically and experimentally.
Through our theoretical analysis, we prove that the confined models learned by \short can converge toward the centralized optimal solution with bounded difference. 
Our experiments also demonstrate such bound, and show that it is adjustable and can be set to a preferably small range by tuning hyper-parameters in the \short optimization.
 
 
%Through our convergence analysis, we prove that the solution of \short will converge toward the centralized optimal value. In addition, we identify characteristics of \short, specifically,  hyper-parameters that we can tune to adjust the convergence rate and the bound of difference between \short's solution and the centralized optimum. 
%For the convergence rate, it can be adjusted by a deliberately designed adaptive learning rate; and for the bound between \short solution and the centralized optimum, we introduce an initialization hyper-parameter, which decides the range of the initial confined models and can be used to adjust the bound to a preferably small range.


%\baigd{Talking about analysis, experiments, etc. here }
%Experiment standard weight initialization scheme

%\baigd{up to here}



%By confining the global models, we are able to achieve privacy preservation. The randomness introduced in the initialization of confined global models - which also decides their respective final locations - can be regarded as random masks to ensure privacy.
%In addition, in contrast to additive noise based differentially private learning frameworks, in which the privacy loss is accumulated with the growth of training epochs (meaning that privacy can be breached if the privacy parameter reaches to an unacceptable value), in \short, the only information shared among the participants  is the \emph{sum} of the local gradients, which hides the local information including both the private data and the confined model, as long as the underlying cryptographic primitives (secure addition operation)  are not broken.

%Moreover, our approach can be practical and scalable in the presence of large scale datasets, as the extra computation/communication cost in \short only lies in the secure addition operation, which is far more efficient than the secure multiplication operations and non-linear functions on ciphertext~\cite{gentry2009fully,albrecht2018homomorphic,yao1986generate, goldreich2019play}. \baigd{what is the point to address?}



\subsection{Contribution}

We summarize the main contributions of this paper as follows:

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	We propose a new optimization algorithm \short for privacy-preserving decentralized federated learning.
	In \short, we eliminate the explicit sharing of the central global model and let each participant learns and confines a proprietary global model.
	%It preserves privacy while enabling a wide range of machine learning algorithms that use gradient descent for optimization.
	We also eliminate the necessity of a centralized coordinating server, and the optimization can be achieved in a peer-to-peer communication scheme.
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short optimization under certain assumptions on the loss function (such as convexity).
	We prove the solution of \short will converge toward the optimal solution of centralized training with regard to the number of iterations.
	The maximum gap between  \short solution and the centralized optimal solution is bounded, and can be tuned by the hyper-parameter setting.
	%That is, each  global model converges to a different neighborhood of the optimal solution of centralized training
	
	\item \textbf{Provable Privacy Preservation.}
	We prove the privacy preservation of \short, demonstrating that given only the \emph{sum} of the local gradients which are computed on different confined model, an  \emph{honest-but-curious} adversary who may control $t$ out of $m$ participants (where $t \leq m-2$), including the aggregator for secure addition operation (if there is any), can learn ``nothing more” than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Experimental Evaluations.} We implement \short and conduct experiments on both the MNIST dataset and the CIFAR-10 dataset.
	Extensive experimental results have demonstrated that \short can closely approach the performance of centralized learning with respect to validation loss and accuracy. %, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro4.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow and PyTorch, and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or its mini-batch mode)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in centralized FL)~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep} or a peer-to-peer communication scheme~(in decentralized FL)~\cite{kim2019blockchained, roy2019braintorrent}.
Each of them obtains the current model parameters, works out a local gradient based on the local data, and
disseminates it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared are still susceptible to attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}. %\remove{ (illustrated in Figure ref{fig:fl})}.
%can be abused to infer information about the raw datasets (refer to~\cite{nasr2019comprehensive} and also illustrated in Figure \ref{fig:fl}).
%\highlight{abused by the model inversion attack to infer information about the raw datasets} (illustrated in Figure \ref{fig:fl}). \baigd{Is this precise?} \yanjun{I thought we might not restrict the attack to the model inversion attack, as there are also some others in the literature such as membership inference attack, model extraction attack...?} \baigd{Then a single reference and Figure 1a is too weak to support your argument. You can say such as model inversion [] and membership inference [] }

This work further decreases the dependency among FL participants by approaching the ambition of \emph{eliminating the explicit sharing of the central global model} which is the root cause of the information leakage~\cite{fredrikson2015model, nasr2019comprehensive}.  %model inversion attack
We propose a new optimization algorithm named \codename (\short) that enables each participant to learn a proprietary global model.
%\replace{Each of them}{A \short participant} 
A \short participant maintains %\replace{their}{its} 
its own global models locally, which are strictly confined within %\replace{themselves}{itself} 
itself from the very beginning of and throughout the whole training process. %\remove{(Figure ref{fig:confined})}.
We name these localized global models as \emph{confined models}, to distinguish them from the global model in traditional FL.
%\add{We also illustrate the comparison between our work and traditional FL in Figure}~\ref{fig:compgd}. 
We also illustrate the comparison between our work and traditional FL in Figure~\ref{fig:compgd}.
\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$ using the updates computed by $f$.
	Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and $f$, the adversary is able to derive information about the local raw data $\xi_a, \xi_b, \xi_c$.
	 %values of $f$ \baigd{This sentence is too long. Does $f$ have a name in ML context? } which is a composite function for computing the model updates with \replace{arguments $w$ and  $\xi_a, \xi_b, \xi_c$}{local gradients?}, the adversary is able to derive information about the raw data.
	 ]{{\includegraphics[width=7.2cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
\subfloat[\codename. Each participant strictly confines their own global models from their initialization~($w_0^a, w_0^b, w_0^c$) to optimal values~($w_*^a, w_*^b, w_*^c$).
The confined models descend in the same pace, and when \short converges, reach the bottom of the valley where the centralized model is located.  %\replace{a ``almost flat land" near the centralized optimal point where the loss is close to minimun}{the valley where the central model is located},
%\remove{The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data.} \baigd{it is said in the text}
Any two confined models keep the same distance throughout the training process. 
In other words, $w^a, w^b, w^c$ would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others. 
]{{\includegraphics[width=6.7cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Comparison of \short and the gradient descent in  traditional FL. %\replace{$w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration,}{This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$}, and $iter$ \replace{is the abstraction to indicate}{represents} the sum-up of all iterations. %\replace{are the abstractions for model updates going through all training iterations.}{indicate the model updates}
		This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$, and $iter$ represents the sum-up of all iterations.
	}
	%\baigd{some confusion here: $iter_{FL}$ and $iter_{\short}$ indicate one iteration or sum-up of all iterations? Confirm this and you will know whether you need $w_k$ or $w$}
	\label{fig:compgd}
\end{figure*}


The key observation that inspires \short's solution is that, when a convex smooth function moves to its global minimum, the steepness of its first derivative will decrease and become flat when the function converges.
%the Hessian matrix (i.e. the second derivative) of a convex function is positive semidefinite. It indicates that the steepness of the error curve will decrease towards its global minimum, and become very gradual when the function converges.
As such, a gradient descent algorithm $\mathcal{A}$, when applied on a convex objective function $F$, could start with a colony of discrete points.
Iteratively descending the colony would lead it to the neighborhood of a flat valley bottom where the loss is close to minimum. 

%the gradient descent algorithm $\mathcal{A}$, when applied on a convex %\highlight{convex} \baigd{do we have to restrict GCD to convex function?} %\yanjun{yes, our convergence is guaranteed based on the assumption of convexity}
%objective function $F$, could start with a colony of nearby %proximate
%points. Iteratively descending using the joint gradient of the colony would lead $\mathcal{A}$ to another colony at the neighborhood of the optimum of $F$.
%Our idea is inspired by ... \baigd{observation? theorem? any mathematical theorem to support something like ``in a convex objective function f, the optimization algorithm could start with multiple discrete points, and the sum of the gradient at those points lead the algorithm to a neighborhood of the optimal of f"}
\short first lets each participant %\highlight{randomly}
randomly initialize the starting point of their own confined models solely.
%The weight initialization scheme and the hyper-parameter for adjusting the range of the initial weight are also confined within each participant to protect the information about the average model distance.
A default setting is to sample based on the Gaussian distribution of mean 0 and the variance 1, %and then calibrated by the sample size,
which is the standard weight initialization scheme used in machine learning~\cite{glorot2010understanding}. %\baigd{Good. Be careful when you use ``random''. It is quite different from its Chinese translation, also vague. Either uniformly random or non-uniformly random could be called random. When you sample something at random, you sample it based on some distribution}
%\short lets each participant arbitrarily~\baigd{is this to strong?} initialize their own confined models.
%That is, to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$ to protect the information about the average model distance
In every training iteration, each participant independently computes the local gradient from its current confined model and local data.
All of them then jointly work out the \emph{sum} of all local gradients in a secure way and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
In this way, \short is guaranteed to converge to %\replace{a model parameter}{confined models}
confined models adjacent to the global model learned when using aggregated data~(referred to as the \emph{centralized model}). %\baigd{We need to unify this. Sometimes we use central model}
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}).
%, and thus we call the convergence a \emph{bounded convergence}.
%In addition, in order to protect the information about the average model distance, \short introduces a hyper-parameter, which is also confined within each participant, for adjusting the range of the initial weight.

%\short retains the merits of traditional FL such as algorithm independence and \highlight{asynchronicity}. \baigd{I am not sure on asynchronicity, because participants need to jointly work out the sum to proceed with update}
\short retains the merits of traditional FL such as algorithm independence. %\replace{the algorithm independence in traditional FL}{the merits of traditional FL such as algorithm independence}.
Therefore, it can easily accommodate any FL schemes regardless of their underlying machine learning or deep learning algorithms.
To prevent the adversary from learning indirect information from the local gradients of other participants,
we further equip \short with the secure sharing of the sum of the local gradients.
This has been proved to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}. 
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL.
In addition, to avoid leaking the average distance between the confined models, 
\short allows independent initialization of the confined models. 
%\highlight{Our experiment finds that it keeps robust~(in terms of accuracy?) at a difference by X orders (cf. Section X). } \baigd{to update}
Our experiment finds that it keeps robust in terms of validation accuracy at a difference by $2$ orders (cf. Section \ref{sec:init}).

%\short introduces a hyper-parameter for adjusting the range of the initial weight.
%\highlight{In addition, to further protect the information about the average model distance, we  introduces a hyper-parameter for adjusting the range of the initial weight, which is also confined within each participant. }
%\yanjun{Here, I refer the hyper-parameter to $\delta$. My thought is to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$, which increase the difficulty of inferring the the average model distance. Would you think it may alleviate the concern on the privacy aspect of the privacy-utitily tradeoff?}

We theoretically and experimentally evaluate \short.
We formally prove that the confined models learned by \short are proximal to the centralized model with bounded variance,
%\highlight{The variance indicates the tradeoff between the adversary's knowledge of the average model distance and the accuracy of the confined models, } \baigd{check this}
and it is adjustable via tuning hyper-parameters in the \short optimization.
Our experimental results on two datasets demonstrate that the accuracy performance of \short closely approaches the %\replace{optimal}{product}
product of its centralized counterpart. The difference of validation  accuracy between \short and the centralized baseline is within $0.5\%$ on  MNIST and $1.43\%$ on  CIFAR-10.

%For example, in the experiment on the  MNIST dataset, \short achieves  $97.08\%$ in validation  accuracy with $(1000 \times 112)$ participants , which closely approaches $97.61\%$ our centralized learning baseline in which the validation loss  and  accuracy are $0.078$ and $97.61\%$ respectively.
%... \baigd{give some statistics on accuracy here}

\paragraph{Contribution}
We summarize the main contributions of this paper as follows.

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	We propose a new optimization algorithm \short for privacy-preserving decentralized FL.
	In \short, we eliminate the explicit sharing of the global model and let each participant learn a proprietary confined model.
	We also eliminate the necessity of a central coordinating server, and the optimization can be conducted in a fully decentralized manner.
%\baigd{does secure addition scheme need a central server?} \yanjun{some need, some need not, depending on the choice of particular technique}
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short under certain realistic assumptions on the loss function (such as convexity).
	We prove \short converges toward the centralized model as the number of iterations increases. %\remove{optimal of centralized training}{central model} \replace{with regard to the number of iterations}{as the number of iterations increases}.
	The distance among the trained confined models and the centralized model is bounded, and can be tuned by the hyper-parameter setting.

	\item \textbf{Provable Privacy Preservation.}
	We prove the privacy preservation of \short, demonstrating that given only the \emph{sum} of the local gradients, an \emph{honest-but-curious} white-box adversary who may control $t$ out of $m$ participants~(where $t \leq m-2$), including the aggregator for secure addition operation~(if any), can learn no information other than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Functional Evaluations.} We implement \short and conduct experiments on MNIST and CIFAR-10 datasets.
	The results demonstrate that \short can closely approach the performance of centralized learning in terms of the validation loss and accuracy. %, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro5.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
To increase dataset participation from multiple dataset owners/entities and reduce barriers for sharing datasets to another party, federated learning (FL) approaches are proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}. 
%Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow and PyTorch, and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or %\replace{its}{SGD} 
the mini-batch mode)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in centralized FL)~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep} or a peer-to-peer communication scheme~(in decentralized FL)~\cite{kim2019blockchained, roy2019braintorrent}.
Each of them obtains the current model parameters, works out a local gradient based on the local data, and
disseminates it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared are still susceptible to attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}. %\remove{ (illustrated in Figure ref{fig:fl})}.
%can be abused to infer information about the raw datasets (refer to~\cite{nasr2019comprehensive} and also illustrated in Figure \ref{fig:fl}).
%\highlight{abused by the model inversion attack to infer information about the raw datasets} (illustrated in Figure \ref{fig:fl}). \baigd{Is this precise?} \yanjun{I thought we might not restrict the attack to the model inversion attack, as there are also some others in the literature such as membership inference attack, model extraction attack...?} \baigd{Then a single reference and Figure 1a is too weak to support your argument. You can say such as model inversion [] and membership inference [] }

This work further decreases the dependency among FL participants by %approaching the ambition of 
\emph{eliminating the explicit sharing of the central global model} which is the root cause of the information leakage~\cite{fredrikson2015model, nasr2019comprehensive}.  %model inversion attack
We propose a new optimization algorithm named \codename (\short) that enables each participant to learn a proprietary global model.
%\replace{Each of them}{A \short participant}
The \short participants maintain %\replace{their}{its}
their own global models locally, which are strictly confined within %\replace{themselves}{itself}
themselves from the very beginning of and throughout the whole training process. %\remove{(Figure ref{fig:confined})}.
We name these localized global models as \emph{confined models}, to distinguish them from the global model in traditional FL.
%\add{We also illustrate the comparison between our work and traditional FL in Figure}~\ref{fig:compgd}.
In Figure~\ref{fig:compgd}, we %\replace{also}{further}
further illustrate %\replace{the}{a holistic}
a holistic comparison between our work and traditional FL.

\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$ using the iterate updates computed by $f$. %, \add{e.g., the XXX function}.
	Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and $f$, the adversary is able to derive information about the local raw data $\xi_a, \xi_b, \xi_c$.
	 %values of $f$ \baigd{This sentence is too long. Does $f$ have a name in ML context? } which is a composite function for computing the model updates with \replace{arguments $w$ and  $\xi_a, \xi_b, \xi_c$}{local gradients?}, the adversary is able to derive information about the raw data.
	 ]{{\includegraphics[width=7cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
\subfloat[\codename. Each participant strictly confines their own global models from their initialization~($w_0^a, w_0^b, w_0^c$) to optimal values~($w_*^a, w_*^b, w_*^c$).
The confined models descend in the same pace, and when \short converges, reach the bottom of the valley where the centralized model is located.  %\replace{a ``almost flat land" near the centralized optimal point where the loss is close to minimun}{the valley where the central model is located},
%\remove{The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data.} \baigd{it is said in the text}
Any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$ would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.
]{{\includegraphics[width=6.2cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Comparison of \short and the gradient descent in  traditional FL. %\replace{$w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration,}{This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$}, and $iter$ \replace{is the abstraction to indicate}{represents} the sum-up of all iterations. %\replace{are the abstractions for model updates going through all training iterations.}{indicate the model updates}
		This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$, and $iter$ represents the sum-up of all iterations.
	}
	%\baigd{some confusion here: $iter_{FL}$ and $iter_{\short}$ indicate one iteration or sum-up of all iterations? Confirm this and you will know whether you need $w_k$ or $w$}
	\label{fig:compgd}
\end{figure*}

%\baigd{Check my writing at the bottom of this paragraph} 
%The key observation that inspires \short's solution is that, when a convex smooth function moves to its global minimum, the steepness of its first derivative will decrease and become flat when the function converges.
%the Hessian matrix (i.e. the second derivative) of a convex function is positive semidefinite. It indicates that the steepness of the error curve will decrease towards its global minimum, and become very gradual when the function converges.
%As such, a gradient descent algorithm $\mathcal{A}$, when applied on a convex objective function $F$, could start with a colony of discrete points.
%Iteratively descending the colony would lead it to the neighborhood of a flat valley bottom where the loss is close to minimum.


\short's solution is inspired by an observation that, in a smooth convex function, the steepness of its first derivative drops when approaching its global minimum, due to a positive semidefinite Hessian matrix, (i.e.,  the second derivative of the function). 
This gives the function, if plotted, a flat valley bottom. 
As such, a gradient descent algorithm $\mathcal{A}$, when applied on a convex objective function $F$, could start with a colony of discrete points.
Iteratively descending the colony using the joint gradient of the colony would lead $\mathcal{A}$ to the neighborhoods of the ``flat valley bottom'' where $F$'s global minimum is. 
The points in the colony would also end up with similar losses that are close to the global minimum. 


%the gradient descent algorithm $\mathcal{A}$, when applied on a convex %\highlight{convex} \baigd{do we have to restrict GCD to convex function?} %\yanjun{yes, our convergence is guaranteed based on the assumption of convexity}
%objective function $F$, could start with a colony of nearby %proximate
%points. Iteratively descending using the joint gradient of the colony would lead $\mathcal{A}$ to another colony at the neighborhood of the optimum of $F$.
%Our idea is inspired by ... \baigd{observation? theorem? any mathematical theorem to support something like ``in a convex objective function f, the optimization algorithm could start with multiple discrete points, and the sum of the gradient at those points lead the algorithm to a neighborhood of the optimal of f"}
%\add{We thus design the workflow of \short as follows.} 
We thus design the workflow of \short as follows.
It first lets each participant %\highlight{randomly}
randomly initialize the starting point of their own confined models. %\remove{solely}.
%The weight initialization scheme and the hyper-parameter for adjusting the range of the initial weight are also confined within each participant to protect the information about the average model distance.
A default setting is to sample based on the Gaussian distribution of mean 0 and the variance 1, %and then calibrated by the sample size,
i.e., the standard weight initialization scheme used in %\add{most} machine learning \add{approaches}
most machine learning approaches~\cite{glorot2010understanding}. %\baigd{Good. Be careful when you use ``random''. It is quite different from its Chinese translation, also vague. Either uniformly random or non-uniformly random could be called random. When you sample something at random, you sample it based on some distribution}
%\short lets each participant arbitrarily~\baigd{is this to strong?} initialize their own confined models.
%That is, to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$ to protect the information about the average model distance
In every training iteration, each participant independently computes the local gradient from its current confined model and local data.
All %\replace{of them}{participants} 
participants then jointly work out the \emph{sum} of all local gradients in a secure way and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
In this way, \short is guaranteed to converge to %\replace{a model parameter}{confined models}
confined models adjacent to the %\add{ideal}
ideal global model %\replace{learned when}{that were to learn}
that learned using aggregated data~(referred to as the \emph{centralized model}). %\baigd{We need to unify this. Sometimes we use central model}
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}).
%, and thus we call the convergence a \emph{bounded convergence}.
%In addition, in order to protect the information about the average model distance, \short introduces a hyper-parameter, which is also confined within each participant, for adjusting the range of the initial weight.

%\short retains the merits of traditional FL such as algorithm independence and \highlight{asynchronicity}. \baigd{I am not sure on asynchronicity, because participants need to jointly work out the sum to proceed with update}
\short retains the merits of traditional FL such as algorithm independence. %\replace{the algorithm independence in traditional FL}{the merits of traditional FL such as algorithm independence}.
Therefore, it can easily accommodate any FL schemes regardless of their underlying machine/deep learning algorithms.
To prevent adversaries from learning indirect information from the local gradients of other participants,
we further equip \short with the secure sharing of the sum of the local gradients.
This has been proven to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}.
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL.
In addition, to avoid leaking the average distance between the confined models,
\short allows independent initialization of the confined models.
%\highlight{Our experiment finds that it keeps robust~(in terms of accuracy?) at a difference by X orders (cf. Section X). } \baigd{to update}
Our experiment finds that it keeps robust in terms of validation accuracy at a difference by $2$ orders %\add{of magnitude}
of magnitude on the interval range of initial weights~(cf. Section \ref{sec:init}).%\yanjun{interval?}

%\short introduces a hyper-parameter for adjusting the range of the initial weight.
%\highlight{In addition, to further protect the information about the average model distance, we  introduces a hyper-parameter for adjusting the range of the initial weight, which is also confined within each participant. }
%\yanjun{Here, I refer the hyper-parameter to $\delta$. My thought is to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$, which increase the difficulty of inferring the the average model distance. Would you think it may alleviate the concern on the privacy aspect of the privacy-utitily tradeoff?}

We conduct theoretical and experimental evaluation on \short.
We formally prove that the confined models learned by \short are proximal to the centralized model with bounded gap,
%\highlight{The variance indicates the tradeoff between the adversary's knowledge of the average model distance and the accuracy of the confined models, } \baigd{check this}
and %\replace{it}{the bound} 
the bound is adjustable via tuning hyper-parameters. %\remove{ in the short optimization}.
Our experimental results on two %\add{popular benchmark}
popular benchmark datasets demonstrate that the accuracy performance of \short closely approaches the %\replace{optimal}{product}
product of its centralized counterpart, with marginal differences on validation loss ~(within 0.128 on  MNIST and  0.049 on CIFAR-10) and  accuracy~(within 3.8\% on MNIST and 1.43\% on  CIFAR-10), and outperforms state-of-art federated learning with differential privacy. 


%of validation  accuracy between \short and the centralized baseline is within $0.5\%$ on  MNIST and $1.43\%$ on  CIFAR-10

%For example, in the experiment on the  MNIST dataset, \short achieves  $97.08\%$ in validation  accuracy with $(1000 \times 112)$ participants , which closely approaches $97.61\%$ our centralized learning baseline in which the validation loss  and  accuracy are $0.078$ and $97.61\%$ respectively.
%... \baigd{give some statistics on accuracy here}

\paragraph{Contributions}
We summarize the main contributions as follows.

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	A new optimization algorithm \short for privacy-preserving decentralized FL is proposed.
	%We propose a new optimization algorithm \short for privacy-preserving decentralized FL.
	%\replace{In short, we eliminate}{\short eliminates}
	\short eliminates the explicit sharing of the global model and lets each participant learn a proprietary confined model.
	%\replace{We also eliminate}{It also eliminates}
	It also eliminates the necessity of a central coordinating server, %\replace{and}{such that}
	such that the optimization can be conducted in a fully decentralized manner.
%\baigd{does secure addition scheme need a central server?} \yanjun{some need, some need not, depending on the choice of particular technique}
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short under %\remove{certain} \baigd{certain will emphasize the specialty of assumptions} 
	realistic assumptions on the loss function (such as convexity).
	We prove \short converges toward the centralized model as the number of iterations increases. %\remove{optimal of centralized training}{central model} \replace{with regard to the number of iterations}{as the number of iterations increases}.
	The distance between the trained confined models and the centralized model is bounded, and can be tuned by the hyper-parameter setting.

	\item \textbf{Provable Privacy Preservation.}
	%We prove the \highlight{privacy preservation} \baigd{too strong} of \short, demonstrating 
	We demonstrate that in \short,
    given only the \emph{sum} of the local gradients, %\baigd{We demonstrate that in \short, } 
	an \emph{honest-but-curious} white-box adversary who may control $t$ out of $m$ participants~(where $t \leq m-2$), including the aggregator for secure addition operation~(if any), can learn no information other than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Functional Evaluations.} We implement \short and conduct experiments on MNIST and CIFAR-10 datasets.
	The results demonstrate that \short can closely approach the performance of centralized learning on the validation loss and accuracy. %, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro6.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
To increase dataset participation from multiple dataset owners/entities, %and \highlight{reduce barriers for sharing datasets to another party,} \baigd{I don't think this is true, as it implies the entities can freely share datasets} 
federated learning (FL) approaches are proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
%Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow and PyTorch, and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or %\replace{its}{SGD}
the mini-batch mode)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in centralized FL)~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep} or a peer-to-peer communication scheme~(in decentralized FL)~\cite{kim2019blockchained, roy2019braintorrent}.
Each of them obtains the current model parameters, works out a local gradient based on the local data, and
disseminates it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared are still susceptible to attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}. %\remove{ (illustrated in Figure ref{fig:fl})}.
%can be abused to infer information about the raw datasets (refer to~\cite{nasr2019comprehensive} and also illustrated in Figure \ref{fig:fl}).
%\highlight{abused by the model inversion attack to infer information about the raw datasets} (illustrated in Figure \ref{fig:fl}). \baigd{Is this precise?} \yanjun{I thought we might not restrict the attack to the model inversion attack, as there are also some others in the literature such as membership inference attack, model extraction attack...?} \baigd{Then a single reference and Figure 1a is too weak to support your argument. You can say such as model inversion [] and membership inference [] }

This work further decreases the dependency among FL participants by %approaching the ambition of
\emph{eliminating the explicit sharing of the central global model} which is the root cause of the information leakage~\cite{fredrikson2015model, nasr2019comprehensive}.  %model inversion attack
We propose a new optimization algorithm named \codename (\short) that enables each participant to learn a proprietary global model.
%\replace{Each of them}{A \short participant}
The \short participants maintain %\replace{their}{its}
their global models locally, which are strictly confined within %\replace{themselves}{itself}
themselves from the  beginning of and throughout the whole training process. %\remove{(Figure ref{fig:confined})}.
We name these localized global models as \emph{confined models}, to distinguish them from the global model in traditional FL.
%\add{We also illustrate the comparison between our work and traditional FL in Figure}~\ref{fig:compgd}.
In Figure~\ref{fig:compgd}, we %\replace{also}{further}
 illustrate %\replace{the}{a holistic}
a holistic comparison between our work and traditional FL.

\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$ using the descent computed by $f$. %, \add{e.g., the XXX function}.
	Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and $f$, the adversary is able to derive information about the local raw data $\xi_a, \xi_b, \xi_c$.
	 %values of $f$ \baigd{This sentence is too long. Does $f$ have a name in ML context? } which is a composite function for computing the model updates with \replace{arguments $w$ and  $\xi_a, \xi_b, \xi_c$}{local gradients?}, the adversary is able to derive information about the raw data.
	 ]{{\includegraphics[width=7cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
\subfloat[\codename. Each participant strictly confines their own global models from their initialization~($w_0^a, w_0^b, w_0^c$) to optimal values~($w_*^a, w_*^b, w_*^c$).
The confined models descend in the same pace, and when \short converges, reach the bottom of the valley where the centralized model is located.  %\replace{a ``almost flat land" near the centralized optimal point where the loss is close to minimun}{the valley where the central model is located},
%\remove{The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data.} \baigd{it is said in the text}
Any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$ would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.
]{{\includegraphics[width=6.2cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Comparison of \short and the gradient descent in  traditional FL. %\replace{$w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration,}{This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$}, and $iter$ \replace{is the abstraction to indicate}{represents} the sum-up of all iterations. %\replace{are the abstractions for model updates going through all training iterations.}{indicate the model updates}
		This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$, and $iter$ represents the sum-up of all iterations.
	}
	%\baigd{some confusion here: $iter_{FL}$ and $iter_{\short}$ indicate one iteration or sum-up of all iterations? Confirm this and you will know whether you need $w_k$ or $w$}
	\label{fig:compgd}
\end{figure*}

%\baigd{Check my writing at the bottom of this paragraph}
%The key observation that inspires \short's solution is that, when a convex smooth function moves to its global minimum, the steepness of its first derivative will decrease and become flat when the function converges.
%the Hessian matrix (i.e. the second derivative) of a convex function is positive semidefinite. It indicates that the steepness of the error curve will decrease towards its global minimum, and become very gradual when the function converges.
%As such, a gradient descent algorithm $\mathcal{A}$, when applied on a convex objective function $F$, could start with a colony of discrete points.
%Iteratively descending the colony would lead it to the neighborhood of a flat valley bottom where the loss is close to minimum.


%\short's solution is inspired by an observation that, in a smooth convex function, the steepness of its first derivative drops gradually slower when approaching its global minimum, due to \add{the small values in the} \remove{a positive} \baigd{you may want to confirm this, as I don't know what semidefinite Hessian matrix is} semidefinite Hessian matrix, (i.e.,  the second derivative of the function).
%Hessian of the cost (i.e.,  the second derivative) at the optimum ~\cite{bottou2012stochastic}

\short's solution is inspired by an observation that, in the common cost function surface, the steepness of the function's first derivative decreases slower when approaching its minimum, due to the small values in its Hessian (i.e.,  the second derivative) near the optimum ~\cite{bottou2012stochastic}. %in the cost 
This gives the function, if plotted, a flat valley bottom.
As such, a gradient descent algorithm $\mathcal{A}$, when applied on a objective function $F$, could start with a colony of discrete points.
Iteratively descending the colony using the joint gradient of the colony would lead $\mathcal{A}$ to the neighborhood of the $F$'s  minimum  in the ``flat valley bottom''.
The points in the colony would also end up with similar losses that are close to the  minimum.


%the gradient descent algorithm $\mathcal{A}$, when applied on a convex %\highlight{convex} \baigd{do we have to restrict GCD to convex function?} %\yanjun{yes, our convergence is guaranteed based on the assumption of convexity}
%objective function $F$, could start with a colony of nearby %proximate
%points. Iteratively descending using the joint gradient of the colony would lead $\mathcal{A}$ to another colony at the neighborhood of the optimum of $F$.
%Our idea is inspired by ... \baigd{observation? theorem? any mathematical theorem to support something like ``in a convex objective function f, the optimization algorithm could start with multiple discrete points, and the sum of the gradient at those points lead the algorithm to a neighborhood of the optimal of f"}
%\add{We thus design the workflow of \short as follows.}
We thus design the workflow of \short as follows.
It first lets each participant %\highlight{randomly}
randomly initialize the starting point of their confined models. %\remove{solely}.
%The weight initialization scheme and the hyper-parameter for adjusting the range of the initial weight are also confined within each participant to protect the information about the average model distance.
A default setting is to sample based on the Gaussian distribution of mean 0 and the variance 1, %and then calibrated by the sample size,
i.e., the standard weight initialization scheme used in %\add{most} machine learning \add{approaches}
most machine learning approaches~\cite{glorot2010understanding}. %\baigd{Good. Be careful when you use ``random''. It is quite different from its Chinese translation, also vague. Either uniformly random or non-uniformly random could be called random. When you sample something at random, you sample it based on some distribution}
%\short lets each participant arbitrarily~\baigd{is this to strong?} initialize their own confined models.
%That is, to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$ to protect the information about the average model distance
In every training iteration, each participant independently computes the local gradient from its current confined model and local data.
All %\replace{of them}{participants}
participants then jointly work out the \emph{sum} of all local gradients in a secure way and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
In this way, \short is guaranteed to converge to %\replace{a model parameter}{confined models}
confined models adjacent to the %\add{ideal}
ideal global model %\replace{learned when}{that were to learn}
that were to learn using aggregated data~(referred to as the \emph{centralized model}). %\baigd{We need to unify this. Sometimes we use central model}
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}).
%, and thus we call the convergence a \emph{bounded convergence}.
%In addition, in order to protect the information about the average model distance, \short introduces a hyper-parameter, which is also confined within each participant, for adjusting the range of the initial weight.

%\short retains the merits of traditional FL such as algorithm independence and \highlight{asynchronicity}. \baigd{I am not sure on asynchronicity, because participants need to jointly work out the sum to proceed with update}
\short retains the merits of traditional FL such as algorithm independence. %\replace{the algorithm independence in traditional FL}{the merits of traditional FL such as algorithm independence}.
Therefore, it can easily accommodate any FL schemes regardless of their underlying machine/deep learning algorithms.
To prevent adversaries from learning indirect information from the local gradients of other participants,
we further equip \short with the secure sharing of the sum of the local gradients.
This has been proved to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}.
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL.
In addition, to avoid leaking the average distance among the confined models,
\short allows the participants to independently initialize their confined models.
%\highlight{Our experiment finds that it keeps robust~(in terms of accuracy?) at a difference by X orders (cf. Section X). } \baigd{to update}
Our experiment finds that it keeps robust in terms of accuracy at a difference by $2$ orders %\add{of magnitude}
of magnitude on the interval range of initial weights~(cf. Section \ref{sec:init}).%\yanjun{interval?}

%\short introduces a hyper-parameter for adjusting the range of the initial weight.
%\highlight{In addition, to further protect the information about the average model distance, we  introduces a hyper-parameter for adjusting the range of the initial weight, which is also confined within each participant. }
%\yanjun{Here, I refer the hyper-parameter to $\delta$. My thought is to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$, which increase the difficulty of inferring the the average model distance. Would you think it may alleviate the concern on the privacy aspect of the privacy-utitily tradeoff?}

We conduct theoretical and experimental evaluation on \short.
We formally prove that the confined models learned by \short are proximal to the centralized model with bounded gaps,
%\highlight{The variance indicates the tradeoff between the adversary's knowledge of the average model distance and the accuracy of the confined models, } \baigd{check this}
and %\replace{it}{the bound}
the bound is adjustable via tuning hyper-parameters. %\remove{ in the short optimization}.
Our experimental results on two %\add{popular benchmark}
popular benchmark datasets demonstrate that the accuracy performance of \short closely approaches the %\replace{optimal}{product}
product of its centralized counterpart, with marginal differences on validation loss ~(mostly within  0.05) and  accuracy~(mostly within  1\%). %, \highlight{and outperforms state-of-the-art federated learning with differential privacy.}


%of validation  accuracy between \short and the centralized baseline is within $0.5\%$ on  MNIST and $1.43\%$ on  CIFAR-10

%For example, in the experiment on the  MNIST dataset, \short achieves  $97.08\%$ in validation  accuracy with $(1000 \times 112)$ participants , which closely approaches $97.61\%$ our centralized learning baseline in which the validation loss  and  accuracy are $0.078$ and $97.61\%$ respectively.
%... \baigd{give some statistics on accuracy here}

\paragraph{Contributions}
We summarize the main contributions as follows.

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	A new optimization algorithm \short for privacy-preserving decentralized FL is proposed.
	%We propose a new optimization algorithm \short for privacy-preserving decentralized FL.
	%\replace{In short, we eliminate}{\short eliminates}
	\short eliminates the explicit sharing of the global model and lets each participant learn a proprietary confined model.
	%\replace{We also eliminate}{It also eliminates}
	It also eliminates the necessity of a central coordinating server, %\replace{and}{such that}
	such that the optimization can be conducted in a fully decentralized manner.
%\baigd{does secure addition scheme need a central server?} \yanjun{some need, some need not, depending on the choice of particular technique}
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short under %\remove{certain} \baigd{certain will emphasize the specialty of assumptions}
	realistic assumptions on the loss function (such as convexity).
	We prove \short converges toward the centralized model as the number of iterations increases. %\remove{optimal of centralized training}{central model} \replace{with regard to the number of iterations}{as the number of iterations increases}.
	The distance between the trained confined models and the centralized model is bounded, and can be tuned by the hyper-parameter setting.

	\item \textbf{Provable Privacy Preservation.}
	%We prove the \highlight{privacy preservation} \baigd{too strong} of \short, demonstrating
	We demonstrate that in \short,
    given only the \emph{sum} of the local gradients, %\baigd{We demonstrate that in \short, }
	an \emph{honest-but-curious} white-box adversary who may control $t$ out of $m$ participants~(where $t \leq m-2$), including the aggregator for secure addition operation~(if any), can learn no information other than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Functional Evaluations.} We implement \short and conduct experiments on MNIST and CIFAR-10 datasets.
	The results demonstrate that \short can closely approach the performance of centralized learning on the validation loss and accuracy. %, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro7.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
To increase \highlight{dataset participation}\baigd{sounds weird} from multiple dataset owners/entities, %and \highlight{reduce barriers for sharing datasets to another party,} \baigd{I don't think this is true, as it implies the entities can freely share datasets}
\highlight{federated learning (FL) approaches} \baigd{can't it simply be ``federated learning''?} are proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
%Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
\highlight{It} \baigd{If you say approaches, this can't be it} enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow and PyTorch, \baigd{citation} and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or %\replace{its}{SGD}
the mini-batch mode)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in \add{the} centralized FL)~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep} or a peer-to-peer communication scheme~(in \add{the} decentralized FL)~\cite{kim2019blockchained, roy2019braintorrent}.
Each of them obtains the current model parameters, works out a local gradient based on the local data, and
disseminates it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared are still susceptible to attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}. %\remove{ (illustrated in Figure ref{fig:fl})}.
%can be abused to infer information about the raw datasets (refer to~\cite{nasr2019comprehensive} and also illustrated in Figure \ref{fig:fl}).
%\highlight{abused by the model inversion attack to infer information about the raw datasets} (illustrated in Figure \ref{fig:fl}). \baigd{Is this precise?} \yanjun{I thought we might not restrict the attack to the model inversion attack, as there are also some others in the literature such as membership inference attack, model extraction attack...?} \baigd{Then a single reference and Figure 1a is too weak to support your argument. You can say such as model inversion [] and membership inference [] }

This work further decreases the dependency among \remove{FL} participants by %approaching the ambition of
\emph{eliminating the explicit sharing of the central global model} which is the root cause of the information leakage~\cite{fredrikson2015model, nasr2019comprehensive}.  %model inversion attack
We propose a new optimization algorithm named \codename (\short) that enables each participant to learn a proprietary global model.
%\replace{Each of them}{A \short participant}
The \short participants maintain %\replace{their}{its}
their global models locally, which are strictly confined within %\replace{themselves}{itself}
themselves from the  beginning of and throughout the whole training process. %\remove{(Figure ref{fig:confined})}.
We \replace{name}{refer to} these localized global models as \emph{confined models}, to distinguish them from the global model in traditional FL.
%\add{We also illustrate the comparison between our work and traditional FL in Figure}~\ref{fig:compgd}.
In Figure~\ref{fig:compgd}, we %\replace{also}{further}
 illustrate %\replace{the}{a holistic}
a holistic comparison between our work and traditional FL.

\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$ using the descent computed by $f$. %, \add{e.g., the XXX function}.
	Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and $f$, the adversary is able to derive information about the local raw data $\xi_a, \xi_b, \xi_c$.
	 %values of $f$ \baigd{This sentence is too long. Does $f$ have a name in ML context? } which is a composite function for computing the model updates with \replace{arguments $w$ and  $\xi_a, \xi_b, \xi_c$}{local gradients?}, the adversary is able to derive information about the raw data.
	 ]{{\includegraphics[width=7cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
\subfloat[\codename. Each participant strictly confines their own global models from their initialization~($w_0^a, w_0^b, w_0^c$) to optimal values~($w_*^a, w_*^b, w_*^c$).
The confined models descend in the same pace, and when \short converges, reach the bottom of the valley where the centralized model is located.  %\replace{a ``almost flat land" near the centralized optimal point where the loss is close to minimun}{the valley where the central model is located},
%\remove{The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data.} \baigd{it is said in the text}
Any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$ would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.
]{{\includegraphics[width=6.2cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Comparison of \short and the gradient descent in  traditional FL. %\replace{$w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration,}{This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$}, and $iter$ \replace{is the abstraction to indicate}{represents} the sum-up of all iterations. %\replace{are the abstractions for model updates going through all training iterations.}{indicate the model updates}
		This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$, and $iter$ represents the sum-up of all iterations.
	}
	%\baigd{some confusion here: $iter_{FL}$ and $iter_{\short}$ indicate one iteration or sum-up of all iterations? Confirm this and you will know whether you need $w_k$ or $w$}
	\label{fig:compgd}
\end{figure*}

%\baigd{Check my writing at the bottom of this paragraph}
%The key observation that inspires \short's solution is that, when a convex smooth function moves to its global minimum, the steepness of its first derivative will decrease and become flat when the function converges.
%the Hessian matrix (i.e. the second derivative) of a convex function is positive semidefinite. It indicates that the steepness of the error curve will decrease towards its global minimum, and become very gradual when the function converges.
%As such, a gradient descent algorithm $\mathcal{A}$, when applied on a convex objective function $F$, could start with a colony of discrete points.
%Iteratively descending the colony would lead it to the neighborhood of a flat valley bottom where the loss is close to minimum.


%\short's solution is inspired by an observation that, in a smooth convex function, the steepness of its first derivative drops gradually slower when approaching its global minimum, due to \add{the small values in the} \remove{a positive} \baigd{you may want to confirm this, as I don't know what semidefinite Hessian matrix is} semidefinite Hessian matrix, (i.e.,  the second derivative of the function).
%Hessian of the cost (i.e.,  the second derivative) at the optimum ~\cite{bottou2012stochastic}

\short\remove{'s solution} is inspired by an observation that, in the\baigd{a?} \highlight{common}\baigd{what does common mean?} cost function surface, the steepness of the function's first derivative decreases slower when approaching its minimum, due to the small values in its Hessian (i.e.,  the second derivative) near the optimum ~\cite{bottou2012stochastic}. %in the cost
This gives the function, if plotted, a flat valley bottom.
As such, a gradient descent algorithm $\mathcal{A}$, when applied on an objective function $F$, could start with \highlight{a colony of discrete points}\baigd{a set of adjacent points~(referred to as a \emph{colony})??}.
Iteratively descending the colony using the joint gradient of the colony would lead $\mathcal{A}$ to the neighborhood of \remove{the} $F$'s  minimum  in the ``flat valley bottom''.
The points in the colony would also end up with similar losses that are close to the  minimum. \baigd{Is this correct: losses close to the minimum? I think it should be ``similar losses that are close to the loss of the minimum''?}


%the gradient descent algorithm $\mathcal{A}$, when applied on a convex %\highlight{convex} \baigd{do we have to restrict GCD to convex function?} %\yanjun{yes, our convergence is guaranteed based on the assumption of convexity}
%objective function $F$, could start with a colony of nearby %proximate
%points. Iteratively descending using the joint gradient of the colony would lead $\mathcal{A}$ to another colony at the neighborhood of the optimum of $F$.
%Our idea is inspired by ... \baigd{observation? theorem? any mathematical theorem to support something like ``in a convex objective function f, the optimization algorithm could start with multiple discrete points, and the sum of the gradient at those points lead the algorithm to a neighborhood of the optimal of f"}
%\add{We thus design the workflow of \short as follows.}
We thus design the workflow of \short as follows.
It first lets each participant %\highlight{randomly}
randomly initialize the starting point of their confined models. %\remove{solely}.
%The weight initialization scheme and the hyper-parameter for adjusting the range of the initial weight are also confined within each participant to protect the information about the average model distance.
A default setting is to sample based on the Gaussian distribution of mean 0 and the variance 1, %and then calibrated by the sample size,
i.e., the standard weight initialization scheme used in %\add{most} machine learning \add{approaches}
most machine learning approaches~\cite{glorot2010understanding}. \baigd{more citations since ``most''} %\baigd{Good. Be careful when you use ``random''. It is quite different from its Chinese translation, also vague. Either uniformly random or non-uniformly random could be called random. When you sample something at random, you sample it based on some distribution}
%\short lets each participant arbitrarily~\baigd{is this to strong?} initialize their own confined models.
%That is, to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$ to protect the information about the average model distance
In every training iteration, each participant independently computes the local gradient from its current confined model and local data.
All %\replace{of them}{participants}
participants then jointly work out the \emph{sum} of all local gradients in a secure way and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
In this way, \short is guaranteed to converge to %\replace{a model parameter}{confined models}
confined models adjacent to the %\add{ideal}
ideal global model %\replace{learned when}{that were to learn}
that were to learn using aggregated data~(referred to as the \emph{centralized model}). %\baigd{We need to unify this. Sometimes we use central model}
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}).
%, and thus we call the convergence a \emph{bounded convergence}.
%In addition, in order to protect the information about the average model distance, \short introduces a hyper-parameter, which is also confined within each participant, for adjusting the range of the initial weight.

%\short retains the merits of traditional FL such as algorithm independence and \highlight{asynchronicity}. \baigd{I am not sure on asynchronicity, because participants need to jointly work out the sum to proceed with update}
\short retains the merits of traditional FL such as algorithm independence. %\replace{the algorithm independence in traditional FL}{the merits of traditional FL such as algorithm independence}.
Therefore, it can easily accommodate any FL schemes regardless of their underlying machine/deep learning algorithms.
To prevent adversaries from learning indirect information from the local gradients of other participants,
we further equip \short with the secure sharing of the sum of the local gradients.
This has been proved to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}.
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL.
In addition, to avoid leaking the average distance among the confined models,
\short allows the participants to independently initialize their confined models.
%\highlight{Our experiment finds that it keeps robust~(in terms of accuracy?) at a difference by X orders (cf. Section X). } \baigd{to update}
Our experiment finds that \highlight{it keeps robust in terms of accuracy at a difference by $2$ orders %\add{of magnitude}
of magnitude on the interval range of initial weights}~(cf. Section \ref{sec:init}). \baigd{its accuracy is stable even when the interval ranges of initial weights differ by two orders of magnitude }
%\yanjun{interval?}

%\short introduces a hyper-parameter for adjusting the range of the initial weight.
%\highlight{In addition, to further protect the information about the average model distance, we  introduces a hyper-parameter for adjusting the range of the initial weight, which is also confined within each participant. }
%\yanjun{Here, I refer the hyper-parameter to $\delta$. My thought is to let each participant initialize their confined model based on its own randomization scheme $\mathit{Rand}$ and $\delta$, which increase the difficulty of inferring the the average model distance. Would you think it may alleviate the concern on the privacy aspect of the privacy-utitily tradeoff?}

We conduct theoretical and experimental evaluation on \short.
We formally prove that the confined models learned by \short are proximal to the centralized model with bounded gaps,
%\highlight{The variance indicates the tradeoff between the adversary's knowledge of the average model distance and the accuracy of the confined models, } \baigd{check this}
and %\replace{it}{the bound}
the bound is adjustable via tuning hyper-parameters. %\remove{ in the short optimization}.
Our experimental results on two %\add{popular benchmark}
popular benchmark datasets demonstrate that the accuracy performance of \short closely approaches the %\replace{optimal}{product}
product of its centralized counterpart, with marginal differences on validation loss ~(mostly within  0.05) and  accuracy~(mostly within  1\%). %, \highlight{and outperforms state-of-the-art federated learning with differential privacy.}


%of validation  accuracy between \short and the centralized baseline is within $0.5\%$ on  MNIST and $1.43\%$ on  CIFAR-10

%For example, in the experiment on the  MNIST dataset, \short achieves  $97.08\%$ in validation  accuracy with $(1000 \times 112)$ participants , which closely approaches $97.61\%$ our centralized learning baseline in which the validation loss  and  accuracy are $0.078$ and $97.61\%$ respectively.
%... \baigd{give some statistics on accuracy here}

\paragraph{Contributions}
We summarize the main contributions as follows.

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	A new optimization algorithm \short for privacy-preserving decentralized FL is proposed. \baigd{We propose ...}
	%We propose a new optimization algorithm \short for privacy-preserving decentralized FL.
	%\replace{In short, we eliminate}{\short eliminates}
	\short eliminates the explicit sharing of the global model and lets each participant learn a proprietary confined model.
	%\replace{We also eliminate}{It also eliminates}
	It also eliminates the necessity of a central coordinating server, %\replace{and}{such that}
	such that the optimization can be conducted in a fully decentralized manner.
%\baigd{does secure addition scheme need a central server?} \yanjun{some need, some need not, depending on the choice of particular technique}
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short under %\remove{certain} \baigd{certain will emphasize the specialty of assumptions}
	realistic assumptions on the loss function (such as convexity).
	We prove \short converges toward the centralized model as the number of iterations increases. %\remove{optimal of centralized training}{central model} \replace{with regard to the number of iterations}{as the number of iterations increases}.
	The distance between the trained confined models and the centralized model is bounded, and can be tuned by the hyper-parameter setting.

	\item \textbf{Provable Privacy Preservation.}
	%We prove the \highlight{privacy preservation} \baigd{too strong} of \short, demonstrating
	We demonstrate that in \short,
    given only the \emph{sum} of the local gradients, %\baigd{We demonstrate that in \short, }
	an \emph{honest-but-curious} white-box adversary, who may control $t$ out of $m$ participants~(where $t \leq m-2$) including the aggregator for secure addition operation~(if any), can learn no information other than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	
	
	\item \textbf{Functional Evaluations.} We implement \short and conduct experiments on MNIST and CIFAR-10 datasets.
	The results demonstrate that \short can closely approach the performance of centralized learning on the validation loss and accuracy. %, and significantly outperform the local training.
	
\end{itemize}



==> chapters/intro8.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
%To increase \highlight{dataset participation}\baigd{sounds weird} from multiple dataset owners/entities, %and \highlight{reduce barriers for sharing datasets to another party,} \baigd{I don't think this is true, as it implies the entities can freely share datasets}
%\highlight{federated learning (FL) approaches} \baigd{can't it simply be ``federated learning''?} are proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
%Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
To take advantage of massive data owned by multiple entities, federated learning (FL) is proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}. 
%\highlight{It} \baigd{If you say approaches, this can't be it} 
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow~\cite{abadi2016tensorflow} and PyTorch~\cite{paszke2019pytorch}, %\baigd{citation} 
and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or %\replace{its}{SGD}
the mini-batch mode)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in the centralized FL)~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep} or a peer-to-peer communication scheme~(in the decentralized FL)~\cite{kim2019blockchained, roy2019braintorrent}.
Each of them obtains the current model parameters, works out a local gradient based on the local data, and
disseminates it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared are still susceptible to attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}. 

This work further decreases the dependency among %\remove{FL}  
participants by %approaching the ambition of
\emph{eliminating the explicit sharing of the central global model} which is the root cause of the information leakage~\cite{fredrikson2015model, nasr2019comprehensive}.  %model inversion attack
We propose a new optimization algorithm named \codename (\short) that enables each participant to learn a proprietary global model.
%\replace{Each of them}{A \short participant}
The \short participants maintain %\replace{their}{its}
their global models locally, which are strictly confined within %\replace{themselves}{itself}
themselves from the  beginning of and throughout the whole training process. %\remove{(Figure ref{fig:confined})}.
We refer to these localized global models as \emph{confined models}, to distinguish them from the global model in traditional FL.

\short %\remove{'s solution} 
is inspired by an observation that, in the %\baigd{a?} \highlight{common}\baigd{what does common mean?} 
most cost functions' surface, the steepness of the function's first derivative decreases slower when approaching its minimum, due to the small values in its Hessian (i.e.,  the second derivative) near the optimum ~\cite{bottou2012stochastic}. %in the cost
This gives the function, if plotted, a flat valley bottom.
As such, a gradient descent algorithm $\mathcal{A}$, when applied on an objective function $F$, could start with \highlight{a colony of discrete points}\baigd{a set of adjacent points~(referred to as a \emph{colony})??}.
Iteratively descending the colony using the joint gradient of the colony would lead $\mathcal{A}$ to the neighborhood of  $F$'s  minimum  in the ``flat valley bottom''.
The points in the colony would also end up with similar losses that are close to the loss of the minimum. %\baigd{Is this correct: losses close to the minimum? I think it should be ``similar losses that are close to the loss of the minimum''?}

\highlight{\short follows the general workflow of a gradient decent in traditional FL. }
In Figure~\ref{fig:compgd}, we illustrate a holistic comparison between the workflow of a gradient decent in traditional FL and that in \short . 
\short has \highlight{delicate variances} meant to \emph{enhance privacy without sacrificing much model accuracy}. 
For the sake of simplicity, we refer to them as \emph{privacy} and \emph{accuracy}. \yanjun{Can I change to ``accuracy" as I thought ``correctness" may emphasize more on the equivalence between the centralzied training and \short, and ``accuracy" is maybe closer to the desired property that we aim to achieve?} %\emph{correctness}. 
\baigd{I may be wrong as I missed the validation loss. Anyway, define privacy and correctness here}
\highlight{In the remaining of this paper, we focus on the trade-off between them. }
\begin{itemize}
	\item \textbf{Privacy.} The framework should ensure that neither any of the owner’s local data or any intermediate results compute on its local data be observed by other parties or a third aggregator throughout the training process.
	
	\item \textbf{Accuracy.} The prediction made by any confined  model should approach the \emph{centralized model} that were to learn using all the data gathered centrally.
\end{itemize}

In the following, we discuss the workflow of \short, and how the desired privacy and accuracy is achieved.
\paragraph{Initialization} 
Participants in \short should hide their initial points from each other to achieve the desired privacy. 
To this end, \short lets each participant $l$ independently initialize the starting point of its confined model $w_1^l$ (As shown in Figure \ref{fig:confined},  participants $a, b, c$ solely initialize $w_1^a, w_1^b, w_1^c$).
A default setting is to sample based on the Gaussian distribution of mean 0 and the variance 1, which is the standard weight initialization scheme used in most machine learning approaches~\cite{glorot2010understanding, krizhevsky2017imagenet, mishkin2015all}. 
Furthermore, to prevent the colluding participants from inferring others' points by the knowledge of the average distance among the confined models, we introduce a hyper-parameter $\delta^l$ to control the interval range of initial weights $w_1^l$, i.e., $w_1^l \sim   N[-\delta^l, \delta^l]$, and allows each participant $l$ to independently choose its own $\delta^l$.
% \baigd{one sentence like ``if XXX, the colluding participants may infer XXX based on the points their models are located''} 

A proper initialization is also important to the desired accuracy from the following two aspects. (1) Just like that in the centralized training, an inappropriate initialization will drastically impact the accuracy performance, e.g., setting initial weights with very small values will cause numerical instabilities.
(2) When \short converges, the maximum gap between \short's solutions and the centralized optimal is bounded, and such gap is in linear with the distance among initial points of confined model (detailed in Section \ref{sec:convergence}). 
%\baigd{describe the concern on the initialization. What should be addressed by it? }

We find, theoretically and experimentally, that the weight initialization scheme ($w_1^l \sim N[-\delta^l, \delta^l]$) has been sufficient for both. 
Our experiment also finds accuracy performance is stable even when the interval ranges of initial weights $\delta^l$ differ by two orders of magnitude among participants.

%We find \baigd{experimentally or theoretically?} that the standard weight initialization scheme used in most machine learning approaches~\cite{glorot2010understanding}, \baigd{more citations since ``most''}
%i.e., sampling based on the Gaussian distribution of mean 0 and the variance 1, has been sufficient for both. 
%Our experiment finds that \highlight{it keeps robust in terms of accuracy at a difference by $2$ orders %\add{of magnitude}
%of magnitude on the interval range of initial weights}~(cf. Section \ref{sec:init}). \baigd{its accuracy is stable even when the interval ranges of initial weights differ by two orders of magnitude }
%\baigd{will rewrite the last sentence}

\paragraph{Training Iteration} In every training iteration, participants independently compute the local gradient from their current confined model and local data, and then jointly work out the \emph{sum} of all local gradients and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
Secrecy of intermediate local gradients~(for privacy) and convergence~(for accuracy) are our main concerns during this process. 

For privacy, we incorporate the secure addition operation on the local gradients to calculate their sum.
This has been proved to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}.
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL.
In addition, any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$ (in Figure \ref{fig:confined}) would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.

For accuracy, updating the colony with the aggregated gradients ensures \short converges to 
confined models that are adjacent to the centralized model. 
%ideal global model 
%that were to learn using aggregated data~(referred to as the \emph{centralized model}). 
\baigd{there are two aspects here: 1. convergence: what guarantees convergence? 2. converge to neighborhood of optimal: what guarantee this? }
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}).

\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$ using the descent computed by $f$. %, \add{e.g., the XXX function}.
	Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and $f$, the adversary is able to derive information about the local raw data $\xi_a, \xi_b, \xi_c$.
	 %values of $f$ \baigd{This sentence is too long. Does $f$ have a name in ML context? } which is a composite function for computing the model updates with \replace{arguments $w$ and  $\xi_a, \xi_b, \xi_c$}{local gradients?}, the adversary is able to derive information about the raw data.
	 ]{{\includegraphics[width=7cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
\subfloat[\codename. Each participant strictly confines their own global models from their initialization~($w_0^a, w_0^b, w_0^c$) to optimal values~($w_*^a, w_*^b, w_*^c$).
The confined models descend in the same pace, and when \short converges, reach the bottom of the valley where the centralized model is located.  %\replace{a ``almost flat land" near the centralized optimal point where the loss is close to minimun}{the valley where the central model is located},
%\remove{The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data.} \baigd{it is said in the text}
Any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$  would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.
]{{\includegraphics[width=6.2cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Comparison of \short and the gradient descent in  traditional FL. %\replace{$w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration,}{This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$}, and $iter$ \replace{is the abstraction to indicate}{represents} the sum-up of all iterations. %\replace{are the abstractions for model updates going through all training iterations.}{indicate the model updates}
		This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$, and $iter$ represents the sum-up of all iterations.
	}
	%\baigd{some confusion here: $iter_{FL}$ and $iter_{\short}$ indicate one iteration or sum-up of all iterations? Confirm this and you will know whether you need $w_k$ or $w$}
	\label{fig:compgd}
\end{figure*}


\iffalse
\short retains the merits of traditional FL such as algorithm independence. 
Therefore, it can easily accommodate any FL schemes regardless of their underlying machine/deep learning algorithms.
We conduct theoretical and experimental evaluation on \short.
We formally prove that the confined models learned by \short are proximal to the centralized model with bounded gaps,
and the bound is adjustable via tuning hyper-parameters. 
Our experimental results on two 
popular benchmark datasets demonstrate that the accuracy performance of \short closely approaches the 
product of its centralized counterpart, with marginal differences on validation loss ~(mostly within  0.05) and  accuracy~(mostly within  1\%). 
\fi

\paragraph{Contributions}
We summarize the main contributions as follows.

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	We propose a new optimization algorithm \short for privacy-preserving decentralized FL. %\baigd{We propose ...}
	%We propose a new optimization algorithm \short for privacy-preserving decentralized FL.
	%\replace{In short, we eliminate}{\short eliminates}
	\short  eliminates the explicit sharing of the global model and lets each participant learn a proprietary confined model.
	%\replace{We also eliminate}{It also eliminates}
	It also eliminates the necessity of a central coordinating server, %\replace{and}{such that}
	such that the optimization can be conducted in a fully decentralized manner.
%\baigd{does secure addition scheme need a central server?} \yanjun{some need, some need not, depending on the choice of particular technique}
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short under %\remove{certain} \baigd{certain will emphasize the specialty of assumptions}
	realistic assumptions on the loss function (such as convexity).
	We prove \short converges toward the centralized model as the number of iterations increases. %\remove{optimal of centralized training}{central model} \replace{with regard to the number of iterations}{as the number of iterations increases}.
	The distance between the trained confined models and the centralized model is bounded, and can be tuned by the hyper-parameter setting.

	\item \textbf{Enhanced Privacy Preservation Over Traditional FL.}
	%We prove the \highlight{privacy preservation} \baigd{too strong} of \short, demonstrating
	We prove that in \short,
    given only the \emph{sum} of the local gradients, %\baigd{We demonstrate that in \short, }
	an \emph{honest-but-curious} white-box adversary, who may control $t$ out of $m$ participants~(where $t \leq m-2$) including the aggregator for secure addition operation~(if any), can learn no information other than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	We also demonstrate CGD’s privacy enhancement over traditional privacy-preserving FL from the perspective of the attacker’s observation.
	We prove that less information is exposed in CGD compared to that of traditional FL.
	
	
	\item \textbf{Functional Evaluations.} We implement \short and conduct experiments on two popular benchmark datasets MNIST and CIFAR-10.
	The results demonstrate that \short can closely approach the performance of centralized model on the validation loss and accuracy, %, and significantly outperform the local training.
	%Our experimental results on demonstrate that the accuracy performance of \short closely approaches the 
	%product of its centralized counterpart, 
	with marginal differences on validation loss ~(mostly within  0.05) and  accuracy~(mostly within  1\%).
	
\end{itemize}



==> chapters/intro9.tex <==
\section{Introduction}
%
The performance of machine learning largely relies on the availability of large representative datasets.
%To increase \highlight{dataset participation}\baigd{sounds weird} from multiple dataset owners/entities, %and \highlight{reduce barriers for sharing datasets to another party,} \baigd{I don't think this is true, as it implies the entities can freely share datasets}
%\highlight{federated learning (FL) approaches} \baigd{can't it simply be ``federated learning''?} are proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
%Federated learning~(FL) is thus proposed to take advantage of a vast range of data owned by multiple entities~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
To take advantage of massive data owned by multiple entities, federated learning (FL) is proposed~\cite{konevcny2016federated, yang2019federated, konevcny2016federatedo}.
%\highlight{It} \baigd{If you say approaches, this can't be it}
It enables participants to jointly train a global model without the necessity of sharing their datasets, demonstrating the potential to address the issues of data privacy and data ownership. %\baigd{Is it correct to move these citations here?}
It has been incorporated by popular machine learning tools such as TensorFlow~\cite{abadi2016tensorflow} and PyTorch~\cite{paszke2019pytorch}, %\baigd{citation}
and increasingly spread over various industries.

The privacy preservation of FL stems from its parallelization of the gradient descent optimization, which in essence is an application of stochastic gradient descent (SGD)~(or %\replace{its}{SGD}
the mini-batch mode)~\cite{konevcny2016federated}.
During the training process, the participants work on the same intermediate global model via a coordinating server~(in the centralized FL)~\cite{bonawitz2017practical, mohassel2017secureml, abadi2016deep} or a peer-to-peer communication scheme~(in the decentralized FL)~\cite{kim2019blockchained, roy2019braintorrent}.
Each of them obtains the current model parameters, works out a local gradient based on the local data, and
disseminates it to update the global model synchronously~\cite{abadi2016deep,bonawitz2017practical} or asynchronously~\cite{hu2019fdml}.
This paradigm guarantees data locality, but has been found insufficient for data privacy:
although the local gradients can be securely synthesized via a variety of techniques such as differential privacy (DP)~\cite{abadi2016deep, shokri2015privacy,hu2019fdml,zhang2020differentially}, secure multi-party communication (MPC)~\cite{bonawitz2017practical, mohassel2017secureml,gascon2017privacy}, and homomorphic encryption (HE)~\cite{mohassel2017secureml, marc2019privacy, sharma2019confidential}, %\baigd{separate the citations}
the global model parameters that have to be shared are still susceptible to attacks such as model inversion~\cite{ateniese2015hacking, fredrikson2015model} and membership inference~\cite{nasr2019comprehensive}.

This work further decreases the dependency among %\remove{FL}
participants by %approaching the ambition of
\emph{eliminating the explicit sharing of the central global model} which is the root cause of the information leakage~\cite{fredrikson2015model, nasr2019comprehensive}.  %model inversion attack
We propose a new optimization algorithm named \codename (\short) that enables each participant to learn a proprietary global model.
%\replace{Each of them}{A \short participant}
The \short participants maintain %\replace{their}{its}
their global models locally, which are strictly confined within %\replace{themselves}{itself}
themselves from the  beginning of and throughout the whole training process. %\remove{(Figure ref{fig:confined})}.
We refer to these localized global models as \emph{confined models}, to distinguish them from the global model in traditional FL.

%\replace{short %\remove{'s solution} 
%is inspired by an observation that, the %\baigd{a?} \highlight{common}\baigd{what does common mean?}
%most cost functions' surface, the steepness of the function's first derivative decreases slower when approaching its minimum, due to the small values in its Hessian (i.e.,  the second derivative) near the optimum}{
\short %\remove{'s solution}
is inspired by an observation on the surface of the typical cost function.  
The steepness of the first derivative decreases slower when approaching the minimum of the function, due to the small values in the Hessian (i.e.,  the second derivative) near the optimum~\cite{bottou2012stochastic}. %}in the cost
This gives the function, when plotted, a flat valley bottom.
As such, a gradient descent algorithm $\mathcal{A}$, when applied on an objective function $F$, could start with a set of discrete points with certain distance (referred to as a \emph{colony}). 
%a colony of \highlight{ a set of discrete points with certain distance}\baigd{a set of adjacent points~(referred to as a \emph{colony})??}.
Iteratively descending the colony using the joint gradient of the colony would lead $\mathcal{A}$ to the neighborhood of  $F$'s  minimum  in the ``flat valley bottom''.
The points in the colony would also end up with similar losses that are close to the loss of the minimum. %\baigd{Is this correct: losses close to the minimum? I think it should be ``similar losses that are close to the loss of the minimum''?}

%\highlight{\short follows the general workflow of a gradient decent in traditional FL. }
In Figure~\ref{fig:compgd}, we illustrate a holistic comparison between the workflow of a gradient decent in traditional FL and that in \short .
In traditional FL, every participant updates the \emph{same} global model $w$ using their local gradients $g^a, g^b, g^c$. 
In \short,  each participant $l$ first independently initialize the starting point of its confined model $w_1^l$. 
Then, in every training iteration, participants independently compute the local gradient from their current confined model and local data, and then jointly work out the \emph{sum} of all local gradients and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
%\short has \highlight{delicate variances} meant to 
By doing this, \short aims to \emph{enhance privacy without sacrificing much model accuracy}.
For the sake of simplicity, we refer to them as \emph{privacy} and \emph{accuracy}. %\yanjun{Can I change to ``accuracy" as I thought ``correctness" may emphasize more on the equivalence between the centralzied training and \short, and ``accuracy" is maybe closer to the desired property that we aim to achieve?} %\emph{correctness}.
%\baigd{I may be wrong as I missed the validation loss. Anyway, define privacy and correctness here}
%\highlight{In the remaining of this paper, we focus on the trade-off between them. }
\begin{itemize}
	\item \textbf{Privacy.} %\replace{The framework }{\short}should ensure that \replace{neither any of the owner's local data or any intermediate results compute on its local data be observed by other parties or a third aggregator throughout the training process.}{, throughout the training process, neither local data of a participant nor intermediate results computed on them can be observed by other participants or a aggregator.}
	\short should ensure that, throughout the training process, neither local data of a participant nor intermediate results computed on them can be observed by other participants or a aggregator.
	\item \textbf{Accuracy.} The prediction made by any confined  model should approach the \emph{centralized model} that were to learn using all the data gathered centrally.
\end{itemize}
\short achieves desired privacy preservation from the following two aspects. 
(1) Secrecy of confined models. 
Participants in \short hide their proprietary global models from each other throughout the training process. 
In the beginning, each participant independently initializes its $w_1^l$ at random. 
Throughout the training process, any two confined models keep the same distance, i.e., they will not become closer to each other during descending, preventing any participant from predicting models of others. 
In addition, \short allows each participant to choose its own interval range of initial weights to avoid leaking the average distance between the confined models.
(2) Secrecy of local gradients. We incorporate the secure addition operation on the local gradients to calculate their sum.
This has been proved to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}.
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL. 
With secrecy of both confined model and local gradients, \short  achieves enhanced privacy preservation over traditional FL. 
We prove that the adversary's observation in \short is only the sum of local gradients,  whereas in traditional FL, extra indicative information about local data can be obtained~(cf. Section~\ref{sec:privacy}).

A highlight of \short is its theoretical guarantee of convergence. 
We prove that, updating the colony with the aggregated gradients ensures \short converges to confined models that are adjacent to the centralized model, and this adjacency is bounded~(cf. Section~\ref{sec:convergence}). 
Our experiments shows that, the performance of \short can closely approach to the centralized learning with standard initialization scheme, (i.e., each participant randomly initializes its $w_1^l$ based on the Gaussian distribution of mean 0 and the variance 1) %, with marginal differences on validation loss~(mostly within  0.05) and  accuracy~(mostly within  1\%)
~(cf. Section~\ref{subsec:performace}). 
Our experiment also finds accuracy performance is stable even when the interval ranges of initial weights among participants differ by two orders of magnitude~(cf. Section~\ref{sec:init}).

\iffalse
In the following, we discuss the workflow of \short, and how the desired privacy and accuracy is achieved. \yanjun{too detailed, general idea, move to workflow}
\paragraph{Initialization}
Participants in \short should hide their initial points from each other to achieve the desired privacy. 
To this end, \short lets each participant $l$ independently initialize the starting point of its confined model $w_1^l$ (As shown in Figure \ref{fig:confined},  participants $a, b, c$ solely initialize $w_1^a, w_1^b, w_1^c$).
A default setting is to sample based on the Gaussian distribution of mean 0 and the variance 1, which is the standard weight initialization scheme used in most machine learning approaches~\cite{glorot2010understanding, krizhevsky2017imagenet, mishkin2015all}.
Furthermore, to prevent the colluding participants from inferring others' points by the knowledge of the average distance among the confined models, we introduce a hyper-parameter $\delta^l$ to control the interval range of initial weights $w_1^l$, i.e., $w_1^l \sim   N[-\delta^l, \delta^l]$, and allows each participant $l$ to independently choose its own $\delta^l$.
% \baigd{one sentence like ``if XXX, the colluding participants may infer XXX based on the points their models are located''}

A proper initialization is also important to the desired accuracy from the following two aspects. (1) Just like that in the centralized training, an inappropriate initialization will drastically impact the accuracy performance, e.g., setting initial weights with very small values will cause numerical instabilities.
(2) When \short converges, the maximum gap between \short's solutions and the centralized optimal is bounded, and such gap is in linear with the distance among initial points of confined model (detailed in Section \ref{sec:convergence}).
%\baigd{describe the concern on the initialization. What should be addressed by it? }

We find, theoretically and experimentally, that the weight initialization scheme ($w_1^l \sim N[-\delta^l, \delta^l]$) has been sufficient for both.
Our experiment also finds accuracy performance is stable even when the interval ranges of initial weights $\delta^l$ differ by two orders of magnitude.

%We find \baigd{experimentally or theoretically?} that the standard weight initialization scheme used in most machine learning approaches~\cite{glorot2010understanding}, \baigd{more citations since ``most''}
%i.e., sampling based on the Gaussian distribution of mean 0 and the variance 1, has been sufficient for both.
%Our experiment finds that \highlight{it keeps robust in terms of accuracy at a difference by $2$ orders %\add{of magnitude}
%of magnitude on the interval range of initial weights}~(cf. Section \ref{sec:init}). \baigd{its accuracy is stable even when the interval ranges of initial weights differ by two orders of magnitude }
%\baigd{will rewrite the last sentence}

\paragraph{Training Iteration} In every training iteration, participants independently compute the local gradient from their current confined model and local data, and then jointly work out the \emph{sum} of all local gradients and use it to update their confined models~(the equation in Figure \ref{fig:confined}).
Secrecy of intermediate local gradients~(for privacy) and convergence~(for accuracy) are our main concerns during this process.

For privacy, we incorporate the secure addition operation on the local gradients to calculate their sum.
This has been proved to be viable through the additive secret sharing scheme, in which the sum of a set of secret values is collaboratively calculated without revealing any addends~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}.
A previous study~\cite{zhang2020privcoll} demonstrates it is efficient when applied to achieve decentralization in FL.
In addition, any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$ (in Figure \ref{fig:confined}) would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.

For accuracy, updating the colony with the aggregated gradients ensures \short converges to
confined models that are adjacent to the centralized model.
%ideal global model
%that were to learn using aggregated data~(referred to as the \emph{centralized model}).
\baigd{there are two aspects here: 1. convergence: what guarantees convergence? 2. converge to neighborhood of optimal: what guarantee this? }
This adjacency is proved to be bounded~(cf. Section~\ref{sec:convergence}).
\fi

\begin{figure*}[!t]
	\centering
	\subfloat[Gradient descent in traditional federated learning. Participants jointly work on the same global model $w$ using the descent computed by $f$. %, \add{e.g., the XXX function}.
	Although the local gradients $g^a, g^b, g^c$ can be securely synthesized, by knowing $w$ and $f$, the adversary is able to derive information about the local raw data $\xi_a, \xi_b, \xi_c$.
	 %values of $f$ \baigd{This sentence is too long. Does $f$ have a name in ML context? } which is a composite function for computing the model updates with \replace{arguments $w$ and  $\xi_a, \xi_b, \xi_c$}{local gradients?}, the adversary is able to derive information about the raw data.
	 ]{{\includegraphics[width=7cm]{fig/federated.pdf} \label{fig:fl}}}%
	\qquad
\subfloat[\codename. Each participant strictly confines their own global models from their initialization~($w_0^a, w_0^b, w_0^c$) to optimal values~($w_*^a, w_*^b, w_*^c$).
The confined models descend in the same pace, and when \short converges, reach the bottom of the valley where the centralized model is located.  %\replace{a ``almost flat land" near the centralized optimal point where the loss is close to minimun}{the valley where the central model is located},
%\remove{The only shared information is the \emph{sum} of the local gradients which hides both the confined models and the raw data.} \baigd{it is said in the text}
Any two confined models keep the same distance throughout the training process.
In other words, $w^a, w^b, w^c$  would not become closer to each other during descending, %in favor of \replace{privacy}{unpredictability}.
preventing any participant from predicting models of others.
]{{\includegraphics[width=6.2cm]{fig/confined.pdf} \label{fig:confined}}}%
	\caption{Comparison of \short and the gradient descent in  traditional FL. %\replace{$w, w^a, w^b, w^c$ are the abstractions of the traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ for all $k^{th}$ iteration,}{This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$}, and $iter$ \replace{is the abstraction to indicate}{represents} the sum-up of all iterations. %\replace{are the abstractions for model updates going through all training iterations.}{indicate the model updates}
		This figure does not differentiate each iteration: the occurrences of traditional FL's global model $w_k$ and confined models $w_k^a, w_k^b, w_k^c$ in all iterations are represented by $w, w^a, w^b, w^c$, and $iter$ represents the sum-up of all iterations.
	}
	%\baigd{some confusion here: $iter_{FL}$ and $iter_{\short}$ indicate one iteration or sum-up of all iterations? Confirm this and you will know whether you need $w_k$ or $w$}
	\label{fig:compgd}
\end{figure*}


\iffalse
\short retains the merits of traditional FL such as algorithm independence.
Therefore, it can easily accommodate any FL schemes regardless of their underlying machine/deep learning algorithms.
We conduct theoretical and experimental evaluation on \short.
We formally prove that the confined models learned by \short are proximal to the centralized model with bounded gaps,
and the bound is adjustable via tuning hyper-parameters.
Our experimental results on two
popular benchmark datasets demonstrate that the accuracy performance of \short closely approaches the
product of its centralized counterpart, with marginal differences on validation loss ~(mostly within  0.05) and  accuracy~(mostly within  1\%).
\fi

\paragraph{Contributions}
We summarize the main contributions as follows.

\begin{itemize}
	\item \textbf{\codename For Privacy-preserving Decentralized Federated Learning.}
	We propose a new optimization algorithm \short for privacy-preserving decentralized FL. %\baigd{We propose ...}
	%We propose a new optimization algorithm \short for privacy-preserving decentralized FL.
	%\replace{In short, we eliminate}{\short eliminates}
	\short  eliminates the explicit sharing of the global model and lets each participant learn a proprietary confined model.
	%\replace{We also eliminate}{It also eliminates}
	It also eliminates the necessity of a central coordinating server, %\replace{and}{such that}
	such that the optimization can be conducted in a fully decentralized manner.
%\baigd{does secure addition scheme need a central server?} \yanjun{some need, some need not, depending on the choice of particular technique}
	
	\item \textbf{Convergence Analysis.}
	We theoretically establish a convergence rate for  \short under %\remove{certain} \baigd{certain will emphasize the specialty of assumptions}
	realistic assumptions on the loss function (such as convexity).
	We prove \short converges toward the centralized model as the number of iterations increases. %\remove{optimal of centralized training}{central model} \replace{with regard to the number of iterations}{as the number of iterations increases}.
	The distance between the trained confined models and the centralized model is bounded, and can be tuned by the hyper-parameter setting.

	\item \textbf{Enhanced Privacy Preservation Over Traditional FL.}
	%We prove the \highlight{privacy preservation} \baigd{too strong} of \short, demonstrating
	We prove that in \short,
    given only the \emph{sum} of the local gradients, %\baigd{We demonstrate that in \short, }
	an \emph{honest-but-curious} white-box adversary, who may control $t$ out of $m$ participants~(where $t \leq m-2$) including the aggregator for secure addition operation~(if any), can learn no information other than their own inputs and the \emph{sum} of the local gradients from other honest parties.
	We also demonstrate CGD’s privacy enhancement over traditional privacy-preserving FL from the perspective of the attacker’s observation.
	We prove that less information is exposed in CGD compared to that of traditional FL.
	
	
	\item \textbf{Functional Evaluations.} We implement \short and conduct experiments on two popular benchmark datasets MNIST and CIFAR-10.
	The results demonstrate that \short can closely approach the performance of centralized model on the validation loss and accuracy, %, and significantly outperform the local training.
	%Our experimental results on demonstrate that the accuracy performance of \short closely approaches the
	%product of its centralized counterpart,
	with marginal differences on validation loss ~(mostly within  0.05) and  accuracy~(mostly within  1\%).
	
\end{itemize}



==> chapters/privacy.tex <==
\section{Privacy Preservation}
\label{sec:privacy}
By confining $w_k^l$ within each participants, we are able to achieve privacy preservation. 
%The property of privacy preservation can be simply achieved. 
Since each participant learns and confines a different global model $w_k^l$, and the randomness introduced in the initialization to $w_1^l$  can be regarded as random masks to make the final global model $w_*^l$ to be private. 

In \short, the only information shared among the participants is $ \sum\limits_{j=1}^{m}g^j(w^j_{k}, \xi_j)$, i.e., the sum of local gradients. 
Since the addends $g^l(w^l_{k}, \xi_l)$ are computed from a function of $w^l_{k} \cdot \xi_l$, a direct release of it may leak information about the $\xi_l$ or $w^l_k$ during training iterations~\cite{zhang2020privcoll}.  
Therefore, we incorporate secure addition operation on the local gradients to  protect information about $w_k^l$ or $\xi_l$ during the training iterations. 
We note that there are a variety of existing tools for secure addition operation~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic}, 
one of which is called \emph{additive secret sharing scheme} proposed by \cite{bogdanov2008sharemind}. 
It uses additive sharing over $\mathbb{Z}_{2^{32}}$ for securely evaluating addition operations in a multiparty computation environment,
and guarantees privacy preservation even though the majority ($m-2$ out of $m$) of participants are corrupted\footnote{We detail the additive secret sharing scheme in Appendix \ref{apx:secret}}.

In the following, we formally prove the \emph{view} of the adversary party via the simulation paradigm~\cite{goldreich2019play}\footnote{The background of the simulation paradigm is given in Appendix \ref{apx:sim}} to demonstrate that, given only the sum of the local gradients which are computed on different confined model, an  \emph{honest-but-curious} adversary\footnote{Refer to a white-box adversary who have access to the training internals such as network architecture, and can also observe the intermediate computations during the training iterations.} who may control $t$ out of $m$ participants (where $t \leq m-2$), including the aggregator for secure addition operation (if there is any), can learn ``nothing more” than their own inputs and the sum of the local gradients from other honest parties. 

Before stating the results, we introduce some notations. The involved parties in our framework are $m$ participants nodes denoted by $l \in [1, m]$. 
Denote  $g_k^{m^\prime} = \{g_k^l(w^l_{k}, \xi_l)\}_{l \in m^\prime}$ as the local gradients of any subset of participants nodes $m^\prime \subseteq m$ at $k^{th}$ iteration. 
Let  $t$ be the aforementioned adversary threshold, where $t \leq m-2$.
Given any subset $c \subseteq m$ of the parties, let $VIEW_{real} (g_k^m, t, \mathcal{P}, c)$ denote the combined views of all colluding parties $c$ from the execution of a real protocol $\mathcal{P}$. 
Let $VIEW_{ideal} (g_k^c, z, t, \mathcal{F}_p, c)$ denote the views of $c$ from an ideal execution that securely computes a functionality $\mathcal{F}_p$, where $z$ is the information required by the simulator $\mathcal{S}$ in the ideal execution for simulation.

The following theorem shows that when executing \short with threshold $t$, the joint view of any subset of compromised participants nodes can be simulated given the inputs of the participants nodes in that group, as well as the sum of the local gradients from the remaining honest nodes, i.e., $\sum g_k^l\mid_{l \in m \setminus  c}$, which is the only information 	that the adversary can and only can learn during the execution.

\begin{theorem}
	\label{theorem_party}
	There exists a simulator $\mathcal{S}$ such that for all $t, m, X^m$ and $c$ such that $c \subseteq m$, $\lvert c \lvert \leq t$, the output of $\mathcal{S}$ from $VIEW_{ideal}$ is perfectly indistinguishable from the output of  $VIEW_{real} $, namely
	\[ VIEW_{real} (g_k^m, t, \mathcal{P}, c) \equiv VIEW_{ideal} (g_k^c, z, t, \mathcal{F}_p, c)\]
	where
	\[z = \sum g_k^l\mid_{l \in m \setminus  c}\]
\end{theorem}


\begin{proof}
	We  define the simulator $\mathcal{S}$  through each of the $k^{th}$ training iteration as:
	
	$\text{\textbf{SIM}}_1$: This is the simulator $\mathcal{S}$ for the first training iteration.
	
	Since the inputs of parties in $c$ does not depend on the inputs of the parties not in $c$, instead of sending the actual $g_1^{m \setminus c}$ of the parties $m \setminus  c$ to compute $\sum g_1^m$, the simulator $\mathcal{S}$ can produce a simulation by running the parties $m \setminus  c$ on  a set of pseudorandom vectors  $\eta_1^{m \setminus c} =  \{\eta_1^l\}_{l \in m \setminus c}$ in a way that 
	\[\sum \eta_1^{m \setminus c} = \sum \eta_1^l\mid_{l \in m \setminus c} = \sum g_1^m - \sum g_1^c = \sum g_1^l\mid_{l \in m \setminus  c}\]
	
	Since each  $g_1^l(w^l_{1}, \xi_l)$ is computed from its respective confined model $w_1^l$ which is randomized in the initialization, the pseudorandom vectors $\eta_1^{m \setminus c} $ generated by the simulator $\mathcal{S}$ for the inputs of all honest parties $m \setminus  c$, and the joint view of parties in $c$ in  $VIEW_{ideal}$, will be identical to that in $VIEW_{real}$, namely		
	\[ (\sum \eta_1^{m \setminus c} + \sum g_1^c )\equiv \sum g_1^m,\]
	and the information required by  $\mathcal{S}$ is $z = \sum g_1^l\mid_{l \in m \setminus  c}$.
	%where "$\equiv$" denotes that the two distributions are identical.
	
	$\text{\textbf{SIM}}_{k+1} ( k\geq 1)$: This is the simulator $\mathcal{S}$ for the $(k+1)^{th}$ training iteration. 
	
	In $Real$ execution, $\sum g_{k+1}^m$ is computed as
	\begin{equation}
		\label{equ:real}
		\begin{aligned}
			\sum g_{k+1}^m & = \sum g_{k+1}^l (w^l_{k+1}, \xi_l)\mid_{l \in m} = \sum g_{k+1}^l (w^l_{k} - \alpha_k \sum g_{k}^m, \xi_l)\mid_{l \in m}\\
			&=\sum g_{k+1}^l \big(w^l_{1} -\sum_{i=1}^{k} (\alpha_i \sum g_{i}^m), \xi_l\big)\mid_{l \in m}
		\end{aligned}
	\end{equation}
	
	In $Ideal$ execution, since each $g_{k+1}^l(w^l_{k+1}, \xi_l)\mid_{l \in m}$ is also computed from $w_1^l$ which is randomized in the initialization, the simulator $\mathcal{S}$ can again produce a simulation by running the parties $m \setminus  c$ on  a set of pseudorandom vectors  $\eta_{k+1}^{m \setminus c} =  \{\eta_{k+1}^l\}_{l \in m \setminus c}$ in a way that 
	\[\sum \eta_{k+1}^{m \setminus c} = \sum \eta_{k+1}^l\mid_{l \in m \setminus c} = \sum g_{k+1}^m - \sum g_{k+1}^c = \sum g_{k+1}^l\mid_{l \in m \setminus  c}\].
	
	As such, the joint view of parties in $c$ in  $VIEW_{ideal}$, will be identical to that in $VIEW_{real}$
	\[ (\sum \eta_{k+1}^{m \setminus c} + \sum g_{k+1}^c )\equiv \sum g_{k+1}^m,\]
	and the information required by  $\mathcal{S}$ is $z = \sum g_{k+1}^l\mid_{l \in m \setminus  c}$.
	
	
	Thus, the output of the simulator $VIEW_{ideal}$ of each training iteration is perfectly indistinguishable from the output of $VIEW_{real}$, and knowledge of $z$ is sufficient for the simulation, completing the proof.
	
\end{proof}

From the above proof, we can also demonstrate that sharing or synthesizing one and the same global model (even if the local gradients are protected) in traditional FL is still subject to information leakage of the original dataset. 
Since the information required by the simulator $\mathcal{S}$ is $\sum g_{k}^l (w^l_{k}, \xi_l)\mid_{l \in m \setminus c}$,
if every participant learns/shares one and the same model, which is equivalent to the case that $w_k^l\mid_ {l \in m \setminus c}$ is known to the everyone,  
then by knowing both $\sum g_{k}^l (w^l_{k}, \xi_l)\mid_{l \in m \setminus c}$ and $w_k^l\mid_ {l \in m \setminus c}$, the adversary is able to infer information  of the original dataset $\xi$.



%The proof also demonstrate that, if every participant learns/shares one and the same global model, even though the local gradients are protected, the training process is still subject to information leakage of the original dataset $\xi$.







==> chapters/privacy1.tex <==
\section{Privacy Preservation}
\label{sec:privacy}
%By confining $w_k^l$ within each participants, we are able to achieve privacy preservation.
%The property of privacy preservation can be simply achieved.
%Since each participant learns and confines a different global model $w_k^l$, and the randomness introduced in the initialization to $w_1^l$  can be regarded as random masks to make the final global model $w_*^l$ to be private. \baigd{maybe just remove this paragraph, or tune down to one sentence, as the argument on the random initialization seems not so strong.}

In \short, the only information shared among the participants is $ \sum\limits_{j=1}^{m}g^j(w^j_{k}, \xi_j)$, i.e., the sum of local gradients.
Since the addends $g^l(w^l_{k}, \xi_l)$ are computed from a function of $w^l_{k} \cdot \xi_l$, %\replace{a direct release of}{releasing} 
releasing it may leak information about the $\xi_l$ or $w^l_k$ %\remove{during training iterations}
~\cite{zhang2020privcoll}.
%\replace{Therefore,}{To address this,} 
To address this, we incorporate secure addition operation on the local gradients to  protect information about $w_k^l$ or $\xi_l$ during the training iterations.
We note that there are a variety of existing tools for secure addition operation~\cite{bonawitz2017practical, bogdanov2008sharemind, lin2005efficient, tebaa2012homomorphic},
one of which is called \emph{additive secret sharing scheme} proposed by %\add{Bogdanov et al}
Bogdanov et al~\cite{bogdanov2008sharemind}.
It uses additive sharing over $\mathbb{Z}_{2^{32}}$ for securely evaluating addition operations in a multiparty computation environment,
and guarantees privacy preservation even though the majority ($m-2$ out of $m$) of participants are %\replace{corrupted}{compromised}
compromised\footnote{We detail the additive secret sharing scheme in Appendix \ref{apx:secret}.}.

In %\replace{the following}{this section}
this section, we formally prove the \emph{view} of the adversary party via the simulation paradigm\footnote{The background of the simulation paradigm is given in Appendix \ref{apx:sim}.}~\cite{goldreich2019play}. 
We assume an  \emph{honest-but-curious} white-box adversary\footnote{The white-box adversary refers to the one who have access to the training internals such as network architecture, and can also observe the intermediate computations during the training iterations.} who may control $t$ out of $m$ participants (where $t \leq m-2$), including the aggregator for secure addition operation (if any).
We demonstrate that, given only the sum of the local gradients which are computed on different confined model, the adversary can learn no information other %\replace{``nothing more''}{no information other} \baigd{why quote mark here?} 
than their own inputs and the sum of the local gradients from other honest parties. %\baigd{The whole paragraph includes only one sentence. Separate it. Show the development of your idea}

%\replace{Before stating the results,}{To facilitate the understanding on our analysis,} 
To facilitate the understanding on our analysis, we %\replace{introduce some notations}{first present the used notations}
first present the used notations. The involved parties in our framework are a set $\mathcal{L}$ of $m$ participants nodes denoted with logical identities $l \in [1, m]$.
Denote  $g_k^{\mathcal{L}^\prime} = \{g_k^l(w^l_{k}, \xi_l)\}_{l \in \mathcal{L}^\prime}$ as the local gradients of any subset of participants nodes $\mathcal{L}^\prime \subseteq \mathcal{L}$ %\baigd{$m$ is a number, not a set} 
at $k^{th}$ iteration.
Let  $t$ be the aforementioned adversary threshold, where $t \leq m-2$.
Given any subset %\highlight{$c \subseteq \mathcal{L}$}
$c \subseteq \mathcal{L}$  of the participants, let $VIEW_{real} (g_k^\mathcal{L}, t, \mathcal{P}, c)$ denote the combined views of all colluding parties $c$ from the execution of a real protocol $\mathcal{P}$.
Let $VIEW_{ideal} (g_k^c, z, t, \mathcal{F}_p, c)$ denote the views of $c$ from an ideal execution that securely computes a %\replace{functionality}{function} 
function $\mathcal{F}_p$, where $z$ is the information required by the simulator $\mathcal{S}$ in the ideal execution for simulation.

The following theorem shows that when executing \short with threshold $t$, the joint view of any subset of compromised participants %\remove{nodes} 
can be simulated given the inputs of the participants in that subset, 
%\remove{nodes} \highlight{in that group}\baigd{which group? the subset?}, 
as well as the sum of the local gradients from the remaining honest nodes, i.e., $\sum g_k^l\mid_{l \in m \setminus  c}$, %\highlight{which is the only information that the adversary can learn during the execution.} \baigd{rewrite this}
which is the only information that the adversary can learn during the execution.

\begin{theorem}
	\label{theorem_party}
	There exists a simulator $\mathcal{S}$ such that for all $t, \mathcal{L}, X^\mathcal{L}$ and $c$ with $c \subseteq \mathcal{L}$, $\lvert c \lvert \leq t$, the output of $\mathcal{S}$ from $VIEW_{ideal}$ is perfectly indistinguishable from the output of  $VIEW_{real} $, namely
	\[ VIEW_{real} (g_k^\mathcal{L}, t, \mathcal{P}, c) \equiv VIEW_{ideal} (g_k^c, z, t, \mathcal{F}_p, c)\]
	where
	\[z = \sum g_k^l\mid_{l \in \mathcal{L} \setminus  c}\]
\end{theorem}


\begin{proof}
	We  define the simulator $\mathcal{S}$  %\highlight{through each of the $k^{th}$ training iteration} \baigd{rewrite this. The $k^{th}$ training iteration is a single iteration, why use each?} 
	through each training iteration as:
	
	$\text{\textbf{SIM}}_1$: This is the simulator for the first training iteration.
	
	Since the inputs of parties in $c$ does not depend on the inputs of the parties in $\mathcal{L} \setminus c$, 
		${SIM}_1$ can therefore produce a perfect simulation by running $c$ on their true inputs, and all other users $\mathcal{L} \setminus c$ on a set of pseudorandom vectors  $\eta_1^{\mathcal{L} \setminus c} =  \{\eta_1^l\}_{l \in \mathcal{L} \setminus c}$ in a way that
	%instead of sending the actual $g_1^{\mathcal{L} \setminus c}$ of the parties $\mathcal{L} \setminus  c$ to compute $\sum g_1^\mathcal{L}$, the simulator $\mathcal{S}$ can produce a simulation by running the parties $\mathcal{L} \setminus  c$ on  a set of pseudorandom vectors  $\eta_1^{\mathcal{L} \setminus c} =  \{\eta_1^l\}_{l \in \mathcal{L} \setminus c}$ in a way that \baigd{this sentence is too long, cannot get your idea}
	\[\sum \eta_1^{\mathcal{L} \setminus c} = \sum \eta_1^l\mid_{l \in \mathcal{L} \setminus c} = \sum g_1^\mathcal{L} - \sum g_1^c = \sum g_1^l\mid_{l \in \mathcal{L} \setminus  c}\]
	
	Since each  $g_1^l(w^l_{1}, \xi_l)$ is computed from its respective confined model $w_1^l$ which is randomized in the initialization, the pseudorandom vectors $\eta_1^{m \setminus c} $ generated by ${SIM}_1$
	%the \highlight{simulator} \baigd{don't have to mention it everywhere. } $\mathcal{S}$ 
	for the inputs of all honest parties $\mathcal{L} \setminus  c$, and the joint view of parties in $c$ in  $VIEW_{ideal}$, will be identical to that in $VIEW_{real}$, namely		
	\[ (\sum \eta_1^{\mathcal{L} \setminus c} + \sum g_1^c )\equiv \sum g_1^\mathcal{L},\]
	and the information required by  ${SIM}_1$ is $z = \sum g_1^l\mid_{l \in \mathcal{L} \setminus  c}$.
	
	$\text{\textbf{SIM}}_{k+1} ( k\geq 1)$: This is the simulator %\highlight{$\mathcal{S}$} \baigd{distinguish it with the one above} 
	for the $(k+1)^{th}$ training iteration.
	
	In $Real$ execution, $\sum g_{k+1}^\mathcal{L}$ is computed as
	\begin{equation}
		\label{equ:real}
		\begin{aligned}
			\sum g_{k+1}^\mathcal{L} & = \sum g_{k+1}^l (w^l_{k+1}, \xi_l)\mid_{l \in \mathcal{L}} = \sum g_{k+1}^l (w^l_{k} - \alpha_k \sum g_{k}^\mathcal{L}, \xi_l)\mid_{l \in \mathcal{L}}\\
			&=\sum g_{k+1}^l \big(w^l_{1} -\sum_{i=1}^{k} (\alpha_i \sum g_{i}^\mathcal{L}), \xi_l\big)\mid_{l \in \mathcal{L}}
		\end{aligned}
	\end{equation}
	
	In $Ideal$ execution, since each $g_{k+1}^l(w^l_{k+1}, \xi_l)\mid_{l \in \mathcal{L}}$ is also computed from $w_1^l$ which is randomized in the initialization, ${SIM}_{k+1}$ can therefore produce a perfect simulation by running the parties $\mathcal{L} \setminus  c$ on  a set of pseudorandom vectors  $\eta_{k+1}^{\mathcal{L} \setminus c} =  \{\eta_{k+1}^l\}_{l \in \mathcal{L} \setminus c}$ in a way that
	\[\sum \eta_{k+1}^{\mathcal{L} \setminus c} = \sum \eta_{k+1}^l\mid_{l \in \mathcal{L} \setminus c} = \sum g_{k+1}^\mathcal{L} - \sum g_{k+1}^c = \sum g_{k+1}^l\mid_{l \in \mathcal{L} \setminus  c}\].
	
	As such, the joint view of parties in $c$ in  $VIEW_{ideal}$, will be identical to that in $VIEW_{real}$
	\[ (\sum \eta_{k+1}^{\mathcal{L} \setminus c} + \sum g_{k+1}^c )\equiv \sum g_{k+1}^\mathcal{L},\]
	and the information required by  ${SIM}_{k+1}$  is $z = \sum g_{k+1}^l\mid_{l \in \mathcal{L} \setminus  c}$.
	
	
	Thus, the output of the simulator $VIEW_{ideal}$ of each training iteration is perfectly indistinguishable from the output of $VIEW_{real}$, and knowledge of $z$ is sufficient for the simulation, completing the proof.
	
\end{proof}

From the above proof, %\replace{we}{one} 
one can also %\replace{demonstrate}{find} 
find that sharing/synthesizing the same global model  in traditional FL (even if the local gradients are protected) is still subject to information leakage of the original dataset.
Since the information required by the simulator $\mathcal{S}$ is $\sum g_{k}^l (w^l_{k}, \xi_l)\mid_{l \in \mathcal{L} \setminus c}$,
if every participant learns/shares one and the same model, which is equivalent to the case that $w_k^l\mid_ {l \in \mathcal{L} \setminus c}$ is known to the everyone,
then by knowing both $\sum g_{k}^l (w^l_{k}, \xi_l)\mid_{l \in \mathcal{L} \setminus c}$ and $w_k^l\mid_ {l \in \mathcal{L} \setminus c}$, the adversary is able to infer information  of the original dataset $\xi$.



%The proof also demonstrate that, if every participant learns/shares one and the same global model, even though the local gradients are protected, the training process is still subject to information leakage of the original dataset $\xi$.







==> chapters/related.tex <==
\section{Related works}






